IR characteristic emission and dust properties of star-forming galaxies at 4.5 $<$ z $<$ 6.2

The luminosity functions at z < 4 - 5 suggest that most galaxies have a relatively low stellar mass (logM_star = 10) and a low dust attenuation (A_FUV = 1.0). The physical properties of these objects are quite homogeneous. We used an approach where we combined their rest-frame far-infrared and submillimeter emissions and utilized the universe and the redshift as a spectrograph to increase the amount of information in a collective way. From a subsample of 27 ALMA-detected galaxies at z > 4.5, we built an infrared spectral energy distribution composite template. It was used to fit, with CIGALE, the 105 galaxies (detections and upper limits) in the sample from the FUV to the FIR. The derived physical parameters provide information to decipher the nature of the dust cycle and of the stellar populations in these galaxies. The derived IR composite template is consistent with the galaxies in the studied sample. A delayed star formation history with tau_main = 500 Myrs is slightly favored by the statistical analysis as compared to a delayed with a final burst or a continuous star formation history. The position of the sample in the star formation rate (SFR)- M_star diagram is consistent with previous papers. The redshift evolution of the log M_star versus A_FUV relation is in agreement with evolution in the redshift of this relation. This evolution is necessary to explain the cosmic evolution of the average dust attenuation of galaxies. Evolution is also observed in the L_dust/ L_FUV (IRX) versus UV slope beta_FUV diagram: younger galaxies have bluer beta_FUV. We modeled the shift of galaxies in the IRX versus the beta_FUV diagram with the mass-weighted age as a free parameter, and we provide an equation to make predictions.

==> IR_composite.models_27Jul.tex <==
\onecolumn
\sisetup{table-column-width=12ex,    % local setting for all S columns
         round-mode=places,
         round-precision=3,
         tight-spacing,
         table-format = 5.3e-2,
         table-number-alignment = center
         }

\begin{longtable}[c]{|S|S|S|S|}
 
 \caption{IR template for each of the models, normalized to 200 $\mu$m. Only the first rows are given here.}
 \label{Tab.SED_IR.composite.models}\\

 \hline
 \multicolumn{4}{| c |}{Beginning of table}\\
 \hline
    \multicolumn{1}{|c|}{$\lambda[\mu m]$} &
    \multicolumn{1}{c|}{F$_{\nu}$(DL2014)} &
    \multicolumn{1}{c|}{F$_{\nu}$(PL+OTMBB)} &
    \multicolumn{1}{c|}{F$_{\nu}$(PL+GMBB)} \\
 \hline
 \endfirsthead

 \hline
 \multicolumn{4}{| c |}{Continuation of Table~\ref{Tab.SED_IR.composite.models}}\\
 \hline
    \multicolumn{1}{|c|}{$\lambda[\mu m]$} &
    \multicolumn{1}{c|}{F$_{\nu}$(DL2014)} &
    \multicolumn{1}{c|}{F$_{\nu}$(PL+OTMBB)} &
    \multicolumn{1}{c|}{F$_{\nu}$(PL+GMBB)} \\
 \hline
 \endhead

 \hline
 \multicolumn{4}{| c |}{End of Table}\\
 \hline\hline
 \endlastfoot

\hline
  20.0 & 0.18107749474964585 & 0.033371661115243596 & 0.22818696797630056\\
  20.14 & 0.18551481313133614 & 0.03558839180505059 & 0.23284902077654243\\
  20.32 & 0.1916912479528318 & 0.038600899856686154 & 0.23899800048124503\\
  20.51 & 0.19834306021901293 & 0.0419773937900743 & 0.2456753421353187\\
  20.7 & 0.20531825078431543 & 0.0455757038111942 & 0.25255705038272314\\
  20.867 & 0.21165231238228988 & 0.048922292048504665 & 0.2587737366722555\\
  20.89 & 0.21253443514863027 & 0.04939717591545251 & 0.2596425809753937\\
  21.09 & 0.21999878126005848 & 0.05366062340145448 & 0.26731997222221277\\
  21.28 & 0.22778655101786716 & 0.057962443464595954 & 0.27483454092275683\\
  21.48 & 0.23581520065227968 & 0.0627535518665652 & 0.28297431584426264\\
  21.68 & 0.24424326271690508 & 0.06781394324414101 & 0.291347963724405\\
  21.88 & 0.25299471730114265 & 0.07316857457031122 & 0.29996899869856025\\
  22.08 & 0.26199354449542767 & 0.07881443965404047 & 0.3088337861700852\\
\begin{comment}
22.082 & 0.26208493650531245 & 0.07887231603830122 & 0.3089236300384457\\
  22.28 & 0.2712340694615609 & 0.0847529197682631 & 0.3179420030659557\\
  22.49 & 0.2808044784109833 & 0.09132381546404349 & 0.3277767823905905\\
  22.7 & 0.2906982948240248 & 0.0982402248996817 & 0.337888211755694\\
  22.91 & 0.30092199306747625 & 0.10549864770034634 & 0.3482725682829296\\
  23.12 & 0.31162760870823614 & 0.11312255020626029 & 0.358939632786215\\
  23.33 & 0.32273912203875704 & 0.12111043969589304 & 0.3698864279648628\\
  23.367 & 0.3246328638140299 & 0.12255295860875007 & 0.3718428283287594\\
  23.55 & 0.33410507998527345 & 0.1298658169010314 & 0.3816513341074053\\
  23.77 & 0.34580753271713527 & 0.13903942549564813 & 0.39372695656140905\\
  23.99 & 0.3579158978811169 & 0.14862939797504734 & 0.406109743855343\\
  24.21 & 0.3704366500235844 & 0.1586315049734245 & 0.418795702479763\\
  24.43 & 0.3832937696207079 & 0.16906436125192464 & 0.4317889584821318\\
  24.66 & 0.3964937065636398 & 0.18043150123404914 & 0.4456979944500126\\
  24.728 & 0.40048918485669327 & 0.18387449065390407 & 0.44987131145069026\\
  24.89 & 0.4101129611054971 & 0.19226129750006174 & 0.4599346258577945\\
  25.12 & 0.4239927698164249 & 0.20457181854839696 & 0.4744999741413267\\
  25.35 & 0.4383804218061039 & 0.21735893011265744 & 0.4893891153546033\\
  25.59 & 0.4531109187014845 & 0.23120281058256145 & 0.5052659637022994\\
  25.82 & 0.46819722620993215 & 0.24496358266472368 & 0.5208047830612047\\
  26.06 & 0.48371533973635106 & 0.2598328633318763 & 0.5373512630332274\\
  26.167 & 0.49078470206721386 & 0.26662418026629237 & 0.5448366626782501\\
  26.3 & 0.49966558995663873 & 0.27521548353962055 & 0.5542326650492978\\
  26.55 & 0.5160479316020455 & 0.2917929980735861 & 0.5721659193874856\\
  26.79 & 0.5328055105216525 & 0.3082335832384853 & 0.5897098651878467\\
  27.04 & 0.5499949190914902 & 0.32589907659217654 & 0.6083221832830993\\
  27.29 & 0.5675660383130344 & 0.34411734454148923 & 0.6272664840356141\\
  27.54 & 0.5855819344304354 & 0.36288115715867053 & 0.6465352562903721\\
  27.69 & 0.5961897531348711 & 0.37439746768578636 & 0.6582511056055635\\
  27.8 & 0.6040492950582195 & 0.3829655858786667 & 0.6669161355194035\\
  28.05 & 0.6228986721642351 & 0.40282101937482206 & 0.686824222316167\\
  28.31 & 0.642212273073861 & 0.424026173695583 & 0.7078423399760442\\
  28.58 & 0.661914071623796 & 0.4466381770165294 & 0.7300068789223161\\
  28.84 & 0.6820865555535788 & 0.46896879549147735 & 0.7516515252016847\\
  29.11 & 0.7026537063446253 & 0.49272398228550457 & 0.7744316074517003\\
  29.302 & 0.7175269391168585 & 0.5099619803515605 & 0.7908160789531954\\
  29.38 & 0.7236286072319216 & 0.5170490187762744 & 0.7975206334362198\\
  29.65 & 0.7450049892059205 & 0.5419215354053214 & 0.8208883852937892\\
  29.92 & 0.7668650209888308 & 0.5673280370030406 & 0.8445244955008843\\
  30.2 & 0.7890631462650731 & 0.5942344748886714 & 0.8693211602145551\\
  30.48 & 0.8116753732562163 & 0.6216786189421348 & 0.8943731286693564\\
  30.76 & 0.8350187262608603 & 0.6496426282732526 & 0.9196662732346107\\
  31.008 & 0.8548595738509837 & 0.6748402877570486 & 0.942270609355281\\
  31.05 & 0.8582505863484577 & 0.679152332769373 & 0.9461231546231149\\
  31.33 & 0.8823853875605483 & 0.7081317826121426 & 0.9718786649324272\\
  31.62 & 0.9066496661110436 & 0.738629003785026 & 0.9987558240804495\\
  31.92 & 0.9310434163236954 & 0.7706998525777717 & 1.0267876596063015\\
  32.21 & 0.9563268030679799 & 0.8021530236075685 & 1.0540570673591256\\
  32.51 & 0.9817396567584628 & 0.8351333801848314 & 1.0824275627010183\\
  32.81 & 1.007281968227436 & 0.8685716890291104 & 1.1109746611844822\\
  32.813 & 1.0075446730124258 & 0.868909047859161 & 1.111261644181376\\
  33.11 & 1.0337790474781798 & 0.9024096089058432 & 1.1396496950577937\\
  33.36952048760346 & 1.0560393087306388 & 0.9319805905608953 & 1.1645420030360834\\
  33.39464036570259 & 1.0582115504391076 & 0.9348545544738494 & 1.1669534286864196\\
  33.41976024380173 & 1.0626923923329474 & 0.9399071761961062 & 1.1719139063771202\\
  33.41976024380174 & 1.0626923923330192 & 0.9399071761961744 & 1.1719139063771995\\
  33.42 & 1.0650617835622656 & 0.9421483564797614 & 1.1745301604123795\\
  33.444880121900866 & 1.311347503542033 & 1.1750696171260315 & 1.4464319397101713\\
  33.47 & 2.2498406296966516 & 2.060436138498424 & 2.482624271611956\\
  33.49511987809913 & 1.3165394955798453 & 1.181559076081142 & 1.4521015609782482\\
  33.520239756198265 & 1.0715941423987758 & 0.9514893927655277 & 1.1816169847934666\\
  33.545359634297405 & 1.0715034036795315 & 0.9521990062048595 & 1.1814770755177004\\
  33.57047951239654 & 1.0737352779639726 & 0.9550814278494528 & 1.1838852226382652\\
  33.73 & 1.0879865858558098 & 0.9735185421554495 & 1.1992602545702833\\
  34.04 & 1.1156970249644156 & 1.0096149928150595 & 1.2292071182315665\\
  34.36 & 1.1436016940785239 & 1.0471922740720416 & 1.260173788358445\\
  34.67 & 1.1716358189903378 & 1.0839226554306802 & 1.2902469416334723\\
  34.705497704615375 & 1.1748286258464762 & 1.0881622430138425 & 1.2937058352204787\\
  34.724 & 1.1764950786640591 & 1.0903666084317185 & 1.2955034655614932\\
  34.73162327846153 & 1.1771821459555976 & 1.0912693649186411 & 1.2962395748746254\\
  34.75774885230769 & 1.1796110937194264 & 1.0944349673681302 & 1.2988441900058212\\
  34.783874426153844 & 1.1897003707141884 & 1.10482345534816 & 1.3099066280379204\\
  34.81 & 1.2214295542834774 & 1.1356111817395333 & 1.3448622397940095\\
  34.836125573846154 & 1.1944525035319797 & 1.1110684738873944 & 1.3149979787685648\\
  34.86225114769231 & 1.189068884633971 & 1.1068812061603506 & 1.3089755765784234\\
  34.86225114769232 & 1.1890688846339716 & 1.1068812061603517 & 1.3089755765784241\\
  34.88837672153847 & 1.1913681887220415 & 1.109938131798703 & 1.3114359428861413\\
  34.88837672153848 & 1.1913681887220424 & 1.1099381317987038 & 1.311435942886142\\
  34.91450229538463 & 1.1937433486085214 & 1.11306926754336 & 1.3139798426393043\\
  34.99 & 1.200624633115099 & 1.122104510665785 & 1.321314063418568\\
  35.32 & 1.2298077466558792 & 1.1617078271590886 & 1.3533393218672862\\
  35.65 & 1.2591203305234633 & 1.2015835180506698 & 1.3853882802675854\\
  35.90189521238723 & 1.2829061343859565 & 1.2321412938762055 & 1.4098222858554872\\
  35.928921409290425 & 1.2854755905537694 & 1.2354429527507205 & 1.4124551015448998\\
  35.95594760619362 & 1.2882370288379306 & 1.2389003621533614 & 1.4152786092645742\\
  35.97 & 1.300050432448537 & 1.2504728790235664 & 1.4281991341532307\\
  35.982973803096804 & 1.310889392396598 & 1.2611721986146858 & 1.440144722561829\\
  36.01 & 1.3898850929373556 & 1.3366376400883713 & 1.5273205888022294\\
  36.03702619690319 & 1.315765658136046 & 1.2677884572834808 & 1.4454364468477245\\
  36.064052393806385 & 1.2979581645914604 & 1.2520186343312811 & 1.4257282181520141\\
  36.06405239380639 & 1.2979581645914609 & 1.2520186343312822 & 1.4257282181520148\\
  36.09107859070958 & 1.300183039997525 & 1.2551331252483844 & 1.4281383299426458\\
  36.11810478761277 & 1.3026005236813172 & 1.2584321099574092 & 1.4307609931382297\\
  36.31 & 1.3198485452813526 & 1.2818225227121032 & 1.4493262349702796\\
  36.64 & 1.3497438067674599 & 1.3221803544285216 & 1.4812206797721812\\
  36.745 & 1.3594358836959266 & 1.3350362571298837 & 1.491346153107139\\
  36.98 & 1.3812891204872564 & 1.3638530299388258 & 1.5139819173579916\\
  37.33 & 1.4123333456108014 & 1.406781024538769 & 1.5475580184356106\\
  37.67 & 1.4435070304510424 & 1.4485666377584596 & 1.5800739790600902\\
  38.02 & 1.47563514470154 & 1.4915662131019916 & 1.6133763122909133\\
  38.37 & 1.5071973042173712 & 1.5344911797106622 & 1.6464706947428127\\
  38.73 & 1.5397138878175498 & 1.5786270338844341 & 1.680340374694506\\
  38.884 & 1.5537235521768848 & 1.5974413480793515 & 1.6947369381842503\\
  39.08 & 1.5716646489793473 & 1.6214184208156113 & 1.7130390796681183\\
  39.45 & 1.6045699759773662 & 1.6664568910198836 & 1.7473181108456886\\
  39.81 & 1.6368445807932281 & 1.7101592307165372 & 1.7804404168312757\\
  40.0 & 1.653893524187227 & 1.7331042052113643 & 1.7977850586619681\\
  40.18 & 1.6701383878381724 & 1.7548440995019126 & 1.8141803859315506\\
  40.55 & 1.703561684187478 & 1.79922264065834 & 1.8475734750967412\\
  40.93 & 1.7364837979408416 & 1.8445662521575608 & 1.8815651270589289\\
  41.148 & 1.756361096888629 & 1.8703865167882257 & 1.9008758768065386\\
  41.3 & 1.7702956529644966 & 1.8883825689650744 & 1.9143051344046942\\
  41.69 & 1.8035417322945397 & 1.9341256932133124 & 1.94838703896362\\
  42.07 & 1.8376774596159196 & 1.9783591402536802 & 1.9812363567961515\\
  42.46 & 1.8713120126459066 & 2.023306870360616 & 2.0145242403192034\\
  42.85 & 1.9058362295133404 & 2.067707991818182 & 2.0473323619836212\\
  43.25 & 1.9397945116814084 & 2.1127887558246967 & 2.080550481355495\\
  43.543 & 1.9647382840465029 & 2.1454328343121505 & 2.1045609210462537\\
  43.65 & 1.9738823281801858 & 2.157304274906068 & 2.113278550623783\\
  44.06 & 2.0081645568860407 & 2.202250793244862 & 2.1462678213467705\\
  44.46 & 2.0418808240794695 & 2.24554857105137 & 2.177975522859556\\
  44.87 & 2.076486776001725 & 2.289270251115802 & 2.2099402862095454\\
  45.29 & 2.1105267981518123 & 2.3332613551014028 & 2.2420705050005956\\
  45.71 & 2.1446315448191458 & 2.3765791536528935 & 2.2736540559644998\\
  46.078 & 2.1746747822587658 & 2.413917723890621 & 2.3008477819247255\\
  46.13 & 2.1789305519736017 & 2.4191269421430337 & 2.30464406279144\\
  46.56 & 2.2126637985626325 & 2.461797455029981 & 2.3357144193738137\\
  46.99 & 2.2472219588847424 & 2.503697021708634 & 2.3661892974516774\\
  47.42 & 2.2804539928695964 & 2.5447411248603213 & 2.396030148908198\\
  47.86 & 2.314510956008261 & 2.5857562985562734 & 2.42586575634425\\
  48.31 & 2.347937234073877 & 2.62681863221204 & 2.4557213496836803\\
  48.75 & 2.3814929802330784 & 2.6660211627217927 & 2.484234971570992\\
  48.761 & 2.3822963009876186 & 2.6669807333861564 & 2.484935390478273\\
  49.2 & 2.414353452061257 & 2.7050587658310707 & 2.512667710597855\\
  49.66 & 2.4473434336286184 & 2.7439985472035904 & 2.5410372116041438\\
  50.12 & 2.4803981459689948 & 2.7818908112818717 & 2.5686761581131767\\
  50.58 & 2.512757404676036 & 2.8186569499226897 & 2.5955559801645367\\
  51.05 & 2.544421225020205 & 2.855188841558905 & 2.6222951064259292\\
  51.52 & 2.5762145309571363 & 2.8906218228939555 & 2.648283116495449\\
  51.599 & 2.5813347755822864 & 2.8964281508224183 & 2.65256189651433\\
  51.64449241881862 & 2.5842810544215933 & 2.8997694076387237 & 2.6550208166306386\\
  51.68336931411397 & 2.586801223029032 & 2.902626845581103 & 2.657123253800103\\
  51.683369314113975 & 2.5868012230290347 & 2.9026268455811066 & 2.657123253800105\\
  51.722246209409306 & 2.5982074457304134 & 2.9138596432196566 & 2.6690357281279913\\
  51.72224620940931 & 2.598207445730591 & 2.9138596432198245 & 2.669035728128187\\
  51.76112310470465 & 3.5506301051886204 & 3.812040570329496 & 3.719956714282956\\
  51.76112310470466 & 3.550630105189296 & 3.812040570330133 & 3.719956714283701\\
  51.8 & 7.162055574583377 & 7.21644529367593 & 7.706776377720641\\
  51.83887689529535 & 3.558537362055503 & 3.820456748452437 & 3.7273174357503174\\
  51.877753790590695 & 2.6083100628718547 & 2.925261384124029 & 2.6774327911003013\\
  51.916630685886034 & 2.6018748109316197 & 2.9196197159368107 & 2.6696173255130526\\
  51.95550758118138 & 2.604379084075101 & 2.922403629681786 & 2.6716708637433886\\
  51.95550758118139 & 2.6043790840751018 & 2.9224036296817872 & 2.671670863743389\\
  52.0 & 2.6072477693091267 & 2.925591820572002 & 2.6740222125100153\\
  52.48 & 2.638281009712066 & 2.9594663943705877 & 2.699007295242512\\
  52.97 & 2.668618815681708 & 2.9928658694941053 & 2.7237208422286154\\
  53.46 & 2.6982611695650474 & 3.0250103308535095 & 2.7476189866454135\\
  53.95 & 2.7279034990525486 & 3.0560170941028004 & 2.7707467074828096\\
  54.45 & 2.7567208783746335 & 3.0864497772365205 & 2.7935464289581455\\
  54.603 & 2.7653643957281715 & 3.095474701853549 & 2.8003504186377723\\
  54.95 & 2.784842898788751 & 3.115606553435227 & 2.815529191827085\\
  55.46 & 2.8129001997396257 & 3.1441475098303444 & 2.8371485508350394\\
  55.98 & 2.8394371268424803 & 3.1719777154599442 & 2.858357277866999\\
  56.49 & 2.8659092587883794 & 3.1979866452974455 & 2.8783406494942496\\
  57.02 & 2.8923813998993797 & 3.223768367830644 & 2.898278061432585\\
  57.03825118302342 & 2.8932638731051887 & 3.2246367450931412 & 2.8989500070961842\\
  57.08118838726757 & 2.8953377363644477 & 3.2266765523413707 & 2.9005275474501544\\
  57.081188387267574 & 2.8953377363644477 & 3.226676552341372 & 2.9005275474501544\\
  57.12412559151171 & 2.898233872799194 & 3.2294836375806524 & 2.9030111954297073\\
  57.124125591511714 & 2.898233872799209 & 3.229483637580666 & 2.903011195429724\\
  57.167062795755854 & 2.9885724092413266 & 3.3146809256473633 & 3.0020392289350517\\
  57.21 & 3.326000757748234 & 3.6327693952400932 & 3.3738868056062903\\
  57.25293720424415 & 2.9929621124828567 & 3.3189124932271454 & 3.005446655690554\\
  57.252937204244155 & 2.992962112482843 & 3.318912493227132 & 3.0054466556905375\\
  57.295874408488295 & 2.9064824749021088 & 3.2374464621659347 & 2.9092399670137317\\
  57.338811612732435 & 2.907703137375619 & 3.2386401703557954 & 2.9098651609087725\\
  57.381748816976575 & 2.909750998019316 & 3.2406119996981717 & 2.911402539251711\\
  57.38174881697658 & 2.909750998019317 & 3.2406119996981713 & 2.9114025392517116\\
  57.54 & 2.917268377152138 & 3.247817740679351 & 2.9170240717503924\\
  57.782 & 2.928438593604481 & 3.2585615657230207 & 2.925474277339764\\
  58.08 & 2.942025916026273 & 3.2714548627292825 & 2.9356476391303428\\
  58.61 & 2.966023288080562 & 3.293421642903743 & 2.953107595711561\\
  59.16 & 2.9891309757741813 & 3.314924491067168 & 2.9703813067083336\\
  59.7 & 3.011413685723719 & 3.3347453613022147 & 2.986525245376185\\
  60.0 & 3.022833869627813 & 3.345243660196204 & 2.995141985424619\\
  60.26 & 3.0325476870281256 & 3.3540230486610922 & 3.0024181908561878\\
  60.81 & 3.054199706932453 & 3.3717011542353825 & 3.017203177092459\\
  61.145 & 3.0657566973574717 & 3.381859530171892 & 3.025822794086201\\
  61.38 & 3.073683847266279 & 3.3887171523341366 & 3.031700198777989\\
  61.94 & 3.0931680153903964 & 3.404196410674762 & 3.045114297322599\\
  62.52 & 3.111892012904835 & 3.418955096191708 & 3.0581646162829497\\
  62.98035880495699 & 3.1251136801543664 & 3.4297654260639936 & 3.0679399964541063\\
  62.980358804957 & 3.1251136801543673 & 3.429765426063994 & 3.067939996454107\\
  63.027769103717745 & 3.126440064218981 & 3.4308347336578056 & 3.0689227035100575\\
  63.02776910371775 & 3.1264400642189814 & 3.4308347336578056 & 3.0689227035100575\\
  63.0751794024785 & 3.127796220946889 & 3.4319299125077123 & 3.0699381343101115\\
  63.1 & 3.130520087464073 & 3.4344005632057186 & 3.072693278989121\\
  63.12258970123925 & 3.1330631922641667 & 3.4366497582092355 & 3.0752020789725125\\
  63.17 & 3.149284682635417 & 3.4516271333163164 & 3.0924845660285283\\
  63.21741029876075 & 3.1359460592793393 & 3.438740262290685 & 3.077128088280058\\
  63.2648205975215 & 3.133469570380644 & 3.4360888401599152 & 3.073764294732251\\
  63.264820597521506 & 3.1334695703806448 & 3.436088840159916 & 3.0737642947322508\\
  63.31223089628226 & 3.1348527562570667 & 3.437072745534996 & 3.074661519163616\\
  63.359641195043004 & 3.1362662633188094 & 3.438082768536826 & 3.075592297643434\\
  63.68 & 3.1456516469478855 & 3.444707504499125 & 3.0818133768108082\\
  64.27 & 3.161447482655869 & 3.4559440844549285 & 3.092590534908159\\
  64.705 & 3.1731915567366737 & 3.4634544931120463 & 3.1000256958283408\\
  64.86 & 3.177243322957474 & 3.465986678278511 & 3.102594316812332\\
  65.46 & 3.1908712988262224 & 3.4749857798399857 & 3.111935751312321\\
  66.07 & 3.203739088294088 & 3.48291777950637 & 3.120601975854359\\
  66.68 & 3.2158466750371124 & 3.4896999886067643 & 3.1285094237810944\\
  67.3 & 3.2265465097609107 & 3.4953998285995023 & 3.1357118619982747\\
  67.92 & 3.2378938897186496 & 3.4999420078514665 & 3.1421068533070105\\
  68.472 & 3.24544245935847 & 3.503091150110064 & 3.147193700651981\\
  68.55 & 3.2464257784460666 & 3.503474570121389 & 3.147872288486548\\
  69.18 & 3.2556052892601226 & 3.5058733666657873 & 3.1528258688165636\\
  69.82 & 3.2626168658712644 & 3.5071980750330938 & 3.157060403487827\\
  70.47 & 3.2689808759870447 & 3.5075323120106687 & 3.160655841849954\\
  71.12 & 3.2752322484970176 & 3.506773020632842 & 3.1634454522341873\\
  71.78 & 3.2794283047892643 & 3.5049402413509116 & 3.16549263039284\\
  72.44 & 3.28351172290785 & 3.502194310519959 & 3.166876975706858\\
  72.458 & 3.2836040917549267 & 3.5021065942435476 & 3.1669052329146568\\
  73.11 & 3.286187464678366 & 3.4983740523196847 & 3.1674964292037653\\
  73.79 & 3.2874554588151024 & 3.4934890362393562 & 3.1673521855970783\\
  74.47 & 3.288610816621775 & 3.487778335418922 & 3.1665801097035513\\
  75.16 & 3.2877108594148305 & 3.4810083577933035 & 3.165026309277546\\
  75.86 & 3.286810899456723 & 3.4731979632626624 & 3.162697598105061\\
  76.56 & 3.2843905535991014 & 3.4646521894726625 & 3.1597772174794376\\
  76.676 & 3.2840115021726324 & 3.463147823143745 & 3.159220967015762\\
  77.27 & 3.2813226983171497 & 3.455073421785218 & 3.1560651998524247\\
  77.98 & 3.277494654729431 & 3.444637181602952 & 3.1516372173406118\\
  78.7 & 3.272258861475689 & 3.4334277723315934 & 3.1466076203477416\\
  79.43 & 3.26626288229605 & 3.421221326195262 & 3.1407833151164244\\
  80.0 & 3.2618132549300385 & 3.4111881750411697 & 3.1357921565621774\\
  80.17 & 3.2602668988553507 & 3.4080452840230553 & 3.1341756020536873\\
  80.91 & 3.251455395140615 & 3.394333933538386 & 3.1270674373906093\\
  81.14 & 3.249159901765652 & 3.389883946104681 & 3.1246920042499844\\
  81.66 & 3.2432914957084913 & 3.3796700886488096 & 3.119168501031777\\
  82.41 & 3.2337198518153563 & 3.364290487855638 & 3.1106079606704675\\
  83.18 & 3.2235006563585364 & 3.348072275920242 & 3.1013720215158775\\
  83.95 & 3.2125212613789356 & 3.33115329400932 & 3.0914671153763664\\
  84.72 & 3.200781666918236 & 3.3135953863369583 & 3.080936191536145\\
  85.51 & 3.1883945190334844 & 3.295256570389305 & 3.0697404285085432\\
  85.863 & 3.1824925826285027 & 3.286747714181738 & 3.0644461516152264\\
  86.3 & 3.1745996372213354 & 3.276296042748575 & 3.057915233153818\\
  87.1 & 3.160044594963329 & 3.256525750881487 & 3.0453445727566537\\
  87.9 & 3.1454895385219506 & 3.236526403864775 & 3.032438970543451\\
  88.06482655124033 & 3.1425867625643353 & 3.2323362438970085 & 3.0297060246386267\\
  88.06482655124034 & 3.1425867625643353 & 3.232336243897007 & 3.0297060246386263\\
  88.13111991343024 & 3.1414017724213488 & 3.2306297853424204 & 3.0285911350967063\\
  88.19741327562018 & 3.158077531667425 & 3.2457551536973037 & 3.0471990163378684\\
  88.19741327562019 & 3.158077531667843 & 3.245755153697698 & 3.04719901633833\\
  88.26370663781009 & 5.067414849004426 & 5.044792328478824 & 5.155564261858417\\
  88.2637066378101 & 5.067414849006017 & 5.044792328480325 & 5.155564261860173\\
  88.33 & 12.324812572170227 & 11.88466371788531 & 13.16896390741692\\
  88.39629336218991 & 5.0707281648511575 & 5.046901527872379 & 5.15976776856597\\
  88.46258672437983 & 3.1532157615204532 & 3.2390844598310786 & 3.0428739217442264\\
  88.52888008656976 & 3.133947479535505 & 3.220441359070052 & 3.02190164652343\\
  88.59517344875967 & 3.1326474291896305 & 3.2187317416000685 & 3.02077112289283\\
  88.72 & 3.130174309765373 & 3.2154825068190425 & 3.0186210722077\\
  89.54 & 3.1135639374840536 & 3.1939407334913046 & 3.004245248421198\\
  90.36 & 3.09760111482806 & 3.1722692453232986 & 2.9895968951972445\\
  90.862 & 3.087488358121514 & 3.158704593748059 & 2.9803118715248864\\
  91.2 & 3.0802305737753874 & 3.149605377210562 & 2.974050302362143\\
  92.04 & 3.062099863980153 & 3.1265036460705464 & 2.9579796348115877\\
  92.9 & 3.0433216018698612 & 3.1028327674510052 & 2.9413238115869103\\
  93.76 & 3.023895761338858 & 3.078758609524992 & 2.9241620383148206\\
  94.62 & 3.0043572869265587 & 3.054323295855479 & 2.9065274500253535\\
  95.5 & 2.9834110745100895 & 3.0293922159135653 & 2.888347166474684\\
  96.151 & 2.967657547358089 & 3.0107214253749026 & 2.8745934598142133\\
  96.38 & 2.961817294548396 & 3.0041356256416107 & 2.86971603194849\\
  97.27 & 2.940223545828825 & 2.9782916854572985 & 2.8504401436693105\\
  98.17 & 2.9186297963322265 & 2.9523126456637714 & 2.8308761436006606\\
  99.08 & 2.8956282970690532 & 2.9257916992266946 & 2.8106956884785985\\
  100.0 & 2.871899794777506 & 2.8987698311505166 & 2.7899388972397112\\
  100.9 & 2.8482509290236755 & 2.872533047129863 & 2.7695933841774107\\
  100.92621909870483 & 2.8476442740689585 & 2.871773478381206 & 2.769001789232992\\
  101.749 & 2.827695892129468 & 2.8476431294271185 & 2.750120584421581\\
  101.86101701559753 & 2.824842713457005 & 2.8443348204180916 & 2.74751958394604\\
  101.9 & 2.8238420150727066 & 2.8431752286437812 & 2.746607038504022\\
  102.8 & 2.7994329746604305 & 2.8166045621858706 & 2.7256099554974225\\
  102.80447320933098 & 2.7993293665208783 & 2.816468804626932 & 2.725502140791563\\
  103.75666787451848 & 2.7761339722055887 & 2.7886576988232568 & 2.70334241415636\\
  103.8 & 2.775024067183075 & 2.78739707160732 & 2.7023335187656934\\
  104.7 & 2.749967437146378 & 2.760982496646556 & 2.6811011049651086\\
  104.71768194855203 & 2.7495454947023554 & 2.760458725305474 & 2.6806783199905833\\
  105.68759711848051 & 2.7252366765116576 & 2.7318864942637284 & 2.65752041471617\\
  105.7 & 2.724910937215508 & 2.731535230220183 & 2.657234729858096\\
  106.66649582795388 & 2.700732666573163 & 2.7034307141014646 & 2.634273809713007\\
  106.7 & 2.6998544228359616 & 2.702462137530662 & 2.6334793176483586\\
  107.6 & 2.6740375707372315 & 2.6762375305470094 & 2.611885965526453\\
  107.65446128423159 & 2.6726972094743995 & 2.674639475447456 & 2.610565064932225\\
  107.672 & 2.672264107379238 & 2.674123273868937 & 2.6101382586823303\\
  108.6 & 2.6483334976620805 & 2.6470677538336087 & 2.587688730381337\\
  108.65157746525372 & 2.647024621951013 & 2.645527011319336 & 2.586405345870602\\
  109.6 & 2.621869229920112 & 2.618236917519213 & 2.563593527536167\\
  109.65792912678099 & 2.6205799703630284 & 2.616588162289224 & 2.5622102658805193\\
  110.67360180959746 & 2.596812519983463 & 2.5873639459917754 & 2.537596215118048\\
  110.7 & 2.59616527206062 & 2.5865973166442573 & 2.536948119937409\\
  111.69868184678226 & 2.5704964810018067 & 2.5578680453880027 & 2.512574706728836\\
  111.7 & 2.5704611615350084 & 2.557831654597138 & 2.512543725785041\\
  112.7 & 2.5433492899327876 & 2.5295298714674117 & 2.4883687534559265\\
  112.73325637104871 & 2.5426077213449116 & 2.528598412494089 & 2.4875703473843065\\
  113.77741332214902 & 2.5181975933790905 & 2.4990909565114636 & 2.4621905945429154\\
  113.8 & 2.5176452889213228 & 2.4984474132905565 & 2.4616352087313866\\
  113.94 & 2.514080561884231 & 2.4944339378971234 & 2.458169924454985\\
  114.8 & 2.491293600981909 & 2.470259832505532 & 2.437229683139579\\
  114.83124145435112 & 2.490616868504689 & 2.4693588119020036 & 2.436447240307095\\
  115.89483034398118 & 2.4664724216912224 & 2.439900943972517 & 2.410772107363456\\
  115.9 & 2.466349789572953 & 2.4397590905452398 & 2.410648062245558\\
  116.9 & 2.439998082202881 & 2.4121435904015747 & 2.3864306323443087\\
  116.96827039703847 & 2.438474706224246 & 2.4102501029006356 & 2.3847651016753186\\
  118.0 & 2.414406680549163 & 2.3818705251610637 & 2.359722579989104\\
  118.05165285688055 & 2.413253873380714 & 2.3804187351318524 & 2.3584380536522196\\
  119.1 & 2.3888152655178017 & 2.35210723989937 & 2.3332992373942543\\
  119.14506981197748 & 2.3878087765371787 & 2.3509050092472776 & 2.332228398979511\\
  120.0 & 2.368036705701721 & 2.3279049795922435 & 2.311696699951885\\
  120.2 & 2.3632238350713863 & 2.3225525494809585 & 2.3069051463098726\\
  120.24861420374123 & 2.3621982704019735 & 2.3212402926017326 & 2.3057298276818607\\
  120.573 & 2.35525305896661 & 2.3124527199032037 & 2.2978524216680767\\
  121.3 & 2.339040148782856 & 2.2931386107321523 & 2.2804868823537845\\
  121.33464724652947 & 2.3383557861103164 & 2.2921940395990292 & 2.279636421960174\\
  121.36237983442417 & 2.337806618665048 & 2.2914363961311937 & 2.278954189695336\\
  121.4259854348971 & 2.3365424204118437 & 2.289803046856629 & 2.277481412834328\\
  121.42598543489711 & 2.3365424204118437 & 2.2898030468566284 & 2.2774814128343275\\
  121.51732362326473 & 2.334737436854125 & 2.2874654875461915 & 2.275378582779528\\
  121.60866181163236 & 2.3352260869334 & 2.2872875652156672 & 2.2758089316735965\\
  121.7 & 2.342220276622244 & 2.2932391788637463 & 2.2834229766322043\\
  121.79133818836763 & 2.3315123959992867 & 2.282503617718721 & 2.271492231372263\\
  121.79133818836765 & 2.3315123959992854 & 2.28250361771872 & 2.271492231372262\\
  121.88267637673526 & 2.3272960151418935 & 2.277884354191844 & 2.2667296826235277\\
  121.88267637673528 & 2.3272960151418935 & 2.277884354191844 & 2.2667296826235277\\
  121.9740145651029 & 2.325380000392842 & 2.2754310628737424 & 2.2645077510665526\\
  122.06535275347053 & 2.323472390074124 & 2.2729834692089663 & 2.262295801053031\\
  122.48646137509307 & 2.3145022091632663 & 2.261988887969871 & 2.252342790268411\\
  122.5 & 2.314209024716114 & 2.2616378938759287 & 2.2520246687624663\\
  123.6 & 2.289377758255 & 2.2329779109085264 & 2.225984087059327\\
  123.62095437367691 & 2.288937165801552 & 2.232429487404717 & 2.225484539360818\\
  124.7 & 2.2653066643785538 & 2.204510361146805 & 2.1999846774009173\\
  124.76595526308684 & 2.2640746230614526 & 2.202769283845771 & 2.198391124801283\\
  125.9 & 2.2418832491455016 & 2.174039145735583 & 2.1720029760615622\\
  125.9215613694151 & 2.241494203211327 & 2.173499645188789 & 2.1715060844825347\\
  127.08787092020596 & 2.219459430696998 & 2.144154263236583 & 2.144414988505632\\
  127.1 & 2.2192200044896886 & 2.1438475661217304 & 2.144131193897688\\
  127.592 & 2.209301366255013 & 2.1315515612156246 & 2.1327388828038303\\
  128.2 & 2.1965566352831343 & 2.116397331794881 & 2.118666298412422\\
  128.26498305280597 & 2.19542046238812 & 2.1147435212294035 & 2.1171293007701104\\
  129.4 & 2.1746535749911855 & 2.087028809539482 & 2.091285884911917\\
  129.4529978227916 & 2.1737595332815824 & 2.0857531207546067 & 2.090093194125313\\
  130.6 & 2.1535106865014617 & 2.057982787463109 & 2.064075721973044\\
  130.652016212472 & 2.152600073722537 & 2.056720184878696 & 2.0628902754552225\\
  131.8 & 2.1316076014271452 & 2.02917406276614 & 2.0369643133322914\\
  131.86214013947486 & 2.1305571262609275 & 2.0276543491477343 & 2.0355316584086975\\
  133.0 & 2.110464688395028 & 2.000961163122442 & 2.0102874535884623\\
  133.0834724654076 & 2.1091266635903057 & 1.999034338710427 & 2.0084606327008316\\
  134.3 & 2.088674319593543 & 1.9707775946261268 & 1.981617648268549\\
  134.31611700460155 & 2.0883817783981877 & 1.9704020844150958 & 1.981260235818409\\
  135.02 & 2.0752915417993782 & 1.9542505776318737 & 1.9658632205312352\\
  135.5 & 2.06601102154988 & 1.9431764116284913 & 1.9552880982237522\\
  135.5601785329369 & 2.064946850630065 & 1.941766527628732 & 1.9539412190515346\\
  136.8 & 2.0420527167783473 & 1.9139470653811292 & 1.927279597269806\\
  136.81576279674707 & 2.0417214346711297 & 1.9135981824194979 & 1.9269444699383838\\
  138.0 & 2.0159263467344375 & 1.8872898557136184 & 1.9016320227826653\\
  138.08297652180923 & 2.0141428704378623 & 1.8854450795128308 & 1.8998538525555122\\
  139.3 & 1.9869845871627834 & 1.858701122787877 & 1.8740198292246748\\
  139.36192742241437 & 1.985551880542488 & 1.8573153754134704 & 1.8726795782744536\\
  140.0 & 1.9705036926888424 & 1.8436726714814875 & 1.859454382096889\\
  140.6 & 1.9558748798259733 & 1.8307828018226477 & 1.8469403370500002\\
  140.65272421052364 & 1.9545681429757726 & 1.8296703830819911 & 1.8458588236588478\\
  141.9 & 1.9225972245023235 & 1.80324214473236 & 1.8201252827100969\\
  141.95547660501015 & 1.9211622053498767 & 1.8020653122580643 & 1.8189775148663927\\
  142.88 & 1.8966556095967868 & 1.7827560165283038 & 1.8001136364740364\\
  143.2 & 1.8879118129991068 & 1.7760057581456303 & 1.7935109696790152\\
  143.27029534098293 & 1.8859823859200868 & 1.774507654622447 & 1.7920453966246292\\
  144.5 & 1.8511710914219246 & 1.749399946198156 & 1.767413043379823\\
  144.59729217920196 & 1.8487407037675823 & 1.7474485332972987 & 1.7654945633959531\\
  145.06319781733802 & 1.8369415289866753 & 1.7379647770050652 & 1.7561690646484567\\
  145.1723983630035 & 1.8341374405129827 & 1.7357085995215393 & 1.7539501136228228\\
  145.28159890866903 & 1.831326917251074 & 1.7334687419268502 & 1.7517478958484154\\
  145.28159890866905 & 1.8313269172510733 & 1.7334687419268502 & 1.7517478958484154\\
  145.3907994543345 & 1.8293751271226877 & 1.7321615631524585 & 1.7506139705028225\\
  145.5 & 1.8298766555873145 & 1.7331683174694807 & 1.752192827062191\\
  145.6092005456655 & 1.8236666624031017 & 1.7278507525611477 & 1.7463652426359046\\
  145.71840109133097 & 1.819904648323067 & 1.7248420915770935 & 1.7432445542581518\\
  145.8276016369965 & 1.8170038680294478 & 1.7226467609249916 & 1.74107878453492\\
  145.9 & 1.8150780389869563 & 1.7211896593855092 & 1.7396421875833632\\
  145.93657991557578 & 1.814057911731342 & 1.7204513776791706 & 1.7389142711754486\\
  145.93680218266198 & 1.814051708011738 & 1.720446887482922 & 1.7389098439716493\\
  147.2 & 1.77777137776332 & 1.6953097265190624 & 1.7140801997742456\\
  147.28827239075017 & 1.775586821830467 & 1.693522990629322 & 1.7123137070526102\\
  148.6 & 1.7420499447228313 & 1.6681040987407059 & 1.687112584666423\\
  148.6524844997857 & 1.740728052020541 & 1.6671035061424517 & 1.6861186821470038\\
  150.0 & 1.7056978274965384 & 1.6413271744140054 & 1.6604823357426228\\
  150.02933220192168 & 1.7049928975041055 & 1.6407654816576553 & 1.6599229613829853\\
  151.198 & 1.6761364318467633 & 1.6187406793026693 & 1.6379536374938806\\
  151.4 & 1.670995581546783 & 1.6148789337184386 & 1.634098418277913\\
  151.4189325304352 & 1.6705429686143285 & 1.6145150482505373 & 1.6337351361560917\\
  152.8 & 1.6364876079038115 & 1.589167524434709 & 1.6083615614009643\\
  152.82140360258708 & 1.6359898932332428 & 1.5887807366727047 & 1.6079737089835566\\
  154.2 & 1.6029340760943112 & 1.563812983356591 & 1.5829093739487126\\
  154.23686462966273 & 1.602100697480855 & 1.5631449623127203 & 1.5822379794515422\\
  155.6 & 1.5703349862509393 & 1.538801429459506 & 1.5577327759325972\\
  155.66543592710622 & 1.5688598454908558 & 1.5376132182263558 & 1.5565359300131218\\
  157.0 & 1.537865397804782 & 1.5144296108421595 & 1.5331264175949315\\
  157.10723892474488 & 1.5356838803643813 & 1.512601813074055 & 1.5312776931388716\\
  157.12687268737096 & 1.53528336774614 & 1.5122661726676634 & 1.5309382095533126\\
  157.2451545155282 & 1.532863341934496 & 1.5102376894420846 & 1.5288865134536265\\
  157.3634363436855 & 1.5306923877165932 & 1.508444505185907 & 1.5271122517875062\\
  157.48171817184274 & 1.5562053724791753 & 1.5327451568432915 & 1.555907245284834\\
  157.6 & 1.6599668328093442 & 1.6307988842732681 & 1.6711016092459805\\
  157.71828182815725 & 1.5513622905942226 & 1.528689107299026 & 1.55181751286103\\
  157.8365636563145 & 1.5208380769699523 & 1.5001777386851487 & 1.5187508802164322\\
  157.9548454844718 & 1.5180794316491808 & 1.4979654354359744 & 1.516469486391268\\
  158.07312731262905 & 1.5155713361514225 & 1.4959902234287896 & 1.514467565127204\\
  158.5 & 1.5064151165238415 & 1.4887709740560624 & 1.5071508058397016\\
  158.56239617711373 & 1.5051514980324892 & 1.4877037509066764 & 1.506069175492853\\
  160.0 & 1.4750943352323502 & 1.4634561386527472 & 1.4814581931007313\\
  160.03103137387018 & 1.474439883605701 & 1.4629238994746996 & 1.4809177181082338\\
  161.4 & 1.4447278856436283 & 1.4404865662256452 & 1.4580802357749465\\
  161.51326935030895 & 1.4425655782047446 & 1.4386659430285018 & 1.4562242543899833\\
  162.9 & 1.4152512287142684 & 1.4162931388171502 & 1.4333986466818658\\
  163.0092360979741 & 1.4131787144502845 & 1.4145339624666295 & 1.4316021227618372\\
  164.4 & 1.3859688293097006 & 1.3924520622186618 & 1.4090219530002461\\
  164.5190587753661 & 1.3839156707858309 & 1.3905322886948706 & 1.4070580846267973\\
  165.959 & 1.358264142477074 & 1.3683213121273794 & 1.3842866186458338\\
  166.0 & 1.3575114628771505 & 1.367701145031536 & 1.3836499119931895\\
  166.04286571875295 & 1.3567268944316402 & 1.3670515704240056 & 1.3829830222253618\\
  167.5 & 1.3292482355622255 & 1.344932171992382 & 1.3602578609902327\\
  167.58078645307688 & 1.3278147267424747 & 1.3437074918953407 & 1.3589986029727392\\
  169.0 & 1.301874694077822 & 1.3225188512124906 & 1.3371859172207239\\
  169.1329517029647 & 1.2996759766213417 & 1.3205038350542324 & 1.3351109581283633\\
  169.824 & 1.2880580000896868 & 1.3105185865300157 & 1.3248099419380597\\
  170.6 & 1.2746307715338245 & 1.299232853473765 & 1.3131621063769352\\
  170.6994934038408 & 1.2729933411222552 & 1.2978180239440735 & 1.3117003214546774\\
  172.2 & 1.24751636630272 & 1.2764242266590808 & 1.2895835109633182\\
  172.28054471313922 & 1.2462312426446192 & 1.2752776684541407 & 1.2883973670863582\\
  173.78 & 1.2215654435573389 & 1.2542560051101244 & 1.2666266301948488\\
  173.8 & 1.221226888719091 & 1.2539717463152984 & 1.2663321878199594\\
  173.87624002162505 & 1.2200509193197686 & 1.2528860443844458 & 1.2652076153593177\\
  175.4 & 1.1958157997763847 & 1.232163945557148 & 1.2437019373078797\\
  175.4867149648152 & 1.1944806185005743 & 1.2310070852716626 & 1.242499965588319\\
  177.0 & 1.170469455136789 & 1.2107756613522942 & 1.221469781703125\\
  177.1121064345087 & 1.168771341040403 & 1.209280668158671 & 1.2199148113292098\\
  177.828 & 1.1577592803643688 & 1.1998409420468303 & 1.210090691882295\\
  178.6 & 1.145556699032507 & 1.189741941987124 & 1.1995731298690298\\
  178.75255259042356 & 1.1434226980174849 & 1.1877096436892167 & 1.1974571310902693\\
  180.3 & 1.1210776306435197 & 1.1679953508510563 & 1.1768945947131106\\
  180.40819287193807 & 1.1195827576283368 & 1.1666444195501258 & 1.1754840804915712\\
  181.97 & 1.097331156509757 & 1.1470997975777442 & 1.1550700896881962\\
  182.0 & 1.0968913599314825 & 1.1467259384098158 & 1.1546793960439916\\
  182.07916800994624 & 1.0958207144933712 & 1.1457372744824743 & 1.1536462488373722\\
  183.7 & 1.0732146488213563 & 1.1258096509191902 & 1.132804595278979\\
  183.76562003881722 & 1.0723404383768256 & 1.1249905694881523 & 1.1319479763406135\\
  185.4 & 1.0498954928904756 & 1.1055320049246464 & 1.1115634956278524\\
  185.46769230846976 & 1.0490100438657444 & 1.1047412196612771 & 1.1107343573065602\\
  186.209 & 1.0391735280557661 & 1.0959475220456918 & 1.1015166630869566\\
  187.1 & 1.0270099250732325 & 1.0856519852836706 & 1.0907136918834572\\
  187.18552949655793 & 1.025908377408941 & 1.08465407829542 & 1.0896666984600292\\
  188.8 & 1.0044931876136203 & 1.066120243071118 & 1.0702071508735045\\
  188.91927762076642 & 1.0029798773974477 & 1.0647311236340555 & 1.0687488104887521\\
  190.5 & 0.9823340055487041 & 1.047136031689305 & 1.0502498061374697\\
  190.546 & 0.9817937219464742 & 1.0466365033303713 & 1.0497241474416288\\
  190.66908405122518 & 0.9803438165272927 & 1.0452957298544605 & 1.048313328124586\\
  192.3 & 0.9605437026661922 & 1.0274946287557178 & 1.0295793591799585\\
  192.43509752303325 & 0.9589798812186274 & 1.0260253084659012 & 1.0280325712290757\\
  194.1 & 0.93911095328976 & 1.0081973915947908 & 1.0092535570083625\\
  194.21746814890244 & 0.9377785829037235 & 1.0069215066194788 & 1.0079098691373385\\
  194.984 & 0.9289541925309939 & 0.9990002095376473 & 0.9995560990076983\\
  195.9 & 0.9181117898583923 & 0.9894758356015939 & 0.9895121076393266\\
  196.01634743191858 & 0.9168099764895101 & 0.9882943459940956 & 0.9882652938464529\\
  197.7 & 0.897405437066142 & 0.9711703692630022 & 0.970193336592743\\
  197.83188827841622 & 0.8959597393313563 & 0.9698338387756056 & 0.9687825346048135\\
  199.5 & 0.8771326572507394 & 0.9532013302735367 & 0.9512171028260479\\
  199.526 & 0.8768673399267976 & 0.9529391633749255 & 0.9509402893091586\\
  199.66424501097933 & 0.875452803096201 & 0.9515412744226669 & 0.9494643995452718\\
  201.4 & 0.8571414726103378 & 0.9347869640066355 & 0.9317536659062942\\
  201.51357338155586 & 0.8559358363504833 & 0.9337133682499332 & 0.9306181479420881\\
  203.2 & 0.8375190170176399 & 0.9177488481964976 & 0.9137332573907346\\
  203.38003058469798 & 0.835742718183928 & 0.9160527146290899 & 0.9119391116640254\\
  204.174 & 0.8277865729855587 & 0.9086482583570549 & 0.904104894280881\\
  204.78337341361672 & 0.8215443983045618 & 0.9030527560522308 & 0.8981824293705278\\
  204.93753006021254 & 0.8199465192657921 & 0.9016190046501497 & 0.8966653890986416\\
  204.93753006021257 & 0.8199465192657918 & 0.9016190046501495 & 0.896665389098641\\
  205.09168670680833 & 0.8183565220709474 & 0.9001924622708154 & 0.8951578259343197\\
  205.09168670680836 & 0.8183565220709474 & 0.9001924622708155 & 0.8951578259343199\\
  205.1 & 0.8183588399307853 & 0.9001985287647479 & 0.8951737817460568\\
  205.24584335340415 & 0.8185133308502078 & 0.9003036725994032 & 0.8954526868970799\\
  205.2458433534042 & 0.8185133308502088 & 0.9003036725994041 & 0.8954526868970811\\
  205.26377527092524 & 0.8190697259760373 & 0.9008230879175532 & 0.8960803647224774\\
  205.4 & 0.8233016614383512 & 0.9048555207233371 & 0.9009391812409728\\
  205.55415664659583 & 0.8155136469385794 & 0.897564111691276 & 0.8925514721612493\\
  205.70831329319165 & 0.8123406344588058 & 0.8946222514646883 & 0.8892600132987846\\
  205.86246993978747 & 0.8108045132896677 & 0.8932229427826831 & 0.8877765669162665\\
  206.0166265863833 & 0.8092766766540143 & 0.891831153584293 & 0.8863029308080753\\
  206.01662658638332 & 0.8092766766538975 & 0.8918311535841829 & 0.8863029308079463\\
  207.0 & 0.7993583606642332 & 0.8829684213719055 & 0.8769189538881255\\
  207.1649675602067 & 0.7977847382936084 & 0.8815200248448969 & 0.875384461222256\\
  208.9 & 0.780744029629149 & 0.8662554098907714 & 0.8592145753927803\\
  208.93 & 0.7804795199768959 & 0.8659934369935486 & 0.8589370383474328\\
  209.08376905557498 & 0.7791198490425748 & 0.8646466245388518 & 0.8575103250153084\\
  210.9 & 0.762563336601287 & 0.8489924434264833 & 0.8409229906196174\\
  211.02034285685966 & 0.7614601007288136 & 0.8479408607822354 & 0.839809199553369\\
  212.8 & 0.7446753553821845 & 0.8330988126764785 & 0.8240743139376803\\
  212.97485357455187 & 0.7431776840270428 & 0.8316736464499626 & 0.82256284164805\\
  213.796 & 0.7360379923500083 & 0.8248728428553227 & 0.8153534206041089\\
  214.8 & 0.7270690130711056 & 0.8167711338078887 & 0.8067612363638423\\
  214.94746734379805 & 0.7258324173542962 & 0.8155722483703779 & 0.8054901181404202\\
  216.8 & 0.7098315012398279 & 0.8007584236975482 & 0.7897810132544886\\
  216.93835183851823 & 0.7086951318849619 & 0.7996371341115864 & 0.7885925458406733\\
  218.776 & 0.6931598979357606 & 0.7854243467702612 & 0.7735160766669931\\
  218.8 & 0.6929515464585502 & 0.7852433487108795 & 0.773324014966373\\
  218.94767628566208 & 0.6917581651588115 & 0.7841266506507371 & 0.7721391544977182\\
  220.8 & 0.6763531053944353 & 0.7701030140945804 & 0.7572636612539085\\
  220.97561147959033 & 0.6749644747640113 & 0.7687800852935883 & 0.7558605879284922\\
  222.8 & 0.6601234841684362 & 0.7552654198840694 & 0.7415259568123753\\
  223.02232979659362 & 0.6584795717829268 & 0.7535977219644331 & 0.7397580389601821\\
  223.872 & 0.652100176643532 & 0.7475334453156083 & 0.7333236426768599\\
  224.9 & 0.644175486949383 & 0.7401417646627522 & 0.7254842981418442\\
  225.0880052095462 & 0.6428110175649145 & 0.7388256934741634 & 0.7240880062747336\\
  227.0 & 0.6285202898862284 & 0.7254206653848398 & 0.7098711644818114\\
  227.17281330269074 & 0.6272945490859341 & 0.7242151185306305 & 0.7085929179226009\\
  229.087 & 0.6133200607133726 & 0.7110855160493347 & 0.6946717475152124\\
  229.1 & 0.6132226502915383 & 0.7109954384084402 & 0.6945762902304229\\
  229.2769312865649 & 0.6119911792147521 & 0.7097660866286779 & 0.6932736334593389\\
  231.2 & 0.5982178308131564 & 0.697011518742778 & 0.6797512585699849\\
  231.40053801306541 & 0.5968472844965086 & 0.6957128165581308 & 0.6783742778384975\\
  233.3 & 0.5834945504899378 & 0.6833896584940256 & 0.6653141252465641\\
  233.5438139906477 & 0.5819522570849427 & 0.6818179892865297 & 0.6636489580675774\\
  234.423 & 0.5763054025492645 & 0.6762023973637318 & 0.65769958917539\\
  235.5 & 0.5692049177366697 & 0.669410545935712 & 0.6505051772529913\\
  235.70694139967276 & 0.5679087874556185 & 0.6680815218857407 & 0.649098230844306\\
  237.7 & 0.5550560363450804 & 0.6558641895462409 & 0.6361593713045492\\
  237.89010410788958 & 0.5539017869390114 & 0.6547260350173121 & 0.6349540441744866\\
  239.883 & 0.5414497268413642 & 0.6427799256616328 & 0.622309323969637\\
  239.9 & 0.541340730776886 & 0.6426788873364313 & 0.6222024088902384\\
  240.09348768606517 & 0.5401596227866151 & 0.6415255371448455 & 0.6209821002590085\\
  242.1 & 0.5275606763462269 & 0.6297686586717555 & 0.6085451084043474\\
  242.31727942376008 & 0.5262605682213521 & 0.6284798048749288 & 0.6071826959926239\\
  244.3 & 0.5140621609835082 & 0.6172454523788762 & 0.5953038611300078\\
  244.56166834524439 & 0.5125896081308796 & 0.6158002451524783 & 0.5937758994682765\\
  245.471 & 0.5073956413078294 & 0.610696686731126 & 0.5883831769685259\\
  246.6 & 0.5007804976832472 & 0.6045195204504858 & 0.5818564727675327\\
  246.82684522556923 & 0.4995247861788771 & 0.6032718295462624 & 0.5805387540063385\\
  248.9 & 0.4877156047972655 & 0.5920602737146685 & 0.5687014859322979\\
  249.1130026067791 & 0.4865360629544829 & 0.5908941748309815 & 0.5674712803425351\\
  251.189 & 0.47471491415837264 & 0.5800470912431631 & 0.5560259871987104\\
  251.2 & 0.47465070095478346 & 0.5799911846247904 & 0.5559670034684836\\
  251.42033481427967 & 0.47342978292970705 & 0.5788678967533353 & 0.5547820271429506\\
  253.5 & 0.4615857849380713 & 0.5682515294404129 & 0.5435898602730075\\
  253.74903797335716 & 0.4603018308752512 & 0.5669886080978254 & 0.5422591566657844\\
  255.9 & 0.4488897660465753 & 0.5562620413796384 & 0.5309613918435243\\
  256.0993100258457 & 0.4478454220423222 & 0.555255821100692 & 0.5299024850666068\\
  257.04 & 0.4428503457773681 & 0.5507453752376769 & 0.5251536376487004\\
  258.2 & 0.43653997245585124 & 0.5451339185548837 & 0.5192499512818115\\
  258.4713507469564 & 0.4352029748643151 & 0.5438597231348106 & 0.5179093496565844\\
  260.6000000000001 & 0.424418308597835 & 0.5338459364675615 & 0.5073813456228762\\
  260.8653617622551 & 0.4231396132599622 & 0.5326062040245826 & 0.5060787427903568\\
  263.0 & 0.41256692140026796 & 0.5228027070747695 & 0.49578280644571926\\
  263.027 & 0.4124463876223504 & 0.5226776673017862 & 0.4956515865063651\\
  263.281546564802 & 0.41130633778185044 & 0.5214947016724047 & 0.4944103185017906\\
  265.5 & 0.40108440896302794 & 0.5116577084469104 & 0.4840893414135892\\
  265.7201105324507 & 0.4000760332024629 & 0.5107052725170199 & 0.4830904503659206\\
  267.9 & 0.3898186030049148 & 0.5012633449462124 & 0.47319548049799687\\
  268.1812609453013 & 0.3886130683772376 & 0.5000538277474289 & 0.4719287829032015\\
  269.153 & 0.38438916338556584 & 0.49591018525747305 & 0.4675904334463782\\
  270.4 & 0.3788344186165407 & 0.4906740089699294 & 0.4621109476451922\\
  270.6652070033241 & 0.3777346091401302 & 0.4895397495258546 & 0.460924836978223\\
  272.9 & 0.3682077988320573 & 0.48041627796842923 & 0.4513860779084721\\
  273.1721598441379 & 0.367109834876147 & 0.4793334061859296 & 0.45025445509493617\\
  275.4 & 0.3578739797208842 & 0.47045597030073744 & 0.4409850732630005\\
  275.423 & 0.3577868640586111 & 0.4703653123441136 & 0.44089046992773134\\
  275.70233256095827 & 0.35672535190852783 & 0.4692603075448936 & 0.43973754516299485\\
  278.0 & 0.3477457347523265 & 0.4603265112130297 & 0.4304221859596842\\
  278.25594022071255 & 0.3467701823086432 & 0.45931972701278956 & 0.4293734398985621\\
  280.5 & 0.33798623559948443 & 0.4508907596320281 & 0.42059559079512226\\
  280.833199882317 & 0.33679100380066396 & 0.44967278339758954 & 0.4193278917362178\\
  281.838 & 0.33313490047043803 & 0.44594163978415263 & 0.4154469287706153\\
  283.1 & 0.3284323288689355 & 0.44136912301618236 & 0.410693082164814\\
  283.43433061513093 & 0.32730482514690756 & 0.4401542617900213 & 0.40943078560022056\\
  285.8 & 0.3190952753373235 & 0.4317015432658968 & 0.40065441199233276\\
  286.0595535175745 & 0.3182129213861182 & 0.4307633682131869 & 0.39968132146892454\\
  288.4 & 0.31003968844242047 & 0.4226905652563343 & 0.3913112930356635\\
  288.403 & 0.3100302208042872 & 0.4226805234081609 & 0.3913008865502848\\
  288.7090917359235 & 0.3090611247788026 & 0.4216523287454361 & 0.39023551882423646\\
  291.1 & 0.3012769861903445 & 0.413610395978985 & 0.3819108312137016\\
  291.3831704832789 & 0.30039476394755515 & 0.41266479986313154 & 0.3809328460417734\\
  293.8 & 0.29265504738719944 & 0.4047357505230102 & 0.37273848750207766\\
  294.08201705870607 & 0.29181269311031016 & 0.4037999665872225 & 0.3717724313909785\\
  295.121 & 0.28866745776034036 & 0.40052704509380904 & 0.36839345832423304\\
  296.5 & 0.2843906565735824 & 0.3961446733859593 & 0.36387340910195254\\
  296.80586086656024 & 0.28348487058364197 & 0.3952015267491634 & 0.3629009380891479\\
  299.2 & 0.2762022646589659 & 0.38780856447816436 & 0.3552856307546914\\
  299.55493343598164 & 0.27522408695683753 & 0.3867216520573216 & 0.3541670686537827\\
  301.995 & 0.26830998961996355 & 0.3793772707819177 & 0.3466152335279644\\
  302.0 & 0.26829548081082133 & 0.37936210969327067 & 0.34659965920169356\\
  302.3294684405776 & 0.2674198234173036 & 0.378359520365013 & 0.345569902209465\\
  304.8 & 0.2606702332040651 & 0.3711830299817262 & 0.3382034172521044\\
  305.1297017182871 & 0.25980230162849555 & 0.37025067502519 & 0.3372471425477155\\
  307.6 & 0.25312099281598016 & 0.3632549523185391 & 0.3300794367752446\\
  307.95587129142234 & 0.2522600493342754 & 0.3622554796795312 & 0.3290564050178019\\
  309.03 & 0.24962494301114732 & 0.3592604383489879 & 0.32599218130623425\\
  310.5 & 0.24592938308643814 & 0.35523330790919955 & 0.3218753724323869\\
  310.8082173869064 & 0.2451643266978075 & 0.3543731149770575 & 0.3209967372415829\\
  313.3 & 0.23881371780987973 & 0.34773388433908486 & 0.31421974406011094\\
  313.68698245668793 & 0.2379132354748148 & 0.3467313270677413 & 0.3131972691543732\\
  316.2 & 0.23190364054105223 & 0.34020798725837537 & 0.3065516778188232\\
  316.228 & 0.23184289813413922 & 0.3401362109532938 & 0.306478620389656\\
  316.59241119835207 & 0.23104941802625198 & 0.3391983052245063 & 0.30552414791032695\\
  319.2 & 0.2252103950420852 & 0.33260351067055166 & 0.29881948698224836\\
  319.52475057592136 & 0.22450216596315625 & 0.33177317333350914 & 0.29797632540640423\\
  322.1 & 0.2187338647777695 & 0.32548829026046927 & 0.29159931313871534\\
  322.4842498408439 & 0.21794164321355777 & 0.32457630774884905 & 0.2906748323565064\\
  323.594 & 0.2156219005352494 & 0.3219023476487652 & 0.2879660693244112\\
  325.1 & 0.21239816329675287 & 0.31835828055094695 & 0.2843788763158564\\
  325.4711605531848 & 0.21165902522178995 & 0.3174834026114907 & 0.28349401180214284\\
  328.1 & 0.2062792427670856 & 0.31139615131115916 & 0.27734359972851913\\
  328.4857366030047 & 0.20552839796079053 & 0.3104935546856649 & 0.2764327597401309\\
  331.1 & 0.2003010858503392 & 0.3046501697890223 & 0.2705411680880661\\
  331.131 & 0.2002442927242565 & 0.30458310332354105 & 0.2704736041234342\\
  331.52823423194235 & 0.1995137549155991 & 0.3037200945434313 & 0.26960436703383905\\
  334.2 & 0.1944637668377588 & 0.2979062645171934 & 0.26375555679167617\\
  334.59891205499747 & 0.19375760753770865 & 0.29704582929094064 & 0.2628909461698056\\
  337.3 & 0.18884322952416321 & 0.2913221146982515 & 0.25714575161134345\\
  337.6980310825088 & 0.18815604792778198 & 0.29046986488430576 & 0.25629138443122873\\
  338.844 & 0.1861506488412259 & 0.2881409260271701 & 0.2539574253152642\\
  340.4 & 0.18336344818233816 & 0.28494510245250404 & 0.25075825899188237\\
  340.82585474234514 & 0.1826614299716487 & 0.2840988452544707 & 0.24991163824199097\\
  343.6 & 0.17795972991370781 & 0.2785774566634893 & 0.24439478603310663\\
  343.98264890229285 & 0.17734198480036978 & 0.27782233035975884 & 0.24364119412628857\\
  346.7 & 0.17283748674403407 & 0.2725566950889298 & 0.23839212786407746\\
  346.737 & 0.17277982367317374 & 0.27248457186268055 & 0.23832031150172697\\
  347.16868189265597 & 0.1721043963168061 & 0.27163947499029245 & 0.2374789812842192\\
  349.9 & 0.16771529225721132 & 0.26652992669478315 & 0.23239751420141913\\
  350.3842245290676 & 0.16702182522791195 & 0.2656505234866486 & 0.23152394667843226\\
  353.2 & 0.1628746981502981 & 0.2605261784304232 & 0.22644021134303455\\
  353.6295501355039 & 0.16226755417196387 & 0.25975152493317616 & 0.22567266308331027\\
  354.813 & 0.16057205192441432 & 0.2576297529178733 & 0.22357161291885505\\
  356.5 & 0.15809715801026517 & 0.25466645334920424 & 0.22064039011326228\\
  356.90493456752296 & 0.15752446772106524 & 0.2539416585415969 & 0.2199240767634531\\
  359.7 & 0.1534667942037523 & 0.2491624498911913 & 0.21520600250822688\\
  360.2106562357074 & 0.1528177034840213 & 0.2483151057180915 & 0.21437051154093156\\
  363.078 & 0.14906981928352012 & 0.24354661343866815 & 0.20967498070312052\\
  363.1 & 0.14904038349872745 & 0.24351051720979228 & 0.20963947639097016\\
  363.5469961293318 & 0.14846042248418295 & 0.242774079313688 & 0.20891526200017843\\
  366.4 & 0.14465923760789592 & 0.23815782574911726 & 0.20438124131988822\\
  366.91423784024937 & 0.14402972203198483 & 0.23731775027192215 & 0.20355725648956555\\
  369.8 & 0.14039948894639076 & 0.23281157732899163 & 0.1991428023465715\\
  370.31266758699235 & 0.13980855899301428 & 0.23203457485172996 & 0.1983825858723878\\
  371.535 & 0.13837987207906546 & 0.2301537734923114 & 0.19654375197849436\\
  373.3 & 0.13626760532978124 & 0.22749854686891416 & 0.19395067933166338\\
  373.74257423910643 & 0.13575750738075323 & 0.22683264033583575 & 0.19330094061400638\\
  376.7 & 0.13225699129549504 & 0.22246331665576088 & 0.18904320339378497\\
  377.2042493417001 & 0.13171518483793299 & 0.22171108475493512 & 0.18831120517813998\\
  380.189 & 0.12841933679804304 & 0.21745722894482244 & 0.18417713247852174\\
  380.2 & 0.12840690843021105 & 0.21744207296958912 & 0.18416241989157017\\
  380.6979871402284 & 0.1278821914584303 & 0.216752981211728 & 0.18349363449900669\\
  383.7 & 0.12463254796417234 & 0.2125911811980162 & 0.17946002167188227\\
  384.2240846055061 & 0.1241121211987201 & 0.21187192841221686 & 0.17876389968773013\\
  387.3 & 0.12097198040055142 & 0.20772457568264582 & 0.17475547236560868\\
  387.78284145894537 & 0.1204919071447407 & 0.20706709530658507 & 0.17412091861204\\
  389.045 & 0.1192203442184534 & 0.20543684627805198 & 0.17254852183684383\\
  390.8 & 0.11741213638243483 & 0.2031414321571201 & 0.1703372214722934\\
  391.3745601980384 & 0.11688955606933116 & 0.2024164625764893 & 0.16963944865358413\\
  394.5 & 0.11396614119975804 & 0.19846440047417033 & 0.16584114668149624\\
  394.9995461220647 & 0.11351131394758408 & 0.19783882635060238 & 0.16524078135578557\\
  398.1 & 0.1106121433106847 & 0.1940261988646803 & 0.16158688125967008\\
  398.107 & 0.11060615226560704 & 0.19401754755530215 & 0.16157860034266897\\
  398.6581073580439 & 0.11013254221672508 & 0.19333342040032017 & 0.16092390985426278\\
  401.8 & 0.10735786596659046 & 0.18960699191082184 & 0.15736295982402712\\
  402.35055488692933 & 0.10689819476492314 & 0.18897332599433783 & 0.15675831880416513\\
  405.5 & 0.10419676972780324 & 0.18534106014043217 & 0.15329740927399668\\
  406.07720257003695 & 0.10374139471440251 & 0.18468234792149077 & 0.15267070483092257\\
  407.38 & 0.10269938698706559 & 0.18320128590328238 & 0.1512626259173051\\
  409.3 & 0.10112777876060842 & 0.18106912274289247 & 0.14923814353046416\\
  409.83836717572615 & 0.10070535317249132 & 0.18045974517059027 & 0.14866009175908373\\
  413.0 & 0.09815838236392506 & 0.1770391144712664 & 0.14542007841550295\\
  413.6343684063278 & 0.09769792060593277 & 0.17637399284763242 & 0.14479103431309306\\
  416.869 & 0.09528426466876873 & 0.17297399079151346 & 0.14158025310834965\\
  416.9 & 0.09526059938532247 & 0.17294188994816348 & 0.14154997840386274\\
  417.46552892531344 & 0.09485351405991602 & 0.17235362061949783 & 0.14099530616751887\\
  420.7 & 0.0924624147290514 & 0.1690495170568054 & 0.13788451417632316\\
  421.3321743847289 & 0.09202920102772534 & 0.1683978918857663 & 0.13727193896971387\\
  424.6 & 0.08972818523872633 & 0.16517726007943534 & 0.13424906868595138\\
  425.2346334528686 & 0.08930902032310684 & 0.16457096754410833 & 0.13368089900643926\\
  426.58 & 0.08840816621428188 & 0.16326637083195317 & 0.13245924696052508\\
  428.5 & 0.08709361103217116 & 0.16144334768115778 & 0.13075432851181892\\
  429.17323784221577 & 0.08667072931732628 & 0.160805867924802 & 0.13015876607109117\\
  432.5 & 0.08452298960266812 & 0.1577104785770204 & 0.12727141352806906\\
  433.14832233764025 & 0.08412825003010106 & 0.15710182196520642 & 0.12670453532542342\\
  436.5 & 0.08203147157759878 & 0.15409327560933225 & 0.12390706584699103\\
  436.516 & 0.08202233416336652 & 0.15407942262517063 & 0.12389420251162074\\
  437.1602248248502 & 0.08165279455122508 & 0.15351895531447204 & 0.12337391083565097\\
  440.6 & 0.07962446524537317 & 0.1505200481814911 & 0.12059427588497726\\
  441.209286319119 & 0.07927451407202088 & 0.14999444154030095 & 0.12010788606419484\\
  444.6 & 0.07727482940831368 & 0.14712219950459896 & 0.11745408523391433\\
  445.295850994266 & 0.07689676553938452 & 0.14652757142031014 & 0.11690553347865172\\
  446.684 & 0.07613210992449194 & 0.145402121044499 & 0.11586827087980253\\
  448.7 & 0.07499674321208549 & 0.1437447797744499 & 0.11434271997009522\\
  449.42026621191417 & 0.07462670765129706 & 0.1431746404213258 & 0.11381853430925123\\
  452.9 & 0.07278907936649523 & 0.14041267924975107 & 0.11128317772170108\\
  453.58288255101905 & 0.07244735360142274 & 0.13987674264822691 & 0.11079202559923224\\
  457.088 & 0.07064514813223843 & 0.13717456506416337 & 0.10831966739800702\\
  457.1 & 0.07063883942658615 & 0.13716527590961497 & 0.108311179609464\\
  457.78405383766165 & 0.07030764438838225 & 0.1366332305798098 & 0.10782515771416866\\
  461.3 & 0.06855897211159295 & 0.13401834058643503 & 0.1054406150689818\\
  462.0241371751313 & 0.06822607562295106 & 0.13349674687899077 & 0.10496579555721916\\
  465.6 & 0.06653658070326347 & 0.13091444555145293 & 0.10261879707748359\\
  466.30349297427364 & 0.06622333508849193 & 0.13041215124675604 & 0.10216304068025407\\
  467.735 & 0.06557727098823615 & 0.12939209129928345 & 0.101238220372045\\
  469.9 & 0.06457808753063034 & 0.12788994394885908 & 0.09987833588193042\\
  470.62248498412816 & 0.06426571071075865 & 0.1273788487918312 & 0.09941611127792457\\
  474.2 & 0.06267701717554049 & 0.12495785884729049 & 0.09723052410030314\\
  474.9814803228505 & 0.06235664775521522 & 0.12444603246001724 & 0.09676929198053687\\
  478.6 & 0.060832295662525085 & 0.12206891692775801 & 0.09463058611688677\\
  478.63 & 0.060820704138030965 & 0.12204954137463868 & 0.09461317921904684\\
  479.38084950891067 & 0.060529207506014836 & 0.12156211474555272 & 0.09417540211879112\\
  483.1 & 0.059045045366273724 & 0.11919029913470687 & 0.09204882542746082\\
  483.82096649259574 & 0.05876539042458982 & 0.1187264783914532 & 0.09163364024787383\\
  487.5 & 0.057299964973577165 & 0.11646283770499902 & 0.08961107405873235\\
  488.30220868778844 & 0.05700686027107512 & 0.11598514949841147 & 0.0891850395789354\\
  489.779 & 0.05645980973809878 & 0.11509260498854534 & 0.0883896169619376\\
  492.0 & 0.05561883272553598 & 0.11377654906435587 & 0.08721846563909792\\
  492.8249570040513 & 0.055331690361636425 & 0.11328988996353467 & 0.08678590179996797\\
  496.6 & 0.05398109477245934 & 0.11110163587259145 & 0.08484428078732316\\
  497.3895958790068 & 0.05371570007345576 & 0.11064005915526601 & 0.08443540487954125\\
  501.187 & 0.052404243777931236 & 0.10851680970984308 & 0.08255816135229588\\
  501.2 & 0.05239965437444061 & 0.10850980931937101 & 0.08255198194908149\\
  501.99651331100796 & 0.052137891116573784 & 0.10807870357647555 & 0.08217154671727693\\
  505.8 & 0.05085396242398327 & 0.10601423926662913 & 0.08035269167780128\\
  506.64610089212687 & 0.05059065171237447 & 0.10556066875779622 & 0.07995380326722483\\
  510.5 & 0.04935814147413253 & 0.10353081298226378 & 0.07817182128701165\\
  511.3387538414332 & 0.049105742229505124 & 0.10308536656589666 & 0.07778142089808485\\
  512.861 & 0.04864139390188678 & 0.10231872420099414 & 0.07711030267956319\\
  515.2000000000002 & 0.04791213743123037 & 0.10112307299372875 & 0.07606498973762606\\
  516.0748710385907 & 0.04766196748832367 & 0.10069304128655039 & 0.07568956598431441\\
  520.0 & 0.04650839664114787 & 0.09875773940569993 & 0.07400283628070112\\
  520.8548550577666 & 0.04627012964794895 & 0.09834142125699634 & 0.073640657224716\\
  524.8 & 0.04514040025019878 & 0.09645399719282294 & 0.07200161540569812\\
  524.807 & 0.04513856814025446 & 0.09645063833325089 & 0.07199870266683177\\
  525.6791122018419 & 0.044909204568280646 & 0.09602999198372023 & 0.07163403415130172\\
  529.7 & 0.0438222706179898 & 0.09417497149372633 & 0.07002911425341737\\
  530.5480525369575 & 0.04360526543126589 & 0.09379628826285062 & 0.06970213545656925\\
  534.6 & 0.04253988528934938 & 0.0919821392761137 & 0.0681383085817949\\
  535.4620899273614 & 0.04232514626108066 & 0.0916008391538759 & 0.0678102307186136\\
  537.032 & 0.04192884076171079 & 0.09090637314159948 & 0.06721319328335351\\
  539.5 & 0.04129211656226355 & 0.08984675325203721 & 0.06630373808328914\\
  540.4216420705915 & 0.04107500645134781 & 0.08944318177996413 & 0.06595772673970299\\
  544.5 & 0.04008773930561047 & 0.08773403608642198 & 0.06449535155328494\\
  545.4271305329836 & 0.03987575517938348 & 0.08735831015399577 & 0.0641745266073891\\
  549.5 & 0.038919106476117335 & 0.08570221851424502 & 0.06276278848981025\\
  549.541 & 0.03891018206510773 & 0.08568585348708305 & 0.0627488603600011\\
  550.4789807854968 & 0.03870496782195181 & 0.08530937946733744 & 0.06242855114184971\\
  554.6 & 0.03777865948226828 & 0.08368439783700365 & 0.061048538582526304\\
  555.5776222398879 & 0.03757679896512218 & 0.08329590109290365 & 0.060719183615354014\\
  559.8 & 0.03668047825194461 & 0.0816902927228817 & 0.05936087465992324\\
  560.7234882852038 & 0.036491083828684566 & 0.08135056513094302 & 0.0590740626876828\\
  562.341 & 0.036154908962089234 & 0.0807469152464106 & 0.058564817809963324\\
  564.9 & 0.03561151812803603 & 0.07980931877490327 & 0.05777508934409877\\
  565.9170163246242 & 0.035417463026910546 & 0.07943900132072966 & 0.057463588346316014\\
  570.2 & 0.0345772652906656 & 0.07790644770965464 & 0.056176891190052106\\
  571.1586478126435 & 0.034395982776158386 & 0.07756068431095259 & 0.055887107248296666\\
  575.4 & 0.03357223582915192 & 0.0760960109735079 & 0.05466214592972753\\
  575.44 & 0.03356524295773076 & 0.07608274146358956 & 0.05465106801254132\\
  576.4488282925873 & 0.03338795215147213 & 0.0757461613780897 & 0.0543701753117123\\
  580.8 & 0.03260191170759886 & 0.0742897456681053 & 0.053156822109487786\\
  581.7880074344935 & 0.032428867856663476 & 0.0739632790941359 & 0.052885375902397655\\
  586.1 & 0.03165320957288315 & 0.07256368328932718 & 0.051723841846269505\\
  587.1766390733261 & 0.031478450996872055 & 0.07221158741448853 & 0.05143215002254493\\
  588.844 & 0.031204018014999703 & 0.07169453767220836 & 0.05100439508427225\\
  591.6 & 0.03074033879984179 & 0.07082683414672154 & 0.050287504825529225\\
  592.6151812475553 & 0.030576394572384633 & 0.07051960049956844 & 0.050034091670588934\\
  597.0 & 0.02984908876766787 & 0.06918797923790097 & 0.04893760823120411\\
  598.1040962380944 & 0.029683950959390873 & 0.06885726932186888 & 0.04866584259189302\\
  602.56 & 0.02899882956779135 & 0.06754563979178208 & 0.047590073607706125\\
  602.6 & 0.028992544542490072 & 0.06753383932171973 & 0.04758040943127058\\
  603.6438506075863 & 0.028837494483977863 & 0.0672241875991092 & 0.047326900867434005\\
  608.1 & 0.02815761985202236 & 0.06595818880390056 & 0.04629269733272154\\
  609.2349152400711 & 0.027999275666986106 & 0.06564690671377015 & 0.04603897265540144\\
  613.8 & 0.027344448636989104 & 0.06439019790178523 & 0.045016432973080237\\
  614.8777653810029 & 0.027195136512757425 & 0.06409740849263015 & 0.044778679209267834\\
  616.595 & 0.026954031249205933 & 0.06362963955963848 & 0.04439915629670636\\
  619.4 & 0.026551773108995286 & 0.0628906237144187 & 0.04380064926685552\\
  620.5728806776501 & 0.02640208897322217 & 0.06257536326252305 & 0.04354561382666465\\
  625.2 & 0.02579492598960991 & 0.06138415456313704 & 0.042584138367337224\\
  626.3207452198692 & 0.02565330609584162 & 0.0611054491916463 & 0.042359690859124964\\
  630.957 & 0.025051371020281616 & 0.0599483058110681 & 0.041429432994647436\\
  631.0 & 0.02504566772056936 & 0.05993777936445586 & 0.04142098509101693\\
  632.1218475812449 & 0.02491188667760111 & 0.05966158290363633 & 0.041199406367095646\\
  636.8 & 0.024338625671943434 & 0.05853007806797414 & 0.04029342878219597\\
  637.9766808606282 & 0.02420343675178055 & 0.058243388873040786 & 0.040064305050167226\\
  642.7 & 0.02364569055157824 & 0.05714109198669547 & 0.03918534289608454\\
  643.8857427240426 & 0.02351215491750919 & 0.0568739059215463 & 0.038972774022978295\\
  645.654 & 0.023310300440698022 & 0.05646963984782007 & 0.03865138824071011\\
  648.6 & 0.022966818653948534 & 0.055807474721926445 & 0.03812584447997764\\
  649.8495354469889 & 0.022834455615458594 & 0.055528849536104354 & 0.0379050332394079\\
  654.6 & 0.022317255374932825 & 0.05448776757796431 & 0.03708160467700682\\
  655.8685659571436 & 0.022186413919890156 & 0.054207805561707754 & 0.036860586893604046\\
  660.693 & 0.021674954164146387 & 0.05318746629697038 & 0.036056930714040966\\
  660.7 & 0.02167419624978946 & 0.0531860459390182 & 0.03605581418485937\\
  661.9433458774388 & 0.021551562000440564 & 0.05293227745801421 & 0.03585640683569454\\
  666.8 & 0.02105927558638434 & 0.05193700535436683 & 0.03507570342705446\\
  668.0743915695614 & 0.020939997195067766 & 0.051679571372755424 & 0.03487420179481503\\
  673.0 & 0.020466062296313776 & 0.05070172744938592 & 0.03411034731982755\\
  674.2622241778349 & 0.020350672902241677 & 0.050449332936968426 & 0.03391355037552486\\
  676.083 & 0.0201819466166861 & 0.050104287666181226 & 0.03364492688924853\\
  679.2 & 0.0198869118188877 & 0.04950327875946665 & 0.033177641595643265\\
  680.5073696735207 & 0.019773739448391014 & 0.04926163602413779 & 0.032990122850184406\\
  685.5 & 0.019329466562920374 & 0.04833498915981613 & 0.032272293757070594\\
  686.8103588995307 & 0.019217305327026105 & 0.04809526628267841 & 0.032086995689864256\\
  691.8 & 0.018778484008467055 & 0.04719822214437754 & 0.03139499606254687\\
  691.831 & 0.018776055614657592 & 0.047192643989691925 & 0.03139069949770313\\
  693.17172761554 & 0.018670440704791073 & 0.04694993283964068 & 0.03120382588433646\\
  698.2 & 0.018263282401015598 & 0.04607718519380382 & 0.030533432886095363\\
  699.5920165435375 & 0.01815533244226247 & 0.04584426819697149 & 0.03035495777642102\\
  704.7 & 0.017748107528804125 & 0.04498575996712325 & 0.02969827701069988\\
  706.0717714137779 & 0.017644589224168485 & 0.0447585443141641 & 0.02952485309525262\\
  707.946 & 0.017501209422543847 & 0.04444633209210507 & 0.029286752816761675\\
  711.2 & 0.01724699512007113 & 0.04392384005259763 & 0.0288890859176205\\
  712.6115430111745 & 0.01714667574465266 & 0.04369253081631297 & 0.028713243338296324\\
  717.8 & 0.0167675864561757 & 0.04287738458889924 & 0.028095040432444346\\
  719.2118872221192 & 0.016670843861187445 & 0.04266350982093689 & 0.02793324269778384\\
  724.4 & 0.01630548003258942 & 0.041873974149081145 & 0.027336992937051403\\
  724.436 & 0.01630312022423095 & 0.04186861120924593 & 0.027332950304332148\\
  725.8733650817246 & 0.01620836578705468 & 0.04165315047402767 & 0.027170603595894075\\
  731.1 & 0.01585423621614782 & 0.04088309857100026 & 0.02659155499559183\\
  732.596542821523 & 0.01575981955089642 & 0.04066117216994083 & 0.026425001968928226\\
  737.9 & 0.015415800289471294 & 0.03990686626860505 & 0.025860266780676596\\
  739.3819919175874 & 0.01532512209308912 & 0.03970369885122742 & 0.02570853601112141\\
  741.31 & 0.015205515943483265 & 0.03943550930725551 & 0.025508392101012772\\
  744.7 & 0.014990779132525268 & 0.038971248397017794 & 0.02516251770638889\\
  746.2302891391108 & 0.014901311847633672 & 0.03876370595452889 & 0.02500815244661776\\
  751.6 & 0.014578563526520925 & 0.03804778259552502 & 0.024476754474608252\\
  753.1420165974375 & 0.01449233735980741 & 0.037840862991544495 & 0.024323471714092798\\
  758.578 & 0.014179799042060084 & 0.03714117725448915 & 0.023806412736745903\\
  758.6 & 0.01417850750127425 & 0.03713846553795319 & 0.023804413098231815\\
  760.1177617955323 & 0.014096171888672885 & 0.036950218344495876 & 0.02366566163186469\\
  765.6 & 0.013790457432805558 & 0.036267057945556375 & 0.023163000968762094\\
  767.1581176779302 & 0.013709717945197554 & 0.03607585983593073 & 0.023022646363185476\\
  772.7 & 0.01341445397558811 & 0.03540738259017745 & 0.022532940382981988\\
  774.2636826811278 & 0.013335688622220397 & 0.035217517001033746 & 0.02239411926807862\\
  776.247 & 0.013234405410470244 & 0.03498933172657035 & 0.02222756492003706\\
  779.8 & 0.01304916239670927 & 0.03457262860636374 & 0.02192379297289528\\
  781.4350607844542 & 0.012970475808247058 & 0.034389237327506525 & 0.021790394006396895\\
  787.0 & 0.012695154962929084 & 0.03376176877156267 & 0.021334762084077575\\
  788.6728615614156 & 0.012617999084252676 & 0.033576140635449725 & 0.021200288442977652\\
  794.3 & 0.012351138133136994 & 0.03296219513372335 & 0.02075644723658115\\
  794.328 & 0.012349908395782346 & 0.032959140458395104 & 0.02075424238170866\\
  795.9777002314978 & 0.012277035422115331 & 0.03277801689666973 & 0.020623569029311728\\
  801.7 & 0.012017108066864369 & 0.032175278473293656 & 0.020189789438341973\\
  803.3501977124735 & 0.011946524561907947 & 0.03200786840226597 & 0.020069632077097416\\
  809.1 & 0.011693678964471058 & 0.031421619452905745 & 0.01964958171543652\\
  810.7909806731694 & 0.011624330987396568 & 0.03125189162738287 & 0.01952825199864808\\
  812.831 & 0.011539500719830028 & 0.031045302905652244 & 0.019380686526108984\\
  816.6 & 0.011379477941125496 & 0.03067877767418161 & 0.019119455452049898\\
  818.300681586739 & 0.011311632507641351 & 0.030509935386166257 & 0.01899926617269638\\
  824.1 & 0.011073821002530284 & 0.029957240763951537 & 0.018606800892468234\\
  825.8799387844273 & 0.011007101796459985 & 0.0297940248537239 & 0.01849122202669258\\
  831.764 & 0.010780254032447784 & 0.02925152500325678 & 0.01810772025909166\\
  831.8 & 0.010778837158148456 & 0.02924827927081416 & 0.018105430267708108\\
  833.5293965098188 & 0.01071571700252101 & 0.029091355807829962 & 0.01799477049225375\\
  839.5 & 0.010491635203925936 & 0.028558768125333908 & 0.017619974883490246\\
  841.2497049736119 & 0.01042965410499367 & 0.028401725155964497 & 0.017509689860546622\\
  847.2 & 0.010212978961494559 & 0.027889019519920143 & 0.01715052694301433\\
  849.0415204088755 & 0.01015133162515544 & 0.027736354697705138 & 0.01704387095978644\\
  851.138 & 0.01008015594994809 & 0.027559987023447988 & 0.016920740975317535\\
  855.1 & 0.009942824764678938 & 0.027231456973620442 & 0.01669178950460221\\
  856.9055051268348 & 0.009884313173910673 & 0.027083383856650788 & 0.016588786638710943\\
  863.0 & 0.009681214094837274 & 0.026591986931999535 & 0.01624766525754477\\
  864.8423275731726 & 0.00962384931017032 & 0.02644255121465781 & 0.01614414832134403\\
  870.964 & 0.009427840168616553 & 0.02596581820781922 & 0.015814730573531784\\
  871.0 & 0.009426663682620278 & 0.02596313865091522 & 0.015812883342010947\\
  872.852662384837 & 0.00937075117626944 & 0.02582433158813772 & 0.015717245140793416\\
  879.0 & 0.009180007970288999 & 0.025361167920063068 & 0.015398657265727759\\
  880.9371904473991 & 0.009124780431464714 & 0.025217633299207818 & 0.01530017772382973\\
  887.2 & 0.00894109440158612 & 0.024761289721566777 & 0.014987727932631348\\
  889.0965989529167 & 0.008888607453740217 & 0.024622248461566177 & 0.014892721420522694\\
  891.251 & 0.008828155887624999 & 0.024472634702712562 & 0.014790680909445282\\
  895.4 & 0.008709315246032984 & 0.024178718575140735 & 0.01459046988980363\\
  897.3315814583519 & 0.008657336036372297 & 0.024047965271443233 & 0.014501623345709445\\
  903.6 & 0.00848391064202763 & 0.023621135228116423 & 0.014212068833291323\\
  905.6428379445293 & 0.008431948474508911 & 0.023484399227624506 & 0.01411955010214899\\
  912.0 & 0.00826559949060176 & 0.023065869274558816 & 0.013836946013062046\\
  912.011 & 0.008265329518416143 & 0.023065145803284524 & 0.013836458296435067\\
  914.0310748756223 & 0.008215461874583826 & 0.022931402318188254 & 0.013746348172853166\\
  920.4 & 0.008053777970111756 & 0.022526192405674172 & 0.013474019399980318\\
  922.4970052592174 & 0.008004747494983953 & 0.02239800670630533 & 0.013388130459377461\\
  929.0 & 0.007848288835518998 & 0.02199807017770258 & 0.013120600380378843\\
  931.0413487069085 & 0.007802011227588521 & 0.02187459345990684 & 0.013038208346032148\\
  933.254 & 0.007751145919468563 & 0.02173908467979479 & 0.012947847161091314\\
  937.6 & 0.007649174985508399 & 0.02148457223465486 & 0.012778546006794194\\
  939.6648314954691 & 0.00760387658341905 & 0.02136108297357862 & 0.012696509238833637\\
  946.2 & 0.00745643670024439 & 0.020985487927169748 & 0.012447618099557377\\
  948.3681866285928 & 0.007411518826846472 & 0.02086578723046853 & 0.012368543125744142\\
  954.993 & 0.0072702946562708095 & 0.020497721573060304 & 0.012125787461882016\\
  955.0 & 0.007270142401880194 & 0.020497341882429774 & 0.012125537560529821\\
  957.1521538991856 & 0.007226735973305476 & 0.020379816177254817 & 0.012048233463931319\\
  963.8 & 0.00708881396016523 & 0.020022753992145925 & 0.011813847130327433\\
  966.0174799522646 & 0.007045969268965141 & 0.019903023889161417 & 0.011735430571521837\\
  972.7 & 0.00691313565037921 & 0.01955617175288998 & 0.011508833914758414\\
  974.9649183484096 & 0.006871064533218734 & 0.019443174713848804 & 0.011435233155491222\\
  977.237 & 0.00682825283617295 & 0.01932820830307758 & 0.011360396548700495\\
  981.7 & 0.006742457152727386 & 0.01910521032729535 & 0.011215500987845305\\
  983.9952296278226 & 0.006701717746183665 & 0.018992065342998455 & 0.011142137503247699\\
  990.8 & 0.006577425714976435 & 0.01866204282577087 & 0.010928581939595233\\
  993.10918137498 & 0.00653814573341676 & 0.018549478216102144 & 0.010855910447172549\\
\end{comment}

\end{longtable}

% End tab


==> LBG_hiz.tex <==
\begin{table}[h]
\centering

\sisetup{table-column-width=12ex,    % local setting for all S columns
         round-mode=places,
         round-precision=2,
         tight-spacing,
         table-format = 5.2e-2,
         table-number-alignment = center
         }

\begin{tabular}{|l|S|S|S|S|}

\hline
\hline
  \multicolumn{1}{|c|}{id} &
  \multicolumn{1}{c|}{$\lambda\ [\mu m]$} &
  \multicolumn{1}{c|}{$f_\nu\ /\ f_{200\mu m}$} &
  \multicolumn{1}{c|}{error} &
  \multicolumn{1}{c|}{S/N} \\
\hline
  Stack\_hiz\_0 & 15.484 & 0.6041071368176998 & -0.6041071368176998 & -1.0\\
  Stack\_lowz\_0 & 18.299 & 0.4070780403478624 & -0.4070780403478624 & -1.0\\
  Stack\_hiz\_1 & 24.905 & 1.8794443589743441 & -1.8794443589743441 & -1.0\\
  Stack\_lowz\_1 & 29.434 & 1.139818500842144 & -1.139818500842144 & -1.0\\
  Stack\_hiz\_2 & 38.196 & 1.9465673074955887 & 1.141091225093072 & 1.7058822859117322\\
  Stack\_lowz\_2 & 45.141 & 2.035390171409635 & 0.6513248402928382 & 3.1250000698491944\\
  Stack\_hiz\_3 & 53.562 & 3.356150626736888 & 1.2753372221566444 & 2.631578980390385\\
  Stack\_lowz\_3 & 63.3 & 3.5822866822699644 & 0.8141560806957248 & 4.399999910593035\\
  Stack\_hiz\_4 & 77.043 & 2.8191664384404334 & 1.0068452280294997 & 2.799999801317859\\
  Stack\_lowz\_4 & 91.051 & 3.9079490417570293 & 0.8141560806957248 & 4.799999821186068\\
  Band\_0 & 130.428 & 2.3607768939276412 & 0.2981832794287399 & 7.91720078486769\\
  Band\_1 & 130.436 & 2.165732599053267 & 0.6473943153826967 & 3.345306789994023\\
  Band\_2 & 130.593 & 1.7383349717928915 & 0.06065561941986783 & 28.65909190968541\\
  Stack\_hiz\_5 & 131.912 & 2.886289587003844 & 0.7383531338812721 & 3.9090909952959745\\
  Band\_3 & 132.807 & 1.981433127078801 & 0.16127944689702453 & 12.285713804214174\\
  Band\_4 & 132.932 & 2.1963292681861524 & 0.37231538599521935 & 5.899109601165808\\
  Band\_5 & 132.969 & 2.080220715848803 & 0.4840117172916773 & 4.297872637234547\\
  Band\_6 & 132.988 & 2.1875912071262826 & 0.47910729937980717 & 4.56597344677918\\
  Band\_7 & 133.815 & 1.926573426556951 & 0.49219554067981136 & 3.914243968760878\\
  Band\_8 & 136.152 & 2.057241450590362 & 0.6135251699120721 & 3.353149229207984\\
  Band\_9 & 138.248 & 2.0799540884965326 & 0.3253903546858025 & 6.392181140418067\\
  Band\_10 & 140.737 & 1.967469090431378 & 0.5666501690993686 & 3.4721053618645614\\
  Band\_11 & 151.261 & 1.668029595671763 & 0.33084882759697015 & 5.0416669383024235\\
  Band\_12 & 155.91 & 1.7071804939961757 & 0.5190183719080613 & 3.2892486786548374\\
  Band\_13 & 155.958 & 1.7343377926481176 & 0.5241091851108297 & 3.3091154322765193\\
  Band\_14 & 155.98 & 1.7165841217676614 & 0.44392731378008465 & 3.866813481582782\\
  Band\_15 & 156.087 & 1.5105290584441402 & 0.2577302260446886 & 5.86089214922826\\
  Band\_16 & 156.44 & 1.6482686941510394 & 0.1983141484234364 & 8.31140242516479\\
  Band\_17 & 156.88 & 1.4993950340478046 & 0.08418023607021971 & 17.811722846643843\\
  Stack\_lowz\_5 & 156.946 & 1.465480981647917 & 0.569909250421072 & 2.57142866266017\\
  Band\_18 & 156.974 & 1.6857717137991153 & 0.3374836213241303 & 4.995121562299597\\
  Band\_19 & 157.337 & 1.6392424594698074 & 0.327254926319203 & 5.009068856219135\\
  Band\_20 & 157.596 & 1.6579979296267946 & 0.30177525864408145 & 5.494147986406877\\
  Band\_21 & 157.628 & 1.4474635873563206 & 0.2757073666017081 & 5.249999683350329\\
  Band\_22 & 158.184 & 1.6549383338003856 & 0.36096258262153563 & 4.5847919243628805\\
  Band\_23 & 159.984 & 1.7296819522255344 & 0.5653448382309686 & 3.0595166617916165\\
  Band\_24 & 160.702 & 1.5750590728174647 & 0.05011551777173926 & 31.428570288176477\\
  Band\_25 & 160.8 & 1.5945760229282628 & 0.4517856276440482 & 3.529497012208174\\
  Stack\_hiz\_6 & 172.389 & 0.671230135349486 & 0.46986108974358604 & 1.428571443776695\\
  Band\_26 & 174.461 &  &  & \\
  Band\_27 & 176.835 & 1.2341998894178108 & 0.1234199931599031 & 9.99999965823025\\
  Band\_28 & 181.442 &  &  & \\
  Band\_29 & 192.119 & 1.1993270334194406 & 0.19299515456701574 & 6.214285721888348\\
  Stack\_lowz\_6 & 203.732 & 0.6513248402928382 & 0.3256624201464191 & 2.0\\
  Band\_30 & 204.438 & 0.9511903973153636 & 0.15163904854966956 & 6.272727285042283\\
  Band\_31 & 204.647 & 1.0023103287640929 & 0.028637439202970513 & 34.99999848660089\\
  Band\_32 & 218.164 & 0.7875295364087324 & 0.028637439202970513 & 27.499998544808548\\
\hline\hline\end{tabular}
\caption{IR composite built from the sample of ALMA-detected objects. S/N = -1.00 and negative errors mean that the data in the given band is an upper limit.}
\label{Tab.SED_IR.composite.data}
\end{table}

==> Physical_parameters_dl2014_final_21Oct.tex <==
\onecolumn
\sisetup{table-column-width=12ex,    % local setting for all S columns
         round-mode=places,
         round-precision=3,
         tight-spacing,
         table-format = 5.3e-2,
         table-number-alignment = center
         }
%\begin{sidewaystable}
  \begin{table}[h!]
  \centering
\begin{adjustbox}{max width=\textwidth}

%\begin{longtable}{|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|}
\begin{tabular}{|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|}

\hline
  \multicolumn{1}{|c|}{id} &
  \multicolumn{1}{c|}{redshift} &
  \multicolumn{1}{c|}{$\beta_{FUV}$} &
  \multicolumn{1}{c|}{$\beta_{FUV}$\_err} &
  \multicolumn{1}{c|}{sSFR} &
  \multicolumn{1}{c|}{sSFR\_err} &
  \multicolumn{1}{c|}{sM$_{dust}$} &
  \multicolumn{1}{c|}{sM$_{dust}$\_err} &
  \multicolumn{1}{c|}{A$_{FUV}$} &
  \multicolumn{1}{c|}{A$_{FUV}$\_err} &
  \multicolumn{1}{c|}{IRX} &
  \multicolumn{1}{c|}{IRX\_err} &
  \multicolumn{1}{c|}{age$_{main}$} &
  \multicolumn{1}{c|}{age$_{main}$\_err} &
  \multicolumn{1}{c|}{L$_{dust}$} &
  \multicolumn{1}{c|}{L$_{dust}$\_err} &
  \multicolumn{1}{c|}{M$_{dust}$} &
  \multicolumn{1}{c|}{M$_{dust}$\_err} &
  \multicolumn{1}{c|}{L$_{FUV}$} &
  \multicolumn{1}{c|}{L$_{FUV}$\_err} &
  \multicolumn{1}{c|}{SFR} &
  \multicolumn{1}{c|}{SFR\_err} &
  \multicolumn{1}{c|}{M$_{star}$} &
  \multicolumn{1}{c|}{M$_{star}$\_err} \\
     &   &   &   & [yr$^{-1}$] & [yr$^{-1}$] &   &   &   &   &   &   & [Myrs] & [Myrs] & [L$_\odot$] &  & [M$_\odot$] & [M$_\odot$] & [L$_\odot$] & [L$_\odot$] & [M$_\odot$ yr$^{-1}$] & [M$_\odot$ yr$^{-1}$] & [M$_\odot$ yr$^{-1}$] & [M$_\odot$ yr$^{-1}$] \\
\hline
  CANDELS\_GOODSS\_12 & 4.431000232696533 & -2.144344430007398 & 0.1460967634012939 & 1.1149208811350329E-8 & 3.4331387798514106E-9 & 0.013814630122584031 & 0.004252890556071374 & 1.5888425205667631 & 0.09549578768207853 & 0.6576055662636281 & 0.05054404171237296 & 205.2676153342721 & 68.8026706449075 & 3.289149898984435E11 & 3.444087607084101E10 & 5.488870198868826E7 & 5747427.27130018 & 7.200213239389786E10 & 3.6001066196948934E9 & 44.298370236886015 & 4.647950695210735 & 3.97322993823459E9 & 1.150247287111027E9\\
   CANDELS\_GOODSS\_14 & 5.552700042724609 & -1.9627663677483977 & 0.06621954990145637 & 1.326194276577744E-9 & 1.1576960863836385E-10 & 8.389036769235726E-4 & 1.9276863518511448E-4 & 0.38895337243364636 & 0.07643916190570746 & -0.2178516335164711 & 0.10904574939109347 & 1028.232758327914 & 20.615745087813362 & 1.0336335052519156E11 & 2.2754735569254753E10 & 1.7249077475250736E7 & 3797266.5820972957 & 1.6635877899400333E11 & 8.317938949700168E9 & 27.26847962785562 & 1.5620781687034537 & 2.0561451749152596E10 & 1.3543682219820144E9\\
   CANDELS\_GOODSS\_19 & 4.5 & -0.5577911744909068 & 0.10923765003146907 & 2.0791810501074646E-9 & 4.0873965089761124E-10 & 0.0039209999786145675 & 7.389569536895512E-4 & 2.5099058774851524 & 0.1380529502851573 & 1.1267584398851647 & 0.05772417621057204 & 792.2062394855445 & 126.16545886623689 & 5.49213234346225E11 & 6.8077912733368996E10 & 9.165165004362184E7 & 1.136071136553421E7 & 4.073865421849303E10 & 2.0369327109246514E9 & 48.599942622063324 & 6.609169505728361 & 2.3374560199820686E10 & 3.3182618820359697E9\\
   CANDELS\_GOODSS\_21 & 5.571599960327148 & -1.385195733484872 & 0.2240503999483133 & 2.955331329981361E-9 & 1.1827481700911702E-9 & 0.004595338622398079 & 0.0018443431792643092 & 1.7606691956564664 & 0.11242903814406449 & 0.762352550409809 & 0.057306132909870695 & 606.6511224709545 & 194.58770651261204 & 2.0194602332656482E11 & 1.6969794863164623E10 & 3.370036463097957E7 & 2831886.7843056116 & 3.48423369083178E10 & 1.74211684541589E9 & 21.673210966497958 & 1.6990243294516578 & 7.333597673677641E9 & 2.878110178828852E9\\
   CANDELS\_GOODSS\_32 & 4.4105000495910645 & -0.6785370292415938 & 0.10190585887099374 & 1.018539814396081E-8 & 1.9023428175789387E-9 & 0.015229920938262585 & 0.002726856104238399 & 2.4843473871713986 & 0.09002920142052893 & 1.0898551818463362 & 0.0403862337281479 & 223.19913272814188 & 48.48587187087437 & 6.524372506377365E11 & 5.006973065914676E10 & 1.088774756894815E8 & 8355540.51717848 & 5.293865105835035E10 & 2.646932552917518E9 & 72.81458934042845 & 6.797772856448676 & 7.148919297141285E9 & 1.1564475989098332E9\\
%   CANDELS\_GOODSS\_37 & 4.519999980926514 & -0.8526933686190812 & 0.23096820607580118 & 2.09696291726624E-9 & 1.4860857010181376E-9 & 0.004187028346893696 & 0.0029527148790823997 & 3.222897370292023 & 0.4794138598520492 & 1.4435258993623492 & 0.20699668202932772 & 778.6442054794873 & 279.099532605016 & 1.8118853549635223E11 & 7.494639037263376E10 & 3.023639491680463E7 & 1.2506909726314228E7 & 5.915012688294465E9 & 2.957506344147233E8 & 15.143102372210073 & 6.35316875198729 & 7.2214449991093645E9 & 4.1245677055815525E9\\
%   CANDELS\_GOODSS\_38 & 5.5721001625061035 & -1.3342119670909967 & 0.14395279564668623 & 7.278994535891784E-9 & 2.2334057220767056E-9 & 0.008995188261691728 & 0.002785303608947198 & 1.385354617671701 & 0.10068467419277363 & 0.5502221834448126 & 0.05683989094685525 & 300.89753711688104 & 93.33306640355659 & 2.419225182261498E11 & 2.1538673145388878E10 & 4.037156534388456E7 & 3594332.4196748864 & 6.7975976655305275E10 & 3.3987988327652636E9 & 32.66906650470333 & 2.5705579882980225 & 4.488129005127889E9 & 1.3310361111998765E9\\
%   CANDELS\_GOODSS\_42 & 5.525199890136719 & -2.105111640907456 & 0.2265720196887971 & 2.8991324038464925E-9 & 1.8964826233085787E-9 & 0.0022799478181627694 & 0.001708556799887454 & 0.582517294330526 & 0.18539185942414013 & -0.028816814966306132 & 0.2083523495487733 & 579.6567239041378 & 285.2530860552559 & 4.799506810000665E10 & 1.8612241260016224E10 & 8009324.812716695 & 3105975.0854712655 & 4.676623693127884E10 & 2.338311846563942E9 & 10.184484448503719 & 1.3172005511427345 & 3.512942159865211E9 & 2.2526473360638976E9\\
%   CANDELS\_GOODSS\_47 & 5.57450008392334 & -2.0559536536171032 & 0.25094123798543355 & 2.259157829953222E-8 & 8.736662019642934E-9 & 0.019907373490339744 & 0.008147716719777107 & 1.0668687732489313 & 0.13888546199100538 & 0.3657442604404101 & 0.09048716435996125 & 102.81642167552644 & 44.345869531605125 & 1.0380813663519084E11 & 1.790468488558437E10 & 1.7323302527286205E7 & 2987899.436233211 & 4.408926070127181E10 & 2.2044630350635905E9 & 19.65908489342316 & 2.134764367268681 & 8.701952839581031E8 & 3.229847318054487E8\\
%   CANDELS\_GOODSS\_57 & 5.558499813079834 & -1.1003773836681623 & 0.13415852750636048 & 1.4806262511715873E-9 & 1.927000314193144E-10 & 0.0023935002452715134 & 3.473260225941418E-4 & 1.5416696102594343 & 0.0998240453819369 & 0.6637892679819224 & 0.05394042726200411 & 966.1165254241745 & 70.7463678143181 & 2.920238474275526E11 & 2.7936705161784348E10 & 4.873237896512469E7 & 4662023.718178637 & 6.310524562925344E10 & 3.155262281462672E9 & 30.145992138647408 & 2.138628295915079 & 2.036029829593629E10 & 2.2215680160457625E9\\
%   CANDELS\_GOODSS\_8 & 5.517399787902832 & -1.9707045003788612 & 0.15473480803867837 & 6.297670826729823E-9 & 2.7625281338215717E-9 & 0.0038070508534653177 & 0.002864599162714156 & 0.4460001257984469 & 0.2510023997116592 & -0.22974380727674248 & 0.32230972638205035 & 364.49477979475006 & 153.53687680502821 & 4.258574462239581E10 & 2.909405414361301E10 & 7106627.296818523 & 4855159.894125253 & 5.660542906692216E10 & 2.830271453346108E9 & 11.755871178573306 & 3.5849090392069503 & 1.8667014364543645E9 & 5.886157902280306E8\\
%   DEIMOS\_COSMOS\_206253 & 4.474999904632568 & -1.15944008390656 & 0.2697863076576818 & 1.0426246703507454E-9 & 7.99744217124201E-11 & 0.0017175755297459674 & 1.6172926457106384E-4 & 1.460225422389105 & 0.11091239052783547 & 0.6330243060071874 & 0.06197383580915735 & 1166.4210834054077 & 37.63323165077148 & 3.328179762624077E11 & 2.4643641345952126E10 & 5.554002485926858E7 & 4112483.551363021 & 7.749835520899283E10 & 5.307944955208108E9 & 33.71461639228857 & 1.6857308196144285 & 3.233629258067216E10 & 1.8809723648710403E9\\
%   DEIMOS\_COSMOS\_274035 & 4.479100227355957 & -2.1714885466119074 & 0.3293959274170321 & 1.6582036840003455E-8 & 4.1167514643682454E-9 & 0.014847546501397661 & 0.004014026294749582 & 0.9778216088954057 & 0.11645881454871744 & 0.2996054559586316 & 0.08059541096896196 & 139.98254377188104 & 40.920007509726766 & 1.7734478965779654E11 & 2.639519017213331E10 & 2.9594957991361104E7 & 4404778.6564556165 & 8.805294153801823E10 & 4.402647076900912E9 & 33.052240896831584 & 3.418794814370623 & 1.9932557873164573E9 & 4.4986173964975005E8\\
%   DEIMOS\_COSMOS\_308643 & 4.525300025939941 & -1.7365268395008358 & 0.10349143361274572 & 9.294764247654663E-9 & 1.6831235970899877E-9 & 0.009453210631199787 & 0.001874056785507657 & 1.0280471361959607 & 0.09004098602036363 & 0.3319280925922285 & 0.060097331480866115 & 242.4777152239212 & 49.01620779026929 & 3.80895571241315E11 & 4.579991714245029E10 & 6.356312159908242E7 & 7643002.235668144 & 1.7618090641205914E11 & 8.809045320602959E9 & 62.497732586065645 & 5.57179250445766 & 6.723971788938663E9 & 1.0598093324003758E9\\
%   DEIMOS\_COSMOS\_336830 & 5.714000225067139 & -2.4578762256419755 & 0.09420195133547855 & 9.034607729567948E-9 & 5.16249196570846E-9 & 0.003225814576040631 & 0.002911061331175661 & 0.26989268995827703 & 0.18458900454509566 & -0.48270726228245964 & 0.2842209827319804 & 269.32351192372937 & 171.85696828089755 & 1.3949291714896004E10 & 1.0444832386106834E10 & 2327831.018369249 & 1743013.5742364072 & 3.482560421920278E10 & 3.7249288296051517E9 & 6.51960601452188 & 1.7590562098174531 & 7.216257982275075E8 & 3.6348401687369204E8\\
%   DEIMOS\_COSMOS\_351640 & 5.7058000564575195 & -1.9377226217300454 & 0.21650281881772918 & 1.237647498063492E-8 & 4.240326196137238E-9 & 0.011200259058023524 & 0.0040360749176484865 & 0.9320069443246117 & 0.1238842290177489 & 0.2676418191099071 & 0.08891709727254794 & 185.53600279908562 & 69.85892055479827 & 1.708525673995731E11 & 2.3999336445472668E10 & 2.8511548406148884E7 & 4004963.186653623 & 9.153059170446782E10 & 5.820820167115671E9 & 31.505741401139826 & 2.6841043345490414 & 2.545615084297901E9 & 8.447637962522489E8\\
%   DEIMOS\_COSMOS\_372292 & 5.13640022277832 & -1.9057373607111363 & 0.40712467208007763 & 2.0756186679293666E-8 & 5.657964755093977E-9 & 0.019255300945928044 & 0.005339161032741591 & 1.122806653243444 & 0.1085875635670801 & 0.3985050665854552 & 0.06894574493308415 & 111.89543655914052 & 37.2323656613291 & 2.4119167081589206E11 & 2.2758875660112E10 & 4.02496029313073E7 & 3797957.4725104677 & 9.617506210998737E10 & 6.267718089320951E9 & 43.3869236609532 & 3.450395215787353 & 2.0903128465420825E9 & 5.450141108151314E8\\
%   DEIMOS\_COSMOS\_396844 & 4.542399883270264 & -1.0215453178764897 & 0.20069043392384597 & 2.3164068604079837E-8 & 6.179475699203282E-9 & 0.02787745954992331 & 0.007221666149297624 & 2.055552843927238 & 0.10150907824496261 & 0.8962935905311363 & 0.048724563376562106 & 100.5734119414018 & 33.69073424852219 & 7.176680582228765E11 & 5.1285457564091225E10 & 1.1976306761439717E8 & 8558418.688847488 & 9.103853730770421E10 & 4.551926865385212E9 & 99.51408626337977 & 9.527289609235874 & 4.296053856698238E9 & 1.0697120841535115E9\\
%   DEIMOS\_COSMOS\_400160 & 4.54040002822876 & -1.8250578796222117 & 0.09236417750238435 & 8.012087726721988E-9 & 1.4545480649936887E-9 & 0.007248865258267965 & 0.0016009960580552777 & 0.8262065312404206 & 0.10264850294542206 & 0.18850140036200733 & 0.07917022591900143 & 278.04491435654637 & 55.127714927633946 & 2.5212442374969284E11 & 4.04460715606405E10 & 4.207403974972239E7 & 6749562.764502214 & 1.6128272890700647E11 & 8.064136445350326E9 & 46.50395413376883 & 4.630207865743165 & 5.804224282101707E9 & 8.811135407652856E8\\
%   DEIMOS\_COSMOS\_403030 & 4.5594000816345215 & -1.2985310485345152 & 0.14849944400424298 & 1.2438985231779652E-8 & 2.4191161331320865E-9 & 0.014986150226013397 & 0.0029716574204547413 & 1.5369154311544786 & 0.11010990663045979 & 0.6316619756634151 & 0.05933163082674805 & 184.63086246213834 & 42.1342117197352 & 3.915251759469497E11 & 3.9533886390536835E10 & 6.5336969623233825E7 & 6597339.0547352005 & 9.108550609968886E10 & 4.554275304984444E9 & 54.23177987512019 & 5.057628047060258 & 4.359823479536459E9 & 7.440442649529337E8\\
%   DEIMOS\_COSMOS\_412589 & 4.434100151062012 & -2.34350815306745 & 0.11995014134531869 & 2.4019490591864583E-9 & 1.7978094820233706E-9 & 0.001408738586672627 & 0.0017285793336491745 & 0.3584958649964838 & 0.26424739722644863 & -0.3579884837218404 & 0.34316421854027007 & 681.7658421259082 & 306.57609329017396 & 4.5703906153270935E10 & 4.726759554608968E10 & 7626980.106137558 & 7887925.5896857595 & 7.288253893010063E10 & 3.644126946505031E9 & 13.004270532293006 & 4.582792959909972 & 5.414049262434217E9 & 3.5750395928093605E9\\
%   DEIMOS\_COSMOS\_416105 & 5.630899906158447 & -2.3075406947785555 & 0.15822151174141794 & 1.8539313730077767E-8 & 7.440619953514413E-9 & 0.00824185227921933 & 0.004618407402163207 & 0.395770380256314 & 0.1617375341517 & -0.25620001316432006 & 0.22865141495310215 & 125.953909912192 & 57.74094828564061 & 5.6315334827147865E10 & 2.264454926484066E10 & 9397794.949007718 & 3778878.9031773177 & 9.298688547036557E10 & 7.60387375079923E9 & 21.139503964404618 & 1.9784236598581209 & 1.140252777000497E9 & 4.4501591149893403E8\\
%   DEIMOS\_COSMOS\_417567 & 5.670000076293945 & -1.646569580189359 & 0.09330612434239574 & 2.362044352247477E-9 & 4.4171725932494514E-10 & 0.002480974070825937 & 5.593890040165293E-4 & 0.8241072001920278 & 0.10564762955716478 & 0.1976067467861111 & 0.08063975708049753 & 723.3513434830325 & 105.99395367907606 & 2.6178323690081406E11 & 3.889635754781891E10 & 4.368588394320231E7 & 6490949.465534836 & 1.6442385144312424E11 & 8.221192572156212E9 & 41.59172667476835 & 3.2777510407720194 & 1.760835973939015E10 & 2.986198490559388E9\\
%   DEIMOS\_COSMOS\_420065 & 5.7256999015808105 & -2.4478572162822463 & 0.10521420637231943 & 1.357711006578272E-8 & 8.328535164521283E-9 & 0.005034434841895232 & 0.004562273925561621 & 0.3075934332929092 & 0.20794969702475233 & -0.42399912912806237 & 0.3070849720079816 & 191.062632441417 & 132.16054158685878 & 1.8453761759295624E10 & 1.363316168209941E10 & 3079528.3306758855 & 2275075.845474258 & 3.939868836756673E10 & 3.384349453808616E9 & 8.305022591283091 & 2.637466597897766 & 6.116929560889074E8 & 3.2102873631502765E8\\
%   DEIMOS\_COSMOS\_421062 & 5.579999923706055 & -2.115672069608623 & 0.20858317493862438 & 2.3274498209586427E-9 & 5.988695945937867E-10 & 0.0010298662659624978 & 5.705225667136521E-4 & 0.2737894422800386 & 0.1276849185633859 & -0.44526087309204726 & 0.2346428055056955 & 735.0166986272179 & 159.21781564149367 & 5.26981612027065E10 & 2.69641773818107E10 & 8794167.959630892 & 4499730.149535943 & 1.286067515189691E11 & 7.485924390390487E9 & 19.874410221597145 & 2.8885949538972207 & 8.539135857034789E9 & 1.8130854723392317E9\\
%   DEIMOS\_COSMOS\_422677 & 4.4380998611450195 & -1.2079021154450968 & 0.15395633209932366 & 5.752781140105973E-9 & 1.0672006940466796E-9 & 0.007814985397533147 & 0.001496333928172553 & 1.5511104659901118 & 0.10695086920815954 & 0.643949366308706 & 0.05679351208782355 & 370.0993600470184 & 69.59824741824174 & 4.366796306432359E11 & 4.293700607129283E10 & 7.287225832519126E7 & 7165245.132979096 & 9.878090125527965E10 & 4.939045062763983E9 & 53.64285817634666 & 4.62121085431554 & 9.324682596104898E9 & 1.5319938034296598E9\\
%   DEIMOS\_COSMOS\_430951 & 5.6880998611450195 & -2.617968723182169 & 0.19956020207035163 & 7.599947392093801E-8 & 2.872079812143908E-8 & 0.06369699029166952 & 0.02479995156669316 & 1.9391003475873965 & 0.19464216708016135 & 0.8616459957728749 & 0.0923748170718245 & 29.504763198676415 & 14.089496980785174 & 3.0623298735448254E11 & 4.182648549209247E10 & 5.110357295420265E7 & 6979923.590951308 & 4.2068855629728035E10 & 5.278827337327574E9 & 60.973754681586875 & 6.061245687210952 & 8.022917993487383E8 & 2.9251486890055376E8\\
%   DEIMOS\_COSMOS\_431067 & 4.429999828338623 & -2.262704626019596 & 0.15702551648514945 & 2.6123508842705604E-9 & 1.1105880549296852E-9 & 0.0015210702120644949 & 0.001381740009084695 & 0.366905316513529 & 0.252577857137925 & -0.34166485901618787 & 0.33154686834545644 & 703.8832948184742 & 219.34358022863995 & 2.6169760931569603E10 & 2.280196350553254E10 & 4367159.457620507 & 3805147.8894244335 & 4.264218575689523E10 & 2.917122502472913E9 & 7.50034599348379 & 2.540451805766266 & 2.8711097114268746E9 & 7.376571171430348E8\\
%   DEIMOS\_COSMOS\_432340 & 4.4045000076293945 & -1.8449521217962732 & 0.15577108521852837 & 2.837306753430686E-9 & 5.897702875585285E-10 & 0.003079917413030764 & 7.496762189257638E-4 & 0.8938237034213852 & 0.11198576419623514 & 0.2506121935881679 & 0.08100794247019365 & 638.725177992031 & 109.49707887375375 & 2.927782830735786E11 & 4.63206449587653E10 & 4.885827773719692E7 & 7729900.293843481 & 1.6243336954031415E11 & 8.121668477015709E9 & 45.00962291983259 & 4.267642654990247 & 1.5863502550582481E10 & 2.9343960219753385E9\\
%   DEIMOS\_COSMOS\_434239 & 4.48829984664917 & -0.6697443298730388 & 0.2236282507279446 & 1.6860173192610915E-9 & 2.929415557304283E-10 & 0.0027655025370088883 & 4.844310877040298E-4 & 1.6505097698958786 & 0.0922061737756363 & 0.7166148206472688 & 0.04621355448836697 & 894.7379618462644 & 116.024853685531 & 5.350677758555741E11 & 4.2136019962173134E10 & 8.929108309036006E7 & 7031578.109003922 & 1.0258432907529149E11 & 5.129216453764574E9 & 54.43723537811544 & 4.111855437475158 & 3.228747104565505E10 & 5.052022678548604E9\\
%   DEIMOS\_COSMOS\_442844 & 4.491199970245361 & -2.371497012530034 & 0.09388448747878685 & 4.2356491826540545E-9 & 1.7544813091184994E-9 & 0.001884710737771221 & 0.0016658706798933038 & 0.29015055799533956 & 0.19407872560324915 & -0.4513674436752094 & 0.2928046739267928 & 489.5935750487638 & 174.20359673008804 & 2.3594207579441837E10 & 1.9522068652714607E10 & 3937356.05934864 & 3257805.333871882 & 5.216472038675708E10 & 2.608236019337854E9 & 8.848710117882533 & 2.42214012943237 & 2.0891036382616413E9 & 6.494705276679622E8\\
%   DEIMOS\_COSMOS\_454608 & 4.583399772644043 & -1.189441582801063 & 0.13591867378159248 & 1.3255127668638608E-8 & 3.4383256405723317E-9 & 0.015556825947127675 & 0.003991575781807542 & 1.502945822363835 & 0.08685194016646333 & 0.6157815384378502 & 0.047276424921636556 & 173.90428986298818 & 52.55321484059258 & 4.3315380768407025E11 & 3.0999013791577644E10 & 7.228387575943992E7 & 5173055.902604197 & 1.0480112171700421E11 & 5.240056085850211E9 & 61.58917023509488 & 4.993823202387003 & 4.646441118844426E9 & 1.1448722032508066E9\\
%   DEIMOS\_COSMOS\_460378 & 5.389999866485596 & -1.461590816969162 & 0.21277213264813277 & 1.3582724148133732E-9 & 1.8135560595771488E-10 & 0.0015750224903870388 & 3.1598863382996585E-4 & 0.8632119465726279 & 0.12536540544125363 & 0.24213859444648542 & 0.09413734101788118 & 1014.7524344122652 & 72.01912959723451 & 2.1331262127781155E11 & 3.6525191439832565E10 & 3.559720067291202E7 & 6095253.818136323 & 1.2049816688430434E11 & 6.024908344215218E9 & 30.69841606306902 & 2.5493121176624642 & 2.2601074518094357E10 & 2.362989726022478E9\\
%   DEIMOS\_COSMOS\_488399 & 5.670400142669678 & -1.6429269760218148 & 0.29852849960342265 & 3.865576229697449E-9 & 1.147750579756469E-9 & 0.005697627254691807 & 0.001671585686179829 & 1.673226648761272 & 0.12518859730475185 & 0.7120264179006677 & 0.06456173854387326 & 508.2400488664425 & 141.58165345986913 & 5.106977201569205E11 & 4.369267865427476E10 & 8.522425498652643E7 & 7291350.322715581 & 9.912501940757292E10 & 7.80125909643044E9 & 57.820710190949626 & 5.60746568305948 & 1.4957850202704483E10 & 4.1976379870937386E9\\
%   DEIMOS\_COSMOS\_493583 & 4.513400077819824 & -1.5697456400110812 & 0.1471610848848542 & 1.8221026137701766E-8 & 3.3260803281533373E-9 & 0.019712962554511694 & 0.003693209314119954 & 1.4087125294809413 & 0.09751532558985068 & 0.5635248222390832 & 0.05488407031299024 & 126.71238881415552 & 27.916638862612242 & 3.588576052371045E11 & 3.43359244489201E10 & 5.988546814578296E7 & 5729913.1461439375 & 9.770497943165794E10 & 4.885248971582897E9 & 55.353155434421566 & 4.754019313607755 & 3.037872566347315E9 & 4.893225467515784E8\\
%   DEIMOS\_COSMOS\_494057 & 5.5447998046875 & -2.1268652065556517 & 0.2641998157462262 & 7.223049084277442E-9 & 2.2127845168609742E-9 & 0.0064722463513612735 & 0.0020383593448193653 & 0.8096478781365046 & 0.08336527413292745 & 0.18174541960142124 & 0.06432201591482281 & 304.52522595575067 & 98.0957474702956 & 3.3181268211635187E11 & 3.805235692974031E10 & 5.537226330236639E7 & 6350104.262893604 & 2.1717483210138162E11 & 1.085874160506908E10 & 61.795635398891484 & 5.46321371254617 & 8.555339258790765E9 & 2.5094238042439346E9\\
%   DEIMOS\_COSMOS\_494763 & 5.233699798583984 & -2.051448225400101 & 0.5308575688725958 & 2.863741779782335E-8 & 9.076418353129606E-9 & 0.02971969955600261 & 0.00917746444610893 & 1.6186875836171521 & 0.13393689495849478 & 0.682657092588313 & 0.06945186100230771 & 81.75250845521946 & 33.48522345363404 & 3.074539171205554E11 & 2.027287455012804E10 & 5.130731936934713E7 & 3383098.380464862 & 6.404709924100165E10 & 6.132410186178545E9 & 49.43889618054991 & 4.804116873382482 & 1.7263740931386495E9 & 5.208103851958316E8\\
%   DEIMOS\_COSMOS\_510660 & 4.547999858856201 & -1.5901623712670205 & 0.14716858640243205 & 4.039540849033996E-8 & 1.1189192567157595E-8 & 0.03556886404516563 & 0.010157054454217884 & 1.3348963938785499 & 0.10946311276688872 & 0.5322953433113901 & 0.06248486368118972 & 56.25636100970285 & 18.853134460070592 & 2.814650203871017E11 & 3.0810308329926205E10 & 4.6970342181844115E7 & 5141565.0974833295 & 8.225922393711362E10 & 4.1129611968556814E9 & 53.34401899811371 & 4.51446536226587 & 1.3205465915976624E9 & 3.4828971233299553E8\\
%   DEIMOS\_COSMOS\_519281 & 5.575900077819824 & -2.359808562557726 & 0.22766515225618392 & 2.762734101137523E-8 & 1.2664148781262928E-8 & 0.022880190606358538 & 0.010780832437848565 & 1.0626444540395004 & 0.14353296412020652 & 0.36576407745862227 & 0.0936545238249083 & 85.32842520302296 & 46.92526744912347 & 2.8976629735488007E11 & 4.216503683510208E10 & 4.835564334355351E7 & 7036420.389045133 & 1.2359714267781554E11 & 7.880521138855097E9 & 58.388405562737084 & 5.6249860059101895 & 2.1134283439979384E9 & 9.47141877821944E8\\
%   DEIMOS\_COSMOS\_536534 & 5.688600063323975 & -1.093142448135695 & 0.2434660299382998 & 1.4425100205760931E-9 & 1.1930743026132045E-10 & 0.0015194276006115259 & 1.506415666295413E-4 & 0.7612348413130259 & 0.05915436112622012 & 0.1616487285692141 & 0.04802757716502753 & 980.7325752058216 & 42.23382603702602 & 2.0542927510930417E11 & 1.5219537025121778E10 & 3.428164300054668E7 & 2539807.1168348095 & 1.4138193382168817E11 & 7.069096691084407E9 & 32.54621248830679 & 1.6273106244153397 & 2.256220894417694E10 & 1.4864795891199925E9\\
%   DEIMOS\_COSMOS\_539609 & 5.18179988861084 & -2.3850847408020535 & 0.223196134091524 & 2.7325544871454104E-8 & 6.336426800249074E-9 & 0.018475508886324495 & 0.004877110854270705 & 0.7369979275283468 & 0.09697369002538014 & 0.12803975645037094 & 0.08084336161461932 & 84.17382981030968 & 23.47190582740647 & 2.282757877069188E11 & 3.495542811576891E10 & 3.80942251569223E7 & 5833294.728604081 & 1.6813257319771048E11 & 8.406628659885526E9 & 56.34190999952701 & 4.890946578868557 & 2.061876909118293E9 & 4.4335481856086165E8\\
%   DEIMOS\_COSMOS\_549131 & 5.549300193786621 & -2.5128888666346865 & 0.05829519041907302 & 1.3916143252447113E-8 & 5.598893901943371E-9 & 0.003526593900047466 & 0.0022442320549558845 & 0.19457644390149334 & 0.09299783967924714 & -0.5990600123197249 & 0.19778527245451077 & 172.76169208733128 & 83.72430904477652 & 3.4687531335819954E10 & 1.8081212424621113E10 & 5788588.62833517 & 3017358.0130100735 & 1.2418248358448524E11 & 6.209124179224262E9 & 22.84210512027323 & 3.8636363856616907 & 1.641410605359823E9 & 5.991934846254493E8\\
%   DEIMOS\_COSMOS\_550156 & 4.419000148773193 & -1.9303005739836214 & 0.21442690889435806 & 5.232295201600184E-9 & 2.616429993292578E-9 & 0.0036913349667792666 & 0.00305221282581208 & 0.5166997109640459 & 0.3149982732234716 & -0.16600381818088825 & 0.36293176493292423 & 446.7538515585786 & 195.03617056856584 & 8.101958097023395E10 & 6.3290926493363716E10 & 1.352039211255362E7 & 1.0561868292943543E7 & 8.609296852789482E10 & 4.304648426394741E9 & 19.164525411789196 & 8.05369995771092 & 3.662737799260283E9 & 9.926784742846781E8\\
%   DEIMOS\_COSMOS\_552206 & 5.5015997886657715 & -1.1266694229692646 & 0.3589958628425009 & 1.800840532184135E-9 & 3.4313338053282875E-10 & 0.0027195661839588426 & 5.419590512177311E-4 & 1.4248791423564668 & 0.11692353134090111 & 0.5935961997261374 & 0.0645085691326111 & 859.4011876079603 & 122.92674976329667 & 7.526231837823248E11 & 7.589827084262137E10 & 1.2559631185298339E8 & 1.2665757711509842E7 & 1.9133566598920633E11 & 1.1293932968193563E10 & 83.16728249225581 & 6.8391480482089415 & 4.618248035065439E10 & 7.937931458502053E9\\
%   DEIMOS\_COSMOS\_567070 & 4.561999797821045 & -2.2093269967758657 & 0.19532470024606408 & 4.2433636058428875E-9 & 2.115520926871904E-9 & 0.0027587655975872417 & 0.0025369481019304322 & 0.4457378255360268 & 0.3054481020482944 & -0.2543463486344418 & 0.36723830643636474 & 518.5844149097601 & 201.49615668501892 & 7.329488114959586E10 & 6.463679198392591E10 & 1.2231309038115475E7 & 1.078646374191088E7 & 9.254867604554677E10 & 4.627433802277339E9 & 18.813447459816334 & 7.995049208207783 & 4.433616632312916E9 & 1.1557657946280093E9\\
%   DEIMOS\_COSMOS\_586681 & 5.866099834442139 & -2.3403816697948785 & 0.10129599333117063 & 2.889848485899513E-9 & 1.087024631819922E-9 & 0.001521384472062572 & 0.0012528836728789427 & 0.3375065740179698 & 0.22203440179639225 & -0.37509558287746897 & 0.31289697201504724 & 649.6772121430904 & 194.9680508845198 & 5.842742948658018E10 & 4.574234770875982E10 & 9750257.250495633 & 7633395.159108731 & 1.0802275208138873E11 & 8.740756808472752E9 & 18.52047701937942 & 5.113548480349459 & 6.40880555148365E9 & 1.6371756633618288E9\\
%   DEIMOS\_COSMOS\_592644 & 4.526700019836426 & -2.351521713051494 & 0.10836996204733183 & 5.576556698034735E-9 & 1.6117166471155024E-9 & 0.00225724825110023 & 0.0016808645813740754 & 0.2709512958398221 & 0.16248931795530458 & -0.4769302133384829 & 0.2684940680098559 & 390.557699165204 & 105.92381941656438 & 3.979120252197292E10 & 2.8650245954369644E10 & 6640279.476695412 & 4781098.035627896 & 9.738066074154736E10 & 4.869033037077369E9 & 16.404883678407653 & 3.5732834850709505 & 2.9417586096074286E9 & 5.58823496939894E8\\
%   DEIMOS\_COSMOS\_627939 & 4.53410005569458 & -1.3184890020869506 & 0.2525273166718043 & 4.950692192157437E-9 & 9.961117435199032E-10 & 0.006700707589548976 & 0.0013507290781700873 & 1.4797064931131112 & 0.08665189810710523 & 0.6059521269168769 & 0.046589801290044745 & 418.9293433551034 & 85.50551977973446 & 3.8748208639792224E11 & 3.047922296722787E10 & 6.466226660213203E7 & 5086314.207848971 & 9.584254761378337E10 & 4.79212738068917E9 & 47.774503530592824 & 3.711960353125836 & 9.650065420402033E9 & 1.7910473403254356E9\\
%   DEIMOS\_COSMOS\_628063 & 4.532700061798096 & -1.6698914759212593 & 0.19432179840056416 & 1.946853552728873E-9 & 3.628624878334323E-10 & 0.0023279244830481374 & 5.435152755102537E-4 & 0.9686407204208561 & 0.14356371971276852 & 0.30875824974687094 & 0.09926851814325413 & 821.7364686480357 & 117.63427280111421 & 1.332416399639845E11 & 2.3291398983534668E10 & 2.2235109049682904E7 & 3886823.942264242 & 6.455205189970778E10 & 3.905517751947688E9 & 18.59532015059526 & 1.931127130987434 & 9.551473517117146E9 & 1.478294237084895E9\\
%   DEIMOS\_COSMOS\_629750 & 5.118100166320801 & -2.283444199482142 & 0.17966581761352055 & 4.3685619723569394E-9 & 2.2076394842448996E-9 & 0.0027301953444181905 & 0.002558780788027652 & 0.4294769420375848 & 0.30338910639320343 & -0.2756551580580673 & 0.36762543827338573 & 508.44654479480903 & 211.28134187762709 & 5.0254028061951546E10 & 4.499122014768276E10 & 8386295.713902605 & 7508048.433901167 & 6.6930656485116905E10 & 6.7408165010160265E9 & 13.418839285473222 & 5.669709736227626 & 3.0716833984235435E9 & 8.515465494136025E8\\
%   DEIMOS\_COSMOS\_630594 & 4.440299987792969 & -1.4474870055520621 & 0.26433593440545705 & 1.497960587518196E-8 & 3.3891102108133832E-9 & 0.01880974029153314 & 0.004141222872544388 & 1.8331019473577075 & 0.10124496354542639 & 0.786534675173715 & 0.050708430414554494 & 154.63409453769407 & 43.03191768860648 & 4.413190517168719E11 & 3.0215931254153767E10 & 7.364647600614727E7 & 5042376.592298284 & 7.21327155091681E10 & 3.9489012691357927E9 & 58.6502082202971 & 5.046640754084556 & 3.915337206399276E9 & 8.192725113840065E8\\
%   DEIMOS\_COSMOS\_665509 & 4.525599956512451 & -2.17225247751762 & 0.2570547408500491 & 2.15190636912097E-8 & 5.374318264369089E-9 & 0.02128973801850266 & 0.005227954675142509 & 1.2726586306513987 & 0.08202348268376726 & 0.48725001067891527 & 0.04887972404070617 & 108.32018527957396 & 34.3360474162815 & 3.878281600478818E11 & 3.22837015384226E10 & 6.472001870836663E7 & 5387442.127162901 & 1.2599656897906308E11 & 6.299828448953154E9 & 65.41716029907148 & 6.206697826712733 & 3.0399631339812274E9 & 7.023006432940378E8\\
%   DEIMOS\_COSMOS\_680104 & 4.5295000076293945 & -1.7241320352560554 & 0.31437549640425466 & 5.8069215008020047E-8 & 1.3126727802045952E-8 & 0.04646553311186415 & 0.010791430793286969 & 1.334989004337206 & 0.10977954063694453 & 0.5317675234493001 & 0.0631050193349744 & 38.49401084577804 & 10.938087353372412 & 2.6922927203297028E11 & 3.1252121044861576E10 & 4.492846398947026E7 & 5215293.955059535 & 7.869831568986328E10 & 3.9349157844931636E9 & 56.14829876380957 & 5.790738882804715 & 9.66920230556842E8 & 1.945015145491336E8\\
%   DEIMOS\_COSMOS\_683613 & 5.541999816894531 & -1.9099271523067591 & 0.28133955770432223 & 6.165222890503662E-9 & 1.8027738110375134E-9 & 0.008353085635817206 & 0.0024309316347075846 & 1.5991714904886178 & 0.13641904678386949 & 0.6701389544097042 & 0.0718181945741187 & 349.7253647750048 & 106.38400499601009 & 5.3725097021269745E11 & 5.032701126444972E10 & 8.965541037288532E7 & 8398475.010605805 & 1.1480806453792822E11 & 9.714457779689173E9 & 66.1726231942713 & 6.4784707246505295 & 1.0733208574859064E10 & 2.9573600098656683E9\\
%   DEIMOS\_COSMOS\_709575 & 4.412099838256836 & -1.6634274433517835 & 0.25446762761498193 & 1.0065759399377442E-8 & 2.181957674232494E-9 & 0.012176902401225967 & 0.002716179519021234 & 1.4492669294997051 & 0.11919434481993571 & 0.5864518668816617 & 0.0656424903315406 & 225.5900353091065 & 55.35785076131503 & 2.8479941196816797E11 & 3.041229084106246E10 & 4.7526779046771586E7 & 5075144.703145956 & 7.35103402783695E10 & 3.675517013918475E9 & 39.28693087529481 & 3.65107221277801 & 3.9030270162949324E9 & 7.643630355897144E8\\
%   DEIMOS\_COSMOS\_722679 & 5.716800212860107 & -2.7550662761501568 & 0.09962463394948656 & 1.5785845467335778E-7 & 2.5257610062346735E-8 & 0.05446632682541925 & 0.023126172298076033 & 0.6677250797709643 & 0.3019981542363336 & 0.05633390392782945 & 0.2849879446052443 & 13.117766456297442 & 1.7571922296177014 & 5.651614061365936E10 & 2.282072042762006E10 & 9431305.033108285 & 3808278.0085686077 & 4.572600510976665E10 & 8.608312556794716E9 & 27.33452620830513 & 2.500217947066695 & 1.731584555598621E8 & 2.2732109215127412E7\\
%   DEIMOS\_COSMOS\_733857 & 4.54449987411499 & -1.6475478354922082 & 0.12954163577416267 & 1.45847907280026E-8 & 3.0746134763957005E-9 & 0.014844986605082674 & 0.0033189979551065127 & 1.16639374871143 & 0.10420651868594151 & 0.42067020493931334 & 0.06472326795381693 & 158.33567043662129 & 38.93375802126171 & 3.287631392467076E11 & 4.039329746678447E10 & 5.486336144348387E7 & 6740755.92504719 & 1.239590422517261E11 & 6.197952112586308E9 & 53.901742492244075 & 5.267405078740552 & 3.695750148046585E9 & 6.903342446385323E8\\
%   DEIMOS\_COSMOS\_742174 & 5.636000156402588 & -2.320944979772318 & 0.20770081158763865 & 9.38442449740357E-9 & 2.8899829960086096E-9 & 0.007943574442900033 & 0.002876348696099894 & 0.7866617529364027 & 0.16742558040014438 & 0.1579162017481813 & 0.13584568410281303 & 240.96599035574937 & 79.99564011920411 & 1.1064443471779893E11 & 2.3928323999313232E10 & 1.846413082543697E7 & 3993112.7659843303 & 7.528575165160284E10 & 6.328541017756107E9 & 21.813258362092714 & 2.2343013298432397 & 2.3244108755020494E9 & 6.750596348569508E8\\
%   DEIMOS\_COSMOS\_761315 & 4.584700107574463 & -2.115708431316073 & 0.3005496233965986 & 8.404787846959469E-9 & 6.9670628644956866E-9 & 0.006456122484359229 & 0.0065005182274769 & 0.675728883581072 & 0.465174293986443 & -0.042928489347009297 & 0.45673741791932604 & 371.0451324184284 & 253.9301122076845 & 7.079668095259615E10 & 6.377887545171533E10 & 1.1814414185851255E7 & 1.0643296278238233E7 & 4.874382352001875E10 & 3.3393355436953473E9 & 15.380384279999216 & 10.710252878703017 & 1.8299550875116084E9 & 8.229239843347336E8\\
%   DEIMOS\_COSMOS\_773957 & 5.677299976348877 & -1.510970074483927 & 0.37396479991891096 & 3.4063150389468706E-9 & 9.410679738248104E-10 & 0.0041763293294119095 & 0.0011600339647404464 & 1.1383555777549674 & 0.10900360954895061 & 0.4109597339642463 & 0.06901633380508788 & 557.2901074889296 & 139.19565822107896 & 2.3641832605093616E11 & 1.917115153201944E10 & 3.945303632188087E7 & 3199244.958540514 & 9.191971351810316E10 & 8.430553785694496E9 & 32.17884902153155 & 2.4398090358248123 & 9.446821169976185E9 & 2.5096785432393847E9\\
%   DEIMOS\_COSMOS\_787780 & 4.510900020599365 & -1.7407812468038224 & 0.33232798286255927 & 2.1758143769553333E-9 & 1.1571992585627525E-9 & 0.0028192355944841943 & 0.001872778787512275 & 1.1112052856855574 & 0.4858337761598511 & 0.36200419649607707 & 0.33269429646131016 & 827.2818085683318 & 274.7814100544978 & 1.1059094738305293E11 & 6.886340574081725E10 & 1.845520496171167E7 & 1.1491792930449624E7 & 3.975530333606855E10 & 6.164136591366431E9 & 14.243258124263436 & 6.820755814071434 & 6.54617336621994E9 & 1.5146773684354033E9\\
%   DEIMOS\_COSMOS\_803480 & 4.5416998863220215 & -2.3172562331853697 & 0.17267229192105335 & 1.4066997370544299E-8 & 3.7695460780505714E-9 & 0.008418277402595131 & 0.003039417935046507 & 0.5274806646234644 & 0.12713650890464906 & -0.0781710881385953 & 0.14534453122131374 & 164.8360132676666 & 51.11003779204858 & 6.96787522308356E10 & 1.8558480544337997E10 & 1.1627856387216853E7 & 3097003.6004608925 & 8.016583668106638E10 & 4.008291834053319E9 & 19.43022514007702 & 2.16280707785411 & 1.3812631529144304E9 & 3.3669451196837837E8\\
%   DEIMOS\_COSMOS\_814483 & 4.580999851226807 & -1.6407769332404405 & 0.25132565851097577 & 1.0016093868187173E-8 & 1.8621319837652453E-9 & 0.011665866953416983 & 0.0022372070446881457 & 1.3364103531432177 & 0.0935210767164464 & 0.5196424334901764 & 0.05374469801324496 & 226.341487685092 & 48.27078717104114 & 5.159723814504612E11 & 5.0960184748470314E10 & 8.610448033570199E7 & 8504137.785909163 & 1.553199132452128E11 & 7.765995662260641E9 & 73.92768672552519 & 6.419985335334581 & 7.3808899655315895E9 & 1.2133109968256114E9\\
%   DEIMOS\_COSMOS\_818760 & 4.561299800872803 & -0.7748529833838228 & 0.2018656566088453 & 3.956265616661666E-9 & 7.821729257566832E-10 & 0.006781577289155795 & 0.001301064244695771 & 2.4627021892989536 & 0.10130858871416377 & 1.0940770786528622 & 0.04437201468253893 & 501.1143312280943 & 95.31931734842341 & 2.20245573168505E12 & 1.717769263910685E11 & 3.6754158372978157E8 & 2.8665803659855697E7 & 1.7703254239455115E11 & 8.85162711972756E9 & 214.41798395908606 & 19.60804979404104 & 5.419706479162386E10 & 9.499883273335072E9\\
%   DEIMOS\_COSMOS\_834764 & 4.505799770355225 & -2.0297832550855683 & 0.33536445191230724 & 8.061996370510702E-9 & 1.553935128223129E-9 & 0.00935591385940829 & 0.0018884198399189212 & 1.249070752040101 & 0.09548325975744752 & 0.46989310102570614 & 0.056726791937932765 & 276.18768681293926 & 58.649034493107536 & 3.9761980472007275E11 & 4.306309095713721E10 & 6.63540295710426E7 & 7186285.936642459 & 1.340698888687605E11 & 6.703494443438025E9 & 57.17730556407 & 5.1589267094958595 & 7.092201848814278E9 & 1.2079870967113135E9\\
%   DEIMOS\_COSMOS\_838532 & 4.526299953460693 & -2.1002120948010337 & 0.2605960802305365 & 1.3122702789181337E-8 & 7.842684525862301E-9 & 0.008018927380966278 & 0.006781395283105695 & 0.531419808883017 & 0.3273285027705466 & -0.15270772822429862 & 0.3792346480824618 & 216.2632571005948 & 132.47003443881852 & 7.112270561325809E10 & 5.421674970932315E10 & 1.1868820555246467E7 & 9047587.093884597 & 7.305294035891428E10 & 3.652647017945714E9 & 19.422922444006176 & 9.174366630167032 & 1.4801007655236151E9 & 5.419361641477193E8\\
%   DEIMOS\_COSMOS\_842313 & 4.553699970245361 & -1.6667289096089195 & 0.06193913008783693 & 1.012569750653222E-9 & 8.210515505383929E-11 & 0.0010281057889661562 & 1.469705726113742E-4 & 0.6795529846719178 & 0.0703989107544317 & 0.10468357979335048 & 0.062479258828859734 & 1183.8069098199117 & 20.903153774240323 & 4.483386981260224E11 & 5.794382511096867E10 & 7.481790112099774E7 & 9669554.2808269 & 3.4958679770426575E11 & 1.747933988521329E10 & 73.68730367588657 & 3.9287955649526105 & 7.277257060893823E10 & 4.445809034462802E9\\
%   DEIMOS\_COSMOS\_843045 & 5.847300052642822 & -1.848283674407846 & 0.21126805942647955 & 4.6275760210624774E-9 & 1.2404965887265967E-9 & 0.004169680810232588 & 0.0014072272705178133 & 0.7485304960836165 & 0.17296433334978056 & 0.1247381757142773 & 0.1458488853557977 & 441.1252896154283 & 110.58082429419713 & 1.7877535834330115E11 & 4.013160528849492E10 & 2.9833688546868037E7 & 6697085.2367902 & 1.3122755006800171E11 & 1.3249138752453356E10 & 33.109887308528016 & 3.0257531635970962 & 7.154909429435173E9 & 1.803097090569292E9\\
%   DEIMOS\_COSMOS\_845652 & 5.30709981918335 & -1.6281958368488127 & 0.07408274551710058 & 1.2008136124953486E-9 & 8.491034483365763E-11 & 9.243562355289418E-4 & 1.0956169227288935E-4 & 0.4889225023834529 & 0.04988086239182746 & -0.0893173969426323 & 0.05707251889022448 & 1084.607727251318 & 24.0329246499747 & 2.3567007566263837E11 & 2.5326347237041386E10 & 3.932816973374247E7 & 4226412.199654453 & 2.879853338136883E11 & 1.4399266690684416E10 & 51.09047762714732 & 2.5545238813573663 & 4.254655101800424E10 & 2.1273275509002123E9\\
%   DEIMOS\_COSMOS\_848185 & 5.293099880218506 & -1.1742761704435491 & 0.17332191573233116 & 2.221782224402389E-9 & 4.0738526966746217E-10 & 0.0028103555492929085 & 5.518309373448955E-4 & 1.0885931373530295 & 0.08754023852161374 & 0.38809805644326023 & 0.05491542284266359 & 753.5733460041997 & 111.080020524886 & 6.476432902153859E11 & 6.850731824368261E10 & 1.0807746877873164E8 & 1.1432369732625298E7 & 2.638082602091418E11 & 1.3190413010457092E10 & 85.44278287187043 & 6.757150465460734 & 3.845686671422204E10 & 6.361851945070114E9\\
%   DEIMOS\_COSMOS\_859732 & 4.531799793243408 & -2.3440917859242725 & 0.2919793421040324 & 1.4010319862115153E-8 & 3.781775367234734E-9 & 0.018004415915235935 & 0.004812975180069098 & 1.9023844455425516 & 0.15291028235777648 & 0.8198420263614341 & 0.07488518978764402 & 165.06439462904711 & 52.644233371351795 & 3.57209362075123E11 & 2.6625949665093227E10 & 5.9610412491582386E7 & 4443287.357576378 & 5.425260872599718E10 & 5.475525261976857E9 & 46.38645041592007 & 3.8687675113052413 & 3.3108773298853908E9 & 8.499673020989124E8\\
%   DEIMOS\_COSMOS\_869970 & 5.2006001472473145 & -2.4365933672788165 & 0.08389852140464332 & 8.767748899101732E-9 & 3.1913045165405865E-9 & 0.0030996490328032145 & 0.002367493809450628 & 0.2535254524024304 & 0.15442963266304682 & -0.5046267053463499 & 0.26140988332965587 & 269.46675912888895 & 109.8175567309593 & 2.7147919136269535E10 & 1.9357978600255142E10 & 4530392.620730958 & 3230422.3009747285 & 7.192475712543356E10 & 5.792635880085943E9 & 12.81478789777366 & 3.074213101393542 & 1.4615824478146899E9 & 4.00092201765791E8\\
%   DEIMOS\_COSMOS\_873321 & 5.154200077056885 & -1.2892388147909064 & 0.19916908077479117 & 4.9649202099867405E-9 & 9.43645217504726E-10 & 0.005727846766997085 & 0.0011295757980727132 & 1.1018116235251394 & 0.07958761243532932 & 0.3841088529135628 & 0.05059253773529024 & 417.4907481720034 & 79.68572902451416 & 4.2837582214922107E11 & 3.740573508196621E10 & 7.14865347072441E7 & 6242197.250468277 & 1.7644813707634735E11 & 8.82240685381737E9 & 61.96481074789468 & 4.318741184946432 & 1.2480524988751062E10 & 2.2068353876237826E9\\
%   DEIMOS\_COSMOS\_873756 & 4.5457000732421875 & -1.4378127515872585 & 0.2837954379715908 & 2.4311625007731226E-8 & 5.702849409218303E-9 & 0.03352270631459211 & 0.0075288822633688985 & 3.591010437121527 & 0.12245454005394754 & 1.5737699657714994 & 0.05172133533260241 & 95.29100876672872 & 28.41448073824668 & 2.0640977444553093E12 & 1.0320488722276547E11 & 3.444526684719128E8 & 1.722263342359564E7 & 5.519742267312048E10 & 4.057640150901105E9 & 249.8069228126817 & 21.0247227209696 & 1.0275204669915802E10 & 2.249798348493254E9\\
%   DEIMOS\_COSMOS\_880016 & 4.541500091552734 & -1.1185560918155997 & 0.29178408767829844 & 1.5338130983811963E-8 & 3.926319698534465E-9 & 0.019324892142227944 & 0.004836378005032982 & 1.8790170718084935 & 0.11388941823140425 & 0.8091595069764468 & 0.05616260848215668 & 151.2010814893952 & 46.85388265699008 & 4.1264251201638776E11 & 2.5969022843689327E10 & 6.886099012065245E7 & 4333660.670937536 & 6.4111723490854675E10 & 4.528756073078243E9 & 54.65483990141334 & 4.525176843290523 & 3.563331148957893E9 & 8.631269754809865E8\\
%   DEIMOS\_COSMOS\_881725 & 4.577700138092041 & -0.8548539264834502 & 0.182103025562111 & 7.18076920130682E-9 & 1.2881402584349414E-9 & 0.01050827337704589 & 0.0018694798053642526 & 1.9888410937577814 & 0.10954722728574176 & 0.864410355836976 & 0.05278766963984122 & 305.9588474696679 & 60.00040906168504 & 6.46179230875972E11 & 5.259560589511155E10 & 1.0783314936720328E8 & 8777053.726808382 & 8.81631977111399E10 & 4.408159885556994E9 & 73.68717296100755 & 6.232824639944176 & 1.026173810844628E10 & 1.6233429228305519E9\\
%   DEIMOS\_COSMOS\_920848 & 4.552800178527832 & -2.2321025995819075 & 0.15333296915869338 & 2.2087507786361144E-9 & 9.158002858109853E-10 & 0.0013706216160011076 & 0.0012541823331297629 & 0.3836746561457781 & 0.26501436186011657 & -0.31861496366925535 & 0.33804301145596216 & 786.7666630612082 & 218.74255424466406 & 3.4540804380747635E10 & 3.0677072203405373E10 & 5764103.115792375 & 5119330.908506455 & 5.262275398051022E10 & 2.8551939127394605E9 & 9.288827125235542 & 3.2629532641234174 & 4.2054663727029076E9 & 9.26321008539777E8\\
%   DEIMOS\_COSMOS\_926434 & 4.449999809265137 & -1.9133213134380969 & 0.10648154069090557 & 1.1093900416105302E-9 & 1.5699811269088453E-10 & 0.0013336096287160822 & 2.7692937425682993E-4 & 0.8745033650649772 & 0.11949502455038681 & 0.25801125211847664 & 0.08977738933911 & 1130.9401193618705 & 65.29313511699506 & 3.643273963357895E11 & 6.58338724979248E10 & 6.0798256382186554E7 & 1.098623023966046E7 & 1.9779758714939304E11 & 9.889879357469652E9 & 50.57625464403506 & 4.944956976934494 & 4.558924521317336E10 & 4.664334835434328E9\\
%   DEIMOS\_COSMOS\_933876 & 4.4166998863220215 & -2.2741286215429075 & 0.17493668666521117 & 5.724893276624604E-9 & 2.747748513675799E-9 & 0.003151620572470711 & 0.002831245733293205 & 0.38569802072311526 & 0.260299048694715 & -0.3237809854345427 & 0.34229999605868594 & 404.8982172221982 & 166.51892726368186 & 4.5366778562148476E10 & 3.8594397920339386E10 & 7570720.90102502 & 6440559.022671602 & 6.99173284606269E10 & 3.495866423031345E9 & 13.752153277607876 & 5.273809238345603 & 2.4021676235886345E9 & 6.93315949315108E8\\
%   vuds\_cosmos\_5100537582 & 4.550099849700928 & -1.8564992699302598 & 0.37742589578813485 & 1.4198467313523774E-8 & 3.0329931484174166E-9 & 0.018128134738367375 & 0.0038444528287348533 & 1.8595659176633865 & 0.12751800993662685 & 0.7982352033464482 & 0.06343405349098029 & 162.69159839626218 & 41.94663346393587 & 3.895816928437303E11 & 3.3884152741585133E10 & 6.501264489450803E7 & 5654522.351037618 & 6.1924877320120224E10 & 3.9435739292672954E9 & 50.91974032754422 & 4.617057497921021 & 3.586284294153646E9 & 6.936411417965617E8\\
%   vuds\_cosmos\_5100541407 & 4.563000202178955 & -2.1643818540980546 & 0.13377280983261833 & 1.1230591079079635E-8 & 3.28530899113007E-9 & 0.015938406995730996 & 0.004508775110157672 & 2.272505904414628 & 0.11712907102589104 & 0.9955697005331655 & 0.05422940661400543 & 205.0391661483316 & 69.77548946952996 & 6.959654739053646E11 & 4.480618114926422E10 & 1.1614138201303224E8 & 7477169.481124899 & 7.037973544221399E10 & 4.856607690281154E9 & 81.8360560811942 & 8.057643427089657 & 7.286887707418941E9 & 2.0072767773300686E9\\
%   vuds\_cosmos\_5100559223 & 4.562699794769287 & -1.4450857796220564 & 0.31675415941517804 & 1.0375495463939797E-8 & 2.038564056035892E-9 & 0.014086183599308227 & 0.0027571123722515034 & 1.8973658918707546 & 0.12422804373766745 & 0.8162005365340723 & 0.06116403673989033 & 219.40369806478634 & 50.039399868597485 & 4.1046962312987756E11 & 3.790527472642949E10 & 6.849838259527634E7 & 6325559.4672068525 & 6.253772255577437E10 & 3.4394028611743464E9 & 50.45402488857274 & 4.738597713349104 & 4.8628063174357815E9 & 8.392122533039665E8\\
%   vuds\_cosmos\_5100822662 & 4.520500183105469 & -0.9945562732976893 & 0.21255113666765837 & 2.904691972291932E-9 & 5.714059867729635E-10 & 0.004294412516926514 & 8.613659785546285E-4 & 1.5377105162434217 & 0.1036682800649452 & 0.6435101858086135 & 0.05416954197061274 & 629.020128939277 & 109.03792608336457 & 4.701129989852625E11 & 4.63599189343182E10 & 7.84515546411486E7 & 7736454.259476667 & 1.0645094031060654E11 & 5.322547015530327E9 & 53.063742731230874 & 4.80255479216351 & 1.8268285669327343E10 & 3.1907773323514647E9\\
%   vuds\_cosmos\_5100969402 & 4.578499794006348 & -1.775685771479118 & 0.3219585744406674 & 8.15636997923448E-9 & 1.5756651459733085E-9 & 0.011041593484351183 & 0.002155101513877438 & 1.7191232272763106 & 0.10803377232337867 & 0.7275762694078401 & 0.055112470718938614 & 273.27594984718434 & 57.67369122190825 & 4.74302623792011E11 & 4.5489307525289925E10 & 7.915071118470727E7 & 7591168.299135185 & 8.851222607112614E10 & 4.425611303556308E9 & 58.46823517429471 & 5.365809759910355 & 7.168413807018386E9 & 1.218568115430782E9\\
%   vuds\_cosmos\_5100994794 & 4.5802001953125 & -1.3950899978801197 & 0.24658841348203298 & 1.2859321643841523E-8 & 3.205466305442395E-9 & 0.015248159153991704 & 0.0037298705249356467 & 1.5204713151086071 & 0.11519986518156021 & 0.6258252050085116 & 0.06228185045302758 & 180.72708394859575 & 55.685682701171544 & 3.3426634254954694E11 & 3.3216104759132618E10 & 5.578172544436443E7 & 5543039.786395907 & 7.888755201612201E10 & 4.306806169719862E9 & 47.04273755889807 & 5.190974606794934 & 3.6582596548883567E9 & 8.176861598316811E8\\
%   vuds\_cosmos\_5101013812 & 4.416299819946289 & -2.260745457434047 & 0.12765384857413822 & 1.5599528843817957E-9 & 5.331785027605691E-10 & 0.0010119062262184434 & 8.2418347052784E-4 & 0.3927819713855686 & 0.2537787407410719 & -0.290462189575628 & 0.3264670486277929 & 952.7053213933843 & 191.30771429796923 & 6.7898440530183464E10 & 5.3598256065071655E10 & 1.1330761388858031E7 & 8944374.062056221 & 1.0189268601593655E11 & 6.05609992078074E9 & 17.467482117236536 & 4.833422734227668 & 1.1197442110028112E10 & 2.246561908404511E9\\
%   vuds\_cosmos\_5101210235 & 4.576099872589111 & -2.2237543029091507 & 0.10905846008166152 & 4.996192098473196E-9 & 1.0444214807683031E-9 & 0.0026497930605176266 & 9.765225959100163E-4 & 0.37578919954156575 & 0.10762389311159921 & -0.2667913848077658 & 0.16362426514051126 & 416.7718390515992 & 84.00373716539698 & 9.522468244842317E10 & 3.0596025377253136E10 & 1.5890912173059674E7 & 5105805.96977024 & 1.6586930384431094E11 & 8.2934651922155485E9 & 29.962358577942293 & 3.1599058018252486 & 5.997038942337424E9 & 1.0824089105829957E9\\
%   vuds\_cosmos\_5101218326 & 4.57390022277832 & -0.4291648102146993 & 0.13665642945583834 & 1.0280659797602142E-9 & 8.063056057489838E-11 & 0.0019890315320124983 & 1.7140043387462535E-4 & 2.0365661359053853 & 0.07215737529978626 & 0.928881772010432 & 0.03522868720348423 & 1174.7868912639876 & 29.559722167771806 & 1.326781050029107E12 & 8.151434276517009E10 & 2.2141067417381078E8 & 1.3602957010936715E7 & 1.5612829747983597E11 & 7.806414873991799E9 & 114.4400066114377 & 5.722000330571885 & 1.1131581908597894E11 & 6.726244050873537E9\\
%   vuds\_cosmos\_5101244930 & 4.5802998542785645 & -1.9239948795605761 & 0.2304393427036423 & 1.65036916118173E-8 & 3.3366147761235028E-9 & 0.017439680992747845 & 0.003637834755171757 & 1.301346459605106 & 0.10361502176416398 & 0.5023732528192688 & 0.060728756773731095 & 140.37984552299537 & 34.67365037712535 & 3.5365452585903406E11 & 3.86814191138417E10 & 5.9017188249221936E7 & 6455080.952360253 & 1.1067657236608917E11 & 5.53382861830446E9 & 55.84972999602215 & 5.393318495895406 & 3.3840749881700115E9 & 6.01078875069877E8\\
%   vuds\_cosmos\_5101288969 & 5.720900058746338 & -2.1004767903011485 & 0.19965432129040517 & 3.0237531911315E-9 & 8.428854814964742E-10 & 0.0025732342687697666 & 0.001020865338062525 & 0.6435319721730057 & 0.19448798201483342 & 0.029467101314131477 & 0.19351457369057629 & 608.6665681268803 & 140.95851233158947 & 7.722049937252698E10 & 2.3352533351292583E10 & 1.2886408669866405E7 & 3897025.9281760636 & 6.870054228218806E10 & 7.129677907181336E9 & 15.142546409644247 & 1.6426560294097008 & 5.00786454862007E9 & 1.2859235794531057E9\\
%   vuds\_cosmos\_510148750 & 4.508800029754639 & -2.4615572916284165 & 0.07547772153731716 & 1.1096801261165857E-8 & 5.3408057947196005E-9 & 0.003715764168661867 & 0.003036226206473926 & 0.2511260595210722 & 0.14934222333209188 & -0.5051742667340139 & 0.25816496936785854 & 218.04928425853615 & 111.96389339776368 & 2.68656563445032E10 & 1.8983745728760036E10 & 4483289.14799309 & 3167971.037916732 & 7.125527050372833E10 & 3.5627635251864166E9 & 13.388946772027545 & 3.367666302723991 & 1.2065591206795092E9 & 4.950967861924123E8\\
%   vuds\_cosmos\_510327576 & 4.566100120544434 & -2.3019034673864205 & 0.1885808157211991 & 1.608911966511924E-8 & 9.793550433911888E-9 & 0.009113020811433444 & 0.007713671096449279 & 0.5084124783675228 & 0.31259535177926234 & -0.17391846193439234 & 0.37328763145803906 & 179.77129749381896 & 113.16827215935449 & 6.055894497791706E10 & 4.593371508918566E10 & 1.010596046312327E7 & 7665330.180123715 & 6.5801832350503586E10 & 3.29009161752518E9 & 17.842163491841998 & 8.545082305032336 & 1.108958343477506E9 & 4.166394329958334E8\\
%   vuds\_cosmos\_510581738 & 4.50439977645874 & -2.2787636056346243 & 0.14122041807226426 & 3.151636778347752E-9 & 1.46719959186377E-9 & 0.001870827641051059 & 0.0018103428120561866 & 0.38086557139604915 & 0.27360426918678304 & -0.33149408290771853 & 0.347111245221295 & 628.3131148416863 & 210.95405980494613 & 4.017897242012885E10 & 3.750781724449693E10 & 6704989.7727711145 & 6259232.525750927 & 6.1599216579519844E10 & 3.3146885702361774E9 & 11.295371044677786 & 4.400793805164466 & 3.5839698033348227E9 & 9.132253704056442E8\\
%   vuds\_cosmos\_510605533 & 4.5019001960754395 & -1.999047649253923 & 0.2527208673387991 & 1.6819010316514256E-8 & 4.6962616400887204E-9 & 0.015731035115782045 & 0.0046776783892476526 & 1.059151503779184 & 0.11879249923828987 & 0.3553739414982982 & 0.0778857889952574 & 137.7015590223393 & 43.67462230652926 & 1.9061652720189325E11 & 2.6921958795480568E10 & 3.180972007062948E7 & 4492684.792909984 & 8.335199986879036E10 & 4.167599993439518E9 & 34.00971430650517 & 3.313859885845941 & 2.0220996162367353E9 & 5.291237539047335E8\\
%   vuds\_cosmos\_510786441 & 4.463500022888184 & -1.9466749404687251 & 0.09596765572210356 & 6.94496477893142E-9 & 1.212925160373366E-9 & 0.005952652870138335 & 0.001154251178295181 & 0.743596979722237 & 0.06436887388958179 & 0.12842190604569365 & 0.05315657096872125 & 314.260927312882 & 58.49658590040318 & 3.069130127738927E11 & 3.349399004647891E10 & 5.1217054290526845E7 & 5589412.749601084 & 2.2710183002102878E11 & 1.135509150105144E10 & 59.754977467728786 & 4.145314067449293 & 8.604072068011686E9 & 1.3790563253084712E9\\
%   vuds\_cosmos\_5110377875 & 4.55049991607666 & -0.761508212471262 & 0.14626853737656523 & 4.22936441173979E-9 & 7.584265154315115E-10 & 0.006166592275130619 & 0.001108397425266723 & 1.6513984419394963 & 0.08610540642540472 & 0.6967348658212703 & 0.04363673816195311 & 475.25344327699986 & 83.26216267830279 & 7.045262233249691E11 & 5.613749493562198E10 & 1.1756998343930833E8 & 9368117.369367218 & 1.413245960176657E11 & 7.0662298008832855E9 & 80.63550850481917 & 6.3486814462485786 & 1.9065632718001938E10 & 3.0717685526014876E9\\
%   vuds\_cosmos\_5131465996 & 4.473599910736084 & -2.155181020204242 & 0.2507117603022014 & 4.260464054326612E-9 & 3.4869572006114743E-9 & 0.0036657173241869635 & 0.003981038935590954 & 0.6610317988029021 & 0.5008157141246306 & -0.06340870716053047 & 0.4669164951135341 & 597.0234279686475 & 315.5207961465994 & 4.3167275947188126E10 & 4.44524681650387E10 & 7203672.127744192 & 7418142.537455717 & 2.9887794407693817E10 & 3.7617395222667384E9 & 8.372436673418544 & 6.213942064175301 & 1.9651466522563705E9 & 6.779223088771529E8\\
%   vuds\_cosmos\_5180966608 & 4.529600143432617 & -0.9098892949484128 & 0.19656561366393677 & 1.1295896880833912E-9 & 1.2530216681630297E-10 & 0.0022292286894914316 & 2.564462809817772E-4 & 2.2229662032511954 & 0.0964247684966403 & 1.0180310146117586 & 0.044784848616108604 & 1119.433861066708 & 68.52066075744641 & 1.0814504692599115E12 & 7.527543222809999E10 & 1.8047037789631388E8 & 1.2561819599385288E7 & 1.0364115930856772E11 & 5.182057965428386E9 & 91.44753915880037 & 5.722641787218498 & 8.095642171978584E10 & 7.414819548998585E9\\
%   HZ4 & 5.539999961853027 & -2.0743219660201873 & 0.18908890030304912 & 1.1903786929362953E-8 & 4.5290928022850444E-9 & 0.011154508789330192 & 0.00424558951371248 & 0.9845253689148901 & 0.0900844526346481 & 0.3079946485999043 & 0.06139597498276544 & 195.3059815269737 & 83.95598345512462 & 4.35669143706752E11 & 5.023518870520547E10 & 7.270363020539273E7 & 8383151.838220889 & 2.1313447620591043E11 & 1.0656723810295523E10 & 77.5873271787668 & 8.909965933344276 & 6.517869283041594E9 & 2.36423027351835E9\\
%   HZ6 & 5.289999961853027 & -1.1246840100067022 & 0.1262033639563695 & 1.8503912379617593E-9 & 2.897272193514763E-10 & 0.001984266934592969 & 3.1068896653658904E-4 & 0.8160477116248636 & 0.03944924319599454 & 0.20202384483878424 & 0.030117792981569944 & 844.3310238131696 & 93.05065456574634 & 4.761012134686608E11 & 2.3805060673433044E10 & 7.945085637660642E7 & 3972542.818830321 & 2.9898782417845636E11 & 1.494939120892282E10 & 74.09041894758367 & 3.7045209473791836 & 4.004040736228067E10 & 5.941125543491076E9\\
%   566428 & 5.889999866485596 & -1.7247198308040363 & 0.21994562204914003 & 3.4079448795397513E-9 & 1.376846537565123E-9 & 0.004119454536168874 & 0.0019218074434743898 & 1.1038623774304213 & 0.29682476186375406 & 0.37779959212713726 & 0.19500972033248257 & 589.2926811017252 & 209.31146873017357 & 3.8147119922815625E11 & 1.4729157454981442E11 & 6.365918129230534E7 & 2.4579735157116607E7 & 1.479999289121566E11 & 1.0375850113101017E10 & 52.664006609614674 & 16.203779475929416 & 1.5453303521953394E10 & 4.0461802896528244E9\\
%   HZ9 & 5.547999858856201 & -2.4724782759646406 & 0.20459249954084302 & 5.770511631231214E-8 & 1.8871534680278983E-8 & 0.053721707199260414 & 0.017395007737092166 & 1.9455975245351385 & 0.11685591227011607 & 0.8613472272399006 & 0.05417621133799237 & 39.286920211267 & 16.870028435426793 & 7.272957267995934E11 & 6.20808667692828E10 & 1.213697144610989E8 & 1.0359935849535905E7 & 9.987513419290558E10 & 4.993756709645279E9 & 130.36915345583515 & 12.634272847988086 & 2.259230407755355E9 & 7.056592915804071E8\\
%   HZ10 & 5.658999919891357 & -1.8751804883618821 & 0.228544324568629 & 7.787398863299889E-9 & 1.663756938459762E-9 & 0.011999246773852239 & 0.002562833754580558 & 2.4018902131554065 & 0.10488854843784322 & 1.061154945476034 & 0.048247926595384426 & 282.70639821803314 & 60.593263388757315 & 1.4529665470263242E12 & 7.791411221242177E10 & 2.424682676331826E8 & 1.3002157448832866E7 & 1.2633573696055638E11 & 7.410075084419604E9 & 157.35963659548543 & 8.478576251222734 & 2.0206957336817947E10 & 4.177619146578139E9\\
%   CLM1 & 6.1656999588012695 & -1.9814802101777753 & 0.12342473866739936 & 1.7908769605189148E-9 & 1.802773159791595E-10 & 3.383527441481748E-4 & 3.4475542104171026E-5 & 0.10693245997771705 & 0.0061125578300861814 & -0.8376433169922274 & 0.02533702148084591 & 863.1680165625413 & 52.10074288752389 & 3.687228667079784E10 & 1.9331587795778947E9 & 6153176.403847693 & 322601.82541947905 & 2.5358084961730368E11 & 1.2679042480865185E10 & 32.568324171278654 & 1.6284162085639329 & 1.818568494054546E10 & 1.5888601566673987E9\\
%   WMH5 & 6.069499969482422 & -1.658684729448018 & 0.18237343957591107 & 2.2840833458798234E-9 & 4.932870019210283E-10 & 0.0031727658638156945 & 7.156732096138495E-4 & 1.2898867005567842 & 0.09876856142238011 & 0.5105025162875554 & 0.05830866330150712 & 735.8690780496262 & 119.2283309648243 & 6.232425116200159E11 & 5.4083081361473206E10 & 1.0400551369688281E8 & 9025280.776642194 & 1.920056440219665E11 & 9.600282201098324E9 & 74.87387090991646 & 4.295508067276408 & 3.2780708744704422E10 & 6.8252008228998165E9\\
\end{tabular}

%\end{sidewaystable}
\end{adjustbox}
 \caption{Physical parameters. Only the first rows are shown. The table contains for each object in the sample the following information, for PL+OT\_MBB: id, redshift, $\beta_{FUV}$, sSFR, sM\_dust, M\_dust, A\_FUV,  IRX, age\_main, L\_dust, L\_FUV, SFR, M\_star.}
 \label{Tab.Physical_parameters_dl2014}
\end{table}


==> Physical_parameters_plotmbb_final_21Oct.tex <==
\onecolumn
\sisetup{table-column-width=12ex,    % local setting for all S columns
         round-mode=places,
         round-precision=3,
         tight-spacing,
         table-format = 5.3e-2,
         table-number-alignment = center
         }
  \begin{table}[h!]
  \centering
\begin{adjustbox}{max width=\textwidth}
%\begin{sidewaystable}

%\begin{longtable}{|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|}
\begin{tabular}{|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|l|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|S|}
 

\hline
  \multicolumn{1}{|c|}{id} &
  \multicolumn{1}{c|}{redshift} &
  \multicolumn{1}{c|}{$\beta_{FUV}$} &
  \multicolumn{1}{c|}{$\beta_{FUV}$\_err} &
  \multicolumn{1}{c|}{sSFR} &
  \multicolumn{1}{c|}{sSFR\_err} &
  \multicolumn{1}{c|}{sM$_{dust\_dl2014}$} &
  \multicolumn{1}{c|}{sM$_{dust\_dl2014}$\_err} &
  \multicolumn{1}{c|}{sM$_{dust\_pre-shock}$} &
  \multicolumn{1}{c|}{sM$_{dust\_pre-shock}$\_err} &
  \multicolumn{1}{c|}{sM$_{dust\_post-shock}$} &
  \multicolumn{1}{c|}{sM$_{dust\_post-shock}$\_err} &
  \multicolumn{1}{c|}{M$_{dust\_dl2014}$} &
  \multicolumn{1}{c|}{M$_{dust\_dl2014}$\_err} &
  \multicolumn{1}{c|}{M$_{dust\_pre-shock}$} &
  \multicolumn{1}{c|}{M$_{dust\_pre-shock}$\_err} &
  \multicolumn{1}{c|}{M$_{dust\_post-shock}$} &
  \multicolumn{1}{c|}{M$_{dust\_post-shock}$\_err} &
  \multicolumn{1}{c|}{A$_{FUV}$} &
  \multicolumn{1}{c|}{A$_{FUV}$\_err} &
  \multicolumn{1}{c|}{IRX} &
  \multicolumn{1}{c|}{IRX\_err} &
  \multicolumn{1}{c|}{age$_{main}$} &
  \multicolumn{1}{c|}{age$_{main}$\_err} &
  \multicolumn{1}{c|}{L$_{dust}$} &
  \multicolumn{1}{c|}{L$_{dust}$\_err} &
  \multicolumn{1}{c|}{L$_{FUV}$} &
  \multicolumn{1}{c|}{L$_{FUV}$\_err} &
  \multicolumn{1}{c|}{SFR } &
  \multicolumn{1}{c|}{SFR\_err} &
  \multicolumn{1}{c|}{M$_{star}$} &
  \multicolumn{1}{c|}{M$_{star}$\_err} \\
     &   &   &   & [yr$^{-1}$] & [yr$^{-1}$] &   &   &   &   &   &   & [Myrs] & [Myrs] & [L$_\odot$] &  & [M$_\odot$] & [M$_\odot$] & [L$_\odot$] & [L$_\odot$] & [M$_\odot$ yr$^{-1}$] & [M$_\odot$ yr$^{-1}$] & [M$_\odot$ yr$^{-1}$] & [M$_\odot$ yr$^{-1}$] \\
\hline
  CANDELS\_GOODSS\_12 & 4.431000232696533 & -2.144344430007398 & 0.1460967634012939 & 1.0069640335966491E-8 & 3.062395929299864E-9 & 0.004715939430851186 & 0.0014341273933664788 & 0.006620897832979376 & 0.002013429368672506 & 0.0041251007751336825 & 0.0012544520786919304 & 1.9960376874831546E7 & 2060778.414705241 & 2.8023179248544946E7 & 2893210.046531481 & 1.7459631813690756E7 & 1802592.8365973544 & 1.5665890629827568 & 0.09418145081174756 & 0.6520640523959013 & 0.05005426413638634 & 225.65478612399394 & 73.74800516536834 & 3.193129856753339E11 & 3.297188265305342E10 & 7.080738181452225E10 & 3.540369090726112E9 & 42.62010126445132 & 4.402695914241293 & 4.2325346131998286E9 & 1.2106744448488061E9\\
   CANDELS\_GOODSS\_14 & 5.552700042724609 & -1.9627663677483977 & 0.06621954990145637 & 1.3261226412638939E-9 & 1.154215751295264E-10 & 3.160246818134731E-4 & 7.18346280159452E-5 & 4.4367981431202714E-4 & 1.008515355079121E-4 & 2.764313831899319E-4 & 6.283479337573494E-5 & 6498864.565893009 & 1414214.7236769209 & 9124018.43833292 & 1985473.167468151 & 5684651.308894224 & 1237034.1770467116 & 0.3912359041277432 & 0.07600263936782348 & -0.21201247306620347 & 0.10750851771179427 & 1028.2639631966056 & 20.583247293827203 & 1.0384652472279529E11 & 2.2636185114695347E10 & 1.6498025003058682E11 & 8.249012501529341E9 & 27.27094413601888 & 1.5572726300028987 & 2.0564420881938667E10 & 1.3507838486974697E9\\
   CANDELS\_GOODSS\_19 & 4.5 & -0.5577911744909068 & 0.10923765003146907 & 1.9773443241802593E-9 & 3.8441244222937E-10 & 0.0013996563208089308 & 2.6132419496119406E-4 & 0.001965034037701186 & 3.6688359159255866E-4 & 0.001224299730424564 & 2.2858407216672831E-4 & 3.3159068447112266E7 & 4073900.7060818397 & 4.655335541183464E7 & 5719513.736800058 & 2.9004719199543502E7 & 3563500.1693485817 & 2.4803586918253133 & 0.13652862903135152 & 1.1193926838989579 & 0.05711257520244856 & 817.4007981199693 & 126.36315212013255 & 5.306601983330469E11 & 6.51928919687117E10 & 4.003982699611688E10 & 2.0019913498058443E9 & 46.84499674256306 & 6.290140237294263 & 2.3690864645935364E10 & 3.330627792062718E9\\
   CANDELS\_GOODSS\_21 & 5.571599960327148 & -1.385195733484872 & 0.2240503999483133 & 2.9611185823600035E-9 & 1.1881331027579991E-9 & 0.001721959860077444 & 6.927449461230134E-4 & 0.002417528993583035 & 9.72572608246038E-4 & 0.0015062233215053138 & 6.059540747125763E-4 & 1.2567260331853388E7 & 1051205.6831745997 & 1.764368434279015E7 & 1475830.114402064 & 1.0992765300821157E7 & 919504.8923064314 & 1.75737511695253 & 0.11196872998014781 & 0.7622250123623201 & 0.05677219649616781 & 605.7674995415812 & 195.00521795928114 & 2.0108653038935873E11 & 1.6826274387839476E10 & 3.470240296958019E10 & 1.7351201484790096E9 & 21.610926573127653 & 1.6945631482413752 & 7.298230709796094E9 & 2.8719145818186316E9\\
   CANDELS\_GOODSS\_32 & 4.4105000495910645 & -0.6785370292415938 & 0.10190585887099374 & 9.7893077452638E-9 & 1.8377886491969703E-9 & 0.005497588714152909 & 9.892909662905158E-4 & 0.0077182868308334415 & 0.001388905542774694 & 0.004808820765966696 & 8.653471894021303E-4 & 3.9707147414796926E7 & 3097332.168897618 & 5.5746467936499976E7 & 4348469.726077503 & 3.4732419061107926E7 & 2709281.4736299426 & 2.4627444624695802 & 0.09101378818920412 & 1.0856434725558535 & 0.04075595672246265 & 231.66836489551997 & 50.424300468198425 & 6.353298506229738E11 & 4.95524890342018E10 & 5.204480724151431E10 & 2.6022403620757155E9 & 70.70472273222722 & 6.68780420350663 & 7.222647869706122E9 & 1.171256705016367E9\\
%   CANDELS\_GOODSS\_37 & 4.519999980926514 & -0.8526933686190812 & 0.23096820607580118 & 2.0809938034121604E-9 & 1.4536501513634613E-9 & 0.0015567858336171972 & 0.001082551901808362 & 0.002185634506834349 & 0.0015198383367440794 & 0.0013617431994482467 & 9.469238854210877E-4 & 1.1209251281741425E7 & 4545634.174267391 & 1.5737120590458447E7 & 6381799.40502159 & 9804895.043495925 & 3976132.291495555 & 3.2169995832185556 & 0.4726928389389614 & 1.443407802243781 & 0.20409972746658323 & 781.6580987744164 & 277.9004385229867 & 1.7939450686014005E11 & 7.275043780699217E10 & 5.874625003167713E9 & 2.937312501583857E8 & 14.983681091184389 & 6.157104918474725 & 7.200252622865081E9 & 4.0673297556233773E9\\
%   CANDELS\_GOODSS\_38 & 5.5721001625061035 & -1.3342119670909967 & 0.14395279564668623 & 7.1585850981794126E-9 & 2.1817486066046875E-9 & 0.003321573347888539 & 0.0010213306631659624 & 0.004663290973851195 & 0.0014338873672282099 & 0.0029054284926567295 & 8.933727780157865E-4 & 1.509321682400001E7 & 1332895.545304329 & 2.1189976679720186E7 & 1871305.8886552458 & 1.320225616398674E7 & 1165903.1095984029 & 1.3864266568600048 & 0.10009366367934677 & 0.5547418929955149 & 0.05616244345473473 & 305.33326960940894 & 93.88348338844347 & 2.4144794475285568E11 & 2.133079768695092E10 & 6.713880331374475E10 & 3.356940165687238E9 & 32.52858381361956 & 2.548760155203343 & 4.5439962461146555E9 & 1.3383407088925905E9\\
%   CANDELS\_GOODSS\_42 & 5.525199890136719 & -2.105111640907456 & 0.2265720196887971 & 2.903919271133577E-9 & 1.902217481983749E-9 & 8.5443915667087E-4 & 6.409365739889987E-4 & 0.0011995816408935137 & 8.998367421854396E-4 & 7.473903512054665E-4 & 5.606365384757157E-4 & 2996170.1498546605 & 1161679.5845017112 & 4206444.281840522 & 1630928.8862633966 & 2620793.584994598 & 1016138.0197412885 & 0.58139236199047 & 0.1851822120229664 & -0.02885850742587327 & 0.2080969762062213 & 578.8933110642636 & 285.34364512566935 & 4.789762858014822E10 & 1.8595038474703777E10 & 4.666344906885243E10 & 2.333172453442622E9 & 10.182862255117378 & 1.317198506606659 & 3.5065927473742704E9 & 2.251768462330634E9\\
%   CANDELS\_GOODSS\_47 & 5.57450008392334 & -2.0559536536171032 & 0.25094123798543355 & 2.3084971625115538E-8 & 8.935664175406038E-9 & 0.007547220174396312 & 0.0030898793368297657 & 0.010595847217795952 & 0.004338006394134603 & 0.006601663199454524 & 0.0027027623730793886 & 6396902.770377914 & 1100075.4468867881 & 8980870.155605562 & 1544440.3494155877 & 5595463.844152458 & 962251.9850385708 & 1.0570527970366388 & 0.1378378195545063 & 0.3597691065570046 & 0.08943225367640519 & 100.67080450586248 & 43.72043214768835 & 1.022850372889369E11 & 1.7605635540407566E10 & 4.4044446660948326E10 & 2.202222333047416E9 & 19.566451690884872 & 2.1244584721198563 & 8.475839610561767E8 & 3.1490888742028075E8\\
%   CANDELS\_GOODSS\_57 & 5.558499813079834 & -1.1003773836681623 & 0.13415852750636048 & 1.4773331821545958E-9 & 1.9005271591022327E-10 & 8.939644359464973E-4 & 1.2831267483418753E-4 & 0.0012550727768041953 & 1.8014334645517785E-4 & 7.819636875614506E-4 & 1.1223696194131325E-4 & 1.818973569834181E7 & 1722283.243856877 & 2.5537304588723667E7 & 2417983.0051317117 & 1.5910826237045955E7 & 1506506.1899981694 & 1.5403395580507335 & 0.09876793985602753 & 0.6653998936800716 & 0.052951451910768735 & 967.3575339125678 & 69.87156160956287 & 2.910606793039235E11 & 2.7565943642771988E10 & 6.2665286580288826E10 & 3.1332643290144415E9 & 30.059697054202083 & 2.10704936534591 & 2.034726994377933E10 & 2.1949003399090414E9\\
%   CANDELS\_GOODSS\_8 & 5.517399787902832 & -1.9707045003788612 & 0.15473480803867837 & 6.2757822896866546E-9 & 2.7289796539283458E-9 & 0.001408045399321616 & 0.0010499660466425256 & 0.001976811803840838 & 0.0014740897386086014 & 0.0012316377793504998 & 9.184205642113993E-4 & 2619616.0165126836 & 1770548.2272004746 & 3677784.7258815225 & 2485744.164560075 & 2291416.2106443043 & 1548724.2725502928 & 0.44053899498072885 & 0.24643371740710582 & -0.23402259733081116 & 0.3190660028787402 & 365.00777233806116 & 153.10368503569637 & 4.185412753242257E10 & 2.832751265192605E10 & 5.640243466766665E10 & 2.8201217333833323E9 & 11.675859180485599 & 3.4998177858538715 & 1.860462750543975E9 & 5.860882982104288E8\\
%   DEIMOS\_COSMOS\_206253 & 4.474999904632568 & -1.15944008390656 & 0.2697863076576818 & 1.0398601218996082E-9 & 7.841162446972403E-11 & 6.328503574717702E-4 & 5.8558815051513996E-5 & 8.884841762331118E-4 & 8.221308550742569E-5 & 5.535634073398695E-4 & 5.1222246787065005E-5 & 1.9960624192642298E7 & 1463549.183950626 & 2.802352646800806E7 & 2054735.8087524187 & 1.7459848146175046E7 & 1280187.7466164401 & 1.422689703899772 & 0.10845884509099592 & 0.6128111477824076 & 0.061269015812052185 & 1167.9858003972795 & 36.273911484902825 & 3.193986635438917E11 & 2.3430091761363205E10 & 7.791289797789996E10 & 5.215625205859317E9 & 32.7980491139711 & 1.6399024556985553 & 3.154082787024844E10 & 1.7803267693266428E9\\
%   DEIMOS\_COSMOS\_274035 & 4.479100227355957 & -2.1714885466119074 & 0.3293959274170321 & 1.648134547453309E-8 & 4.0834131441673595E-9 & 0.00554609057372186 & 0.0014959560135139485 & 0.007786380550361468 & 0.002100233065614093 & 0.004851246047596574 & 0.0013085344715291383 & 1.1079404888661085E7 & 1647628.3189841781 & 1.5554823995014124E7 & 2313171.9409612636 & 9691316.515909247 & 1441204.4419635616 & 0.9816824317346386 & 0.11681405956354572 & 0.3072700831367291 & 0.08051436266158783 & 140.83906651867755 & 41.10912056391118 & 1.7716275309890588E11 & 2.636277173031094E10 & 8.641357974318927E10 & 4.320678987159463E9 & 32.924723676070975 & 3.412858661298111 & 1.9976963486959317E9 & 4.4954922033214545E8\\
%   DEIMOS\_COSMOS\_308643 & 4.525300025939941 & -1.7365268395008358 & 0.10349143361274572 & 9.130423125783844E-9 & 1.6400270789096754E-9 & 0.0034736436240667174 & 6.813857464359612E-4 & 0.004876788576348381 & 9.566249690332906E-4 & 0.0030384465738546402 & 5.960180176191755E-4 & 2.3485446645116758E7 & 2754967.2638014727 & 3.29721670685539E7 & 3867809.8084775587 & 2.0543061585217584E7 & 2409809.914230425 & 1.0220827907022947 & 0.08789680148635132 & 0.3333201175298585 & 0.05879618567796042 & 246.4057353518198 & 49.346969113792525 & 3.7560386658230975E11 & 4.4079819839301895E10 & 1.7322686599116467E11 & 8.661343299558233E9 & 61.73116426862853 & 5.362590808244058 & 6.761040908860281E9 & 1.0629625073408194E9\\
%   DEIMOS\_COSMOS\_336830 & 5.714000225067139 & -2.4578762256419755 & 0.09420195133547855 & 9.223218810248125E-9 & 5.27687680702833E-9 & 0.0012240398284170933 & 0.0010927858033994912 & 0.0017184789512838237 & 0.0015342061245117438 & 0.0010706854316164319 & 9.558756279116795E-4 & 864186.3788897535 & 635360.663358831 & 1213266.1598346157 & 892008.4960534697 & 755916.3881743636 & 555759.2083912557 & 0.26826255848101654 & 0.1824030100117644 & -0.4837152035360014 & 0.28232718177605226 & 264.55825680065334 & 170.30985877523264 & 1.3784689808748266E10 & 1.0165281858490213E10 & 3.464027727574464E10 & 3.6799770504443846E9 & 6.511699930257662 & 1.73304055521706 & 7.060116499700047E8 & 3.575657677084248E8\\
%   DEIMOS\_COSMOS\_351640 & 5.7058000564575195 & -1.9377226217300454 & 0.21650281881772918 & 1.2043677370440937E-8 & 4.054938133722932E-9 & 0.004118888714103381 & 0.0014549523323344803 & 0.005782674218224247 & 0.0020426663415613376 & 0.003602851833949559 & 0.0012726679555365382 & 1.0719629018794496E7 & 1459400.3217677635 & 1.5049720120783906E7 & 2048911.0535708435 & 9376615.332524203 & 1276558.6765536466 & 0.9381076506463818 & 0.1212022189246512 & 0.27587105211649854 & 0.0861787570858733 & 190.39725097073327 & 70.42454935604484 & 1.714132802376402E11 & 2.335718486316195E10 & 9.014514415147221E10 & 5.444636474985943E9 & 31.344316973439078 & 2.6438204472551545 & 2.6025536893215127E9 & 8.483006221983285E8\\
%   DEIMOS\_COSMOS\_372292 & 5.13640022277832 & -1.9057373607111363 & 0.40712467208007763 & 2.0676352711735338E-8 & 5.6145790718655715E-9 & 0.007207037455903276 & 0.0019911706919016657 & 0.010118250960101641 & 0.002795484953190823 & 0.006304100430398896 & 0.0017417059495830965 & 1.513513007263129E7 & 1427323.2389710385 & 2.124882038225389E7 & 2003876.7415125133 & 1.3238918291851696E7 & 1248500.3859311743 & 1.127127007270394 & 0.10848127885323139 & 0.40402313777659377 & 0.06814071099816978 & 112.31250799831471 & 37.20893450611869 & 2.420300830019558E11 & 2.2843148787515408E10 & 9.52674226292008E10 & 5.841474104534343E9 & 43.42134887385507 & 3.4462551336071043 & 2.1000487600122185E9 & 5.453578034612988E8\\
%   DEIMOS\_COSMOS\_396844 & 4.542399883270264 & -1.0215453178764897 & 0.20069043392384597 & 2.2815058653993442E-8 & 6.192739312506073E-9 & 0.010277129640783294 & 0.002705150993249305 & 0.01442847737245618 & 0.0037978707342841414 & 0.008989554694024711 & 0.0023662348982061146 & 4.407918503915116E7 & 3161468.143081753 & 6.1884548133930884E7 & 4438512.810539916 & 3.855670392684508E7 & 2765382.1425847127 & 2.0382420538526946 & 0.1012535294185412 & 0.8906700664687898 & 0.04859955857337071 & 102.2576173783561 & 34.91844788991212 & 7.051288110479817E11 & 5.057769747420902E10 & 9.06000830659427E10 & 4.530004153297135E9 & 97.85506529932367 & 9.555023675563294 & 4.289056047734314E9 & 1.0862487074109619E9\\
%   DEIMOS\_COSMOS\_400160 & 4.54040002822876 & -1.8250578796222117 & 0.09236417750238435 & 7.94609089061074E-9 & 1.4377770698652328E-9 & 0.0027052393833910107 & 5.952579553965319E-4 & 0.0037979948287739577 & 8.357066846885457E-4 & 0.0023663122143479805 & 5.206807867690381E-4 & 1.578590435192707E7 & 2526477.8504149797 & 2.2162468676241938E7 & 3547024.292859451 & 1.3808160014168635E7 & 2209946.902821828 & 0.8307401356081477 & 0.10290296558123332 & 0.1975291141535978 & 0.07901255429264768 & 280.1269782464781 & 55.319852795807556 & 2.5242211295923734E11 & 4.0425492248892494E10 & 1.581507515752444E11 & 7.907537578762219E9 & 46.367885792667316 & 4.622285052158824 & 5.835307754591196E9 & 8.811558691089693E8\\
%   DEIMOS\_COSMOS\_403030 & 4.5594000816345215 & -1.2985310485345152 & 0.14849944400424298 & 1.2367161313425716E-8 & 2.3964584769267842E-9 & 0.005586771370349653 & 0.0011030107368923624 & 0.00784349396375156 & 0.0015485613216040639 & 0.004886830131778096 & 9.648195258763572E-4 & 2.443532544519567E7 & 2443892.061313456 & 3.430574027941688E7 & 3431078.768088689 & 2.1373934379905146E7 & 2137707.9125563754 & 1.538910000994973 & 0.10938044735102476 & 0.6368622001575313 & 0.05862246989531515 & 185.6409720839661 & 42.22927730263502 & 3.908844698648093E11 & 3.9102053424042984E10 & 8.985099709892435E10 & 4.4925498549462185E9 & 54.09127946968013 & 5.0081735859360865 & 4.373782964321729E9 & 7.445289245026364E8\\
%   DEIMOS\_COSMOS\_412589 & 4.434100151062012 & -2.34350815306745 & 0.11995014134531869 & 2.3991106021341857E-9 & 1.7867952542287603E-9 & 5.24972398972196E-4 & 6.406652403624607E-4 & 7.370299533515525E-4 & 8.994558059485981E-4 & 4.59200988833126E-4 & 5.603991990082429E-4 & 2837674.6307229823 & 2916812.7077292455 & 3983926.021260049 & 4095031.1637750687 & 2482155.250382379 & 2551378.476759187 & 0.3565766295128359 & 0.26231242653425785 & -0.3588601314522054 & 0.3418127006125678 & 682.2822180097999 & 306.20178648720645 & 4.53348823568224E10 & 4.667717441739942E10 & 7.262304184605748E10 & 3.6311520923028746E9 & 12.96810138076475 & 4.528043346842046 & 5.405378713773624E9 & 3.555943071694872E9\\
%   DEIMOS\_COSMOS\_416105 & 5.630899906158447 & -2.3075406947785555 & 0.15822151174141794 & 1.7935984378150614E-8 & 7.090517982861757E-9 & 0.0030544884547085657 & 0.0016819098352008864 & 0.004288319705367867 & 0.002361301146129933 & 0.00267180545401555 & 0.0014711909825440407 & 3582470.3775887736 & 1414183.3752282376 & 5029574.850881664 & 1985429.1561149517 & 3133638.9171600523 & 1237006.7561029398 & 0.40275917629894636 & 0.16212262679351144 & -0.2409096778555497 & 0.22643826560481456 & 130.13829493715318 & 58.71941971546767 & 5.7196310254758865E10 & 2.2640211125358566E10 & 9.138723470370784E10 & 7.425207783974743E9 & 21.036299098976386 & 1.9856242184396389 & 1.1728544503307292E9 & 4.502466003705748E8\\
%   DEIMOS\_COSMOS\_417567 & 5.670000076293945 & -1.646569580189359 & 0.09330612434239574 & 2.292954079552178E-9 & 4.223712227638333E-10 & 9.192428297739362E-4 & 2.0319463690367235E-4 & 0.0012905621348350469 & 2.852731573157068E-4 & 8.040750661108738E-4 & 1.7773730271235873E-4 & 1.662669104831317E7 & 2413968.750707803 & 2.3342883076750014E7 & 3389068.223795337 & 1.4543608359899059E7 & 2111533.5577785266 & 0.8433899936029626 & 0.1051209559896717 & 0.21821370678310534 & 0.07870478527255786 & 737.7585654009478 & 105.57425506538206 & 2.6592825709326733E11 & 3.863540775067962E10 & 1.593595244516255E11 & 7.967976222581274E9 & 41.47352346284716 & 3.252168207012039 & 1.8087376381714146E10 & 3.014797480345991E9\\
%   DEIMOS\_COSMOS\_420065 & 5.7256999015808105 & -2.4478572162822463 & 0.10521420637231943 & 1.3472801096521094E-8 & 8.180985539623153E-9 & 0.0019034826221271137 & 0.0017177192615365775 & 0.0026723761305137493 & 0.002411575446023436 & 0.0016650039202417877 & 0.001502514008316615 & 1173571.545672977 & 869876.9329095861 & 1647624.4908408492 & 1221255.3584515203 & 1026540.0910496118 & 760893.9984983186 & 0.3117121794795826 & 0.2117562774396687 & -0.4158225636999721 & 0.3103200875675253 & 192.55594397763073 & 131.32285008728132 & 1.8725114940956097E10 & 1.3914158412063051E10 & 3.907972022418867E10 & 3.3400106380858607E9 & 8.306509249724567 & 2.67602943224018 & 6.165391435838423E8 & 3.173419494247344E8\\
%   DEIMOS\_COSMOS\_421062 & 5.579999923706055 & -2.115672069608623 & 0.20858317493862438 & 2.3241582849769056E-9 & 5.948306541638562E-10 & 3.848127119533396E-4 & 2.1167444025731364E-4 & 5.402541080165923E-4 & 2.9717829572374654E-4 & 3.36601273115483E-4 & 1.8515470997553326E-4 & 3289689.193857818 & 1670709.1411721574 & 4618527.522279411 & 2345576.0394125865 & 2877538.9596304595 & 1461393.5726541504 & 0.27289216982424175 & 0.12672439112256756 & -0.444264498035276 & 0.23363611837690457 & 735.6615289278029 & 158.64814246204813 & 5.251395834558287E10 & 2.673591221963631E10 & 1.280136889006537E11 & 7.397853013819422E9 & 19.868778128698438 & 2.868804049628349 & 8.548805929926527E9 & 1.8064973297096176E9\\
%   DEIMOS\_COSMOS\_422677 & 4.4380998611450195 & -1.2079021154450968 & 0.15395633209932366 & 5.744227842663182E-9 & 1.066115722377555E-9 & 0.0029197756153196783 & 5.592665627376246E-4 & 0.0040991909094063375 & 7.851769149246751E-4 & 0.0025539701750999216 & 4.891985924083266E-4 & 2.719928077055571E7 & 2673342.604591142 & 3.8186168790523745E7 & 3753213.6527788793 & 2.3791606282239065E7 & 2338411.6382526127 & 1.5479198204348592 & 0.1067541208128697 & 0.6440898346513165 & 0.056524938372073306 & 370.5681052336352 & 69.74224529350612 & 4.3515340175514703E11 & 4.277862754674669E10 & 9.839617597569228E10 & 4.919808798784615E9 & 53.51057289569603 & 4.60864389414925 & 9.315538025540272E9 & 1.5315169234221966E9\\
%   DEIMOS\_COSMOS\_430951 & 5.6880998611450195 & -2.617968723182169 & 0.19956020207035163 & 8.291671392227032E-8 & 3.3476844885245633E-8 & 0.025016125382209226 & 0.010438840858297932 & 0.035121148768171254 & 0.01465551028187119 & 0.021881968527820348 & 0.009131005846758673 & 1.8254676044041414E7 & 2685525.2133869217 & 2.562847696284337E7 & 3770317.3092949796 & 1.5967630501458343E7 & 2349067.9432632034 & 1.918929696176399 & 0.20469115443857447 & 0.8504746036272177 & 0.0968879104915537 & 27.041172892465042 & 13.863423912763915 & 2.9188935249145306E11 & 4.299748230704354E10 & 4.110682280120523E10 & 5.3360190549469795E9 & 60.5056829609571 & 6.206710649228298 & 7.297163635509931E8 & 2.8494811829335314E8\\
%   DEIMOS\_COSMOS\_431067 & 4.429999828338623 & -2.262704626019596 & 0.15702551648514945 & 2.614673587683262E-9 & 1.1113405720687E-9 & 5.71262165298056E-4 & 5.17673996586565E-4 & 8.020180258342161E-4 & 7.267834314765856E-4 & 4.99691320346374E-4 & 4.528169701705349E-4 & 1639265.7317912509 & 1424457.8669446746 & 2301431.3670553435 & 1999853.9299988786 & 1433889.5653801188 & 1245994.0033661916 & 0.3672947589872908 & 0.25272813980291997 & -0.33912012058380303 & 0.3317334137005844 & 703.4812335810293 & 219.42944389736402 & 2.6188865280170994E10 & 2.279258421893273E10 & 4.242461068571554E10 & 2.8316197303988843E9 & 7.502938357334696 & 2.539559456867156 & 2.869550674576819E9 & 7.377221653003802E8\\
%   DEIMOS\_COSMOS\_432340 & 4.4045000076293945 & -1.8449521217962732 & 0.15577108521852837 & 2.836463678421567E-9 & 5.88786997253333E-10 & 0.001152652693841814 & 2.8028386013341625E-4 & 0.0016182556698904988 & 3.9350183126535325E-4 & 0.0010082420672583984 & 2.451683669069372E-4 & 1.829243155408105E7 & 2893898.5123569234 & 2.568148344824671E7 & 4062860.999439923 & 1.6000655794936713E7 & 2531335.0969664846 & 0.8929247694099265 & 0.11195023317157515 & 0.25109860499958503 & 0.08099322788204512 & 638.8705613925509 & 109.38083357257051 & 2.925758280539894E11 & 4.631291240390948E10 & 1.6213121102374402E11 & 8.106560551187203E9 & 45.014268365804995 & 4.267484342261334 & 1.5869855379517673E10 & 2.930598325871077E9\\
%   DEIMOS\_COSMOS\_434239 & 4.48829984664917 & -0.6697443298730388 & 0.2236282507279446 & 1.5771047671474174E-9 & 2.668634110181267E-10 & 9.651758309412552E-4 & 1.6540402249721908E-4 & 0.001355049330302706 & 2.322173874740052E-4 & 8.442533299536994E-4 & 1.4468130293402784E-4 & 3.1756129300874725E7 & 2501483.9652624056 & 4.458371248292841E7 & 3511934.368047896 & 2.7777547933994547E7 & 2188084.3881461723 & 1.6096516684527218 & 0.09128522625796914 & 0.700830669663764 & 0.04611403228196056 & 930.5697912273494 & 114.78719350460923 & 5.081467909821187E11 & 4.003235209457422E10 & 1.0101978028296602E11 & 5.050989014148301E9 & 51.88976070579576 & 3.837386395028361 & 3.290191101232366E10 & 5.007509944925911E9\\
%   DEIMOS\_COSMOS\_442844 & 4.491199970245361 & -2.371497012530034 & 0.09388448747878685 & 4.235010993792338E-9 & 1.753423153819355E-9 & 7.079664094589014E-4 & 6.244737110316302E-4 & 9.939426353833812E-4 & 8.767238639822086E-4 & 6.192685099648135E-4 & 5.462362329285125E-4 & 1479866.6984168033 & 1221709.876915486 & 2077644.6263385734 & 1715207.8382693059 & 1294460.913725487 & 1068647.389167789 & 0.2905046075893224 & 0.19436888811643352 & -0.4490882530796177 & 0.29310012208284586 & 489.66474150857914 & 174.15839375455846 & 2.3624394129562946E10 & 1.954677102844426E10 & 5.19380777582727E10 & 2.5969038879136353E9 & 8.852470475163349 & 2.4230329586709574 & 2.0903063742075913E9 & 6.493507114508816E8\\
%   DEIMOS\_COSMOS\_454608 & 4.583399772644043 & -1.189441582801063 & 0.13591867378159248 & 1.2872291573212733E-8 & 3.3758187917092995E-9 & 0.005641912907940641 & 0.0014625463500440776 & 0.007920909395416129 & 0.0020533278897288476 & 0.004935063236293943 & 0.0012793105532203225 & 2.6349389671217732E7 & 1880031.269027059 & 3.699297235100552E7 & 2639451.8287500683 & 2.3048194182897177E7 & 1644490.6807760494 & 1.4799172283336426 & 0.08582033850474134 & 0.6059389059384968 & 0.046741247335558046 & 178.93913043679575 & 54.52346952810851 & 4.2148836048968695E11 & 3.008021107867379E10 & 1.0430685831347493E11 & 5.215342915673746E9 & 60.11738078174587 & 4.909342080664352 & 4.670293586796175E9 & 1.1639130528117607E9\\
%   DEIMOS\_COSMOS\_460378 & 5.389999866485596 & -1.461590816969162 & 0.21277213264813277 & 1.35988353584366E-9 & 1.8211363775553246E-10 & 5.911174466193027E-4 & 1.1868679066071894E-4 & 8.298936571905142E-4 & 1.666291788965997E-4 & 5.170590235515845E-4 & 1.0381706112461526E-4 & 1.3373566507732779E7 & 2290336.167382579 & 1.87756901479695E7 & 3215495.4468277846 & 1.1698053034025742E7 & 2003390.3399139554 & 0.8645344138221998 & 0.12557642041481168 & 0.24497773434204226 & 0.09407778286847875 & 1014.1004178377698 & 72.45057966193437 & 2.1391976170811414E11 & 3.666011836421811E10 & 1.2004736394642264E11 & 6.002368197321133E9 & 30.76629359087187 & 2.564792760849189 & 2.2624212132831455E10 & 2.371193267900623E9\\
%   DEIMOS\_COSMOS\_488399 & 5.670400142669678 & -1.6429269760218148 & 0.29852849960342265 & 3.7352355591308355E-9 & 1.0817489908858496E-9 & 0.0020655115472662756 & 5.915743152099204E-4 & 0.002899855082494316 & 8.3053507345676E-4 & 0.0018067329764533935 & 5.174586531492341E-4 & 3.146789747611114E7 & 2705539.919665494 & 4.417905218311866E7 & 3798416.763787678 & 2.7525427366887122E7 & 2366575.097796126 & 1.6626521170745503 & 0.12451294466038502 & 0.7094843860530239 & 0.06387073364151429 & 521.7150428387604 & 141.0001451810792 & 5.034883206590015E11 & 4.329213828243986E10 & 9.827579438201823E10 & 7.477856554041738E9 & 56.90600460666469 & 5.4688847231369175 & 1.5234917237697947E10 & 4.162118499539819E9\\
%   DEIMOS\_COSMOS\_493583 & 4.513400077819824 & -1.5697456400110812 & 0.1471610848848542 & 1.824504915199194E-8 & 3.3234847441798055E-9 & 0.007400015388719851 & 0.001382762347521896 & 0.010389180473920161 & 0.0019413159062945762 & 0.006472901033527438 & 0.00120952232640501 & 2.245473784749223E7 & 2138457.683242392 & 3.1525113359597914E7 & 3002267.1089187763 & 1.9641485616662234E7 & 1870540.0219997296 & 1.4130341538827615 & 0.09737026078187411 & 0.5702899926844195 & 0.05440174650486217 & 126.53984844787571 & 27.83301046902127 & 3.591555295661476E11 & 3.4213718285503895E10 & 9.62651121390684E10 & 4.813255606953421E9 & 55.36310050747914 & 4.741457436500925 & 3.034417723201078E9 & 4.878423587454392E8\\
%   DEIMOS\_COSMOS\_494057 & 5.5447998046875 & -2.1268652065556517 & 0.2641998157462262 & 7.239977508432832E-9 & 2.207499273044429E-9 & 0.0024242077038956395 & 7.600617029194784E-4 & 0.0034034431037036432 & 0.0010670813218824368 & 0.0021204897189741933 & 6.648370204569543E-4 & 2.065895383840736E7 & 2368553.669637805 & 2.9003939661634825E7 & 3325308.157269916 & 1.807068723884854E7 & 2071808.3261737614 & 0.8067570829799023 & 0.08316184296162879 & 0.18115567341605038 & 0.06416072494094793 & 303.9293702491044 & 97.60843471835483 & 3.303351274216016E11 & 3.790129982035761E10 & 2.164903455404435E11 & 1.0824517277022175E10 & 61.69865762635176 & 5.452638352152939 & 8.521940510794084E9 & 2.4868352853148236E9\\
%   DEIMOS\_COSMOS\_494763 & 5.233699798583984 & -2.051448225400101 & 0.5308575688725958 & 2.8571752778877447E-8 & 8.998378716853658E-9 & 0.011128055733742419 & 0.0034159585594717282 & 0.015623126881320164 & 0.0047958021843956524 & 0.009733872117332586 & 0.0029879886092934885 & 1.931051594305937E7 & 1275512.986241293 & 2.7110813240033302E7 & 1790744.1964363337 & 1.689118900972992E7 & 1115709.7510235324 & 1.6226646421746949 & 0.13431599788830437 & 0.6863049242462713 & 0.06910404394663594 & 81.90539650605652 & 33.32556747140378 & 3.08853797499079E11 & 2.0416721578533714E10 & 6.378824087400648E10 & 5.982927971637324E9 & 49.58056472387136 & 4.786651723963528 & 1.735300074433142E9 & 5.20203689416958E8\\
%   DEIMOS\_COSMOS\_510660 & 4.547999858856201 & -1.5901623712670205 & 0.14716858640243205 & 4.033039722892525E-8 & 1.1137735653742469E-8 & 0.013284126441590704 & 0.003771637497582179 & 0.01865012162683294 & 0.0052951542106677236 & 0.011619818507993226 & 0.003299106146914901 & 1.750876525297564E7 & 1871769.2161645843 & 2.458126267763532E7 & 2627852.3990510223 & 1.5315171489309698E7 & 1637263.7430329076 & 1.3301692457694525 & 0.10730634749068742 & 0.5319090949742561 & 0.06076515940285458 & 56.37202750773254 & 18.935861022022117 & 2.7997223719839246E11 & 2.995575450855054E10 & 8.190210790534369E10 & 4.0951053952671843E9 & 53.15633366976259 & 4.473765786753803 & 1.3180215748442588E9 & 3.466730192117591E8\\
%   DEIMOS\_COSMOS\_519281 & 5.575900077819824 & -2.359808562557726 & 0.22766515225618392 & 2.8958169424063046E-8 & 1.3460313798362593E-8 & 0.008835991736474431 & 0.004236335487973937 & 0.012405205664333162 & 0.005947562487467696 & 0.007728970419500638 & 0.0037055842343618637 & 1.778976366286424E7 & 2702585.6254237057 & 2.4975767694161013E7 & 3794269.1107844436 & 1.5560964883274812E7 & 2363990.933676661 & 1.0526956990037557 & 0.14818706819210944 & 0.3593531341464988 & 0.09751862405321958 & 81.414222688316 & 45.57687805951204 & 2.8442716392095264E11 & 4.3278619868266556E10 & 1.2295370580521664E11 & 7.8313893579916725E9 & 58.30233951404894 & 5.614141205097417 & 2.0133295948466306E9 & 9.15532618077347E8\\
%   DEIMOS\_COSMOS\_536534 & 5.688600063323975 & -1.093142448135695 & 0.2434660299382998 & 1.436627483117639E-9 & 1.1589634043590338E-10 & 5.693021629632652E-4 & 5.503821699853468E-5 & 7.992662993963921E-4 & 7.727037571194495E-5 & 4.97976877811846E-4 & 4.81427284916704E-5 & 1.2705094610069811E7 & 928282.4382054829 & 1.7837195452789437E7 & 1303253.206201205 & 1.1113330947655162E7 & 811982.1430135024 & 0.7657631473139965 & 0.058621176821294 & 0.17054306446894385 & 0.047154636304888344 & 983.0510440450836 & 40.293271991899324 & 2.032024110445151E11 & 1.4861551295130436E10 & 1.3701226472910329E11 & 6.850613236455165E9 & 32.061160627653955 & 1.6030580313826979 & 2.231696177639434E10 & 1.4128687414003465E9\\
%   DEIMOS\_COSMOS\_539609 & 5.18179988861084 & -2.3850847408020535 & 0.223196134091524 & 2.7089791773331667E-8 & 6.240810452084417E-9 & 0.006893963021636166 & 0.0018088958314191794 & 0.009678713117473701 & 0.0025395819148947407 & 0.006030249671625114 & 0.0015822674794142848 & 1.4323282791161872E7 & 2186430.55913451 & 2.0109035195144117E7 & 3069618.166898455 & 1.2528783673037218E7 & 1912502.5939177175 & 0.7395103485063235 & 0.09686972953696416 & 0.13353618331969366 & 0.08012782013744693 & 84.9133918318164 & 23.505795216929023 & 2.2892067902075375E11 & 3.498554465233873E10 & 1.6646662388757822E11 & 8.323331194378911E9 & 56.28326509808159 & 4.882908756797511 & 2.0776558774988153E9 & 4.4340329924160415E8\\
%   DEIMOS\_COSMOS\_549131 & 5.549300193786621 & -2.5128888666346865 & 0.05829519041907302 & 1.3052097998739415E-8 & 5.103563179672755E-9 & 0.0011753561111490106 & 7.018268472766374E-4 & 0.0016501299143871708 & 9.853230560728263E-4 & 0.0010281010764134832 & 6.138981456740092E-4 & 1954095.532140185 & 929851.191958852 & 2743433.6390207745 & 1305455.6429539358 & 1709275.7683831893 & 813354.3547263335 & 0.18085082109960485 & 0.08053273466425973 & -0.6312316885688182 & 0.18088603220282826 & 182.3345143892831 & 85.69318901540666 & 3.1110027162152763E10 & 1.4875997830970085E10 & 1.220312220222659E11 & 6.101561101113296E9 & 21.699845810525616 & 3.274649063517203 & 1.6625561509438107E9 & 5.997192074643116E8\\
%   DEIMOS\_COSMOS\_550156 & 4.419000148773193 & -1.9303005739836214 & 0.21442690889435806 & 5.1965469242945945E-9 & 2.5783415096521696E-9 & 0.001366025810206704 & 0.0011263547696272905 & 0.0019178188056073145 & 0.0015813349519727185 & 0.0011948826339186513 & 9.852388906586179E-4 & 5006189.341432625 & 3900097.184216129 & 7028391.404974692 & 5475503.952926058 & 4378986.591242621 & 3411471.7022145577 & 0.5122917939402999 & 0.31229476632335407 & -0.1676397119552201 & 0.36179980272846246 & 448.25321539933094 & 194.31803355925746 & 8.001310969909865E10 & 6.239637153194189E10 & 8.550095001717651E10 & 4.275047500858826E9 & 19.044221295292786 & 7.926272241137865 & 3.6647838598855615E9 & 9.898561112648673E8\\
%   DEIMOS\_COSMOS\_552206 & 5.5015997886657715 & -1.1266694229692646 & 0.3589958628425009 & 1.7949832604826522E-9 & 3.3961039236127077E-10 & 0.0010146095345670478 & 2.0094033277620125E-4 & 0.001424451303337182 & 2.8210824870496243E-4 & 8.874937091261862E-4 & 1.7576543012154822E-4 & 4.691714645845064E7 & 4725649.035646266 & 6.586887678925621E7 & 6634529.539299919 & 4.103911003536433E7 & 4133593.90759514 & 1.4228393485013477 & 0.11676359472215944 & 0.5946695681964399 & 0.06426919513656726 & 861.1613227139202 & 122.21955679174143 & 7.506913421203204E11 & 7.563206988941359E10 & 1.9036501066594482E11 & 1.1057842918163239E10 & 83.00285937926664 & 6.8037687436905205 & 4.62415785186476E10 & 7.885161116061943E9\\
%   DEIMOS\_COSMOS\_567070 & 4.561999797821045 & -2.2093269967758657 & 0.19532470024606408 & 4.240471603452628E-9 & 2.109848124881241E-9 & 0.0010341420815408676 & 9.4868462570771E-4 & 0.0014518738349086255 & 0.0013318966612332712 & 9.045791119061572E-4 & 8.298282330055169E-4 & 4589732.120936626 & 4037525.610251816 & 6443710.2933657365 & 5668445.270657362 & 4014705.4064929704 & 3531682.344246254 & 0.44602173514156246 & 0.3053867697509566 & -0.25207748937968993 & 0.3672559028088388 & 518.7480623236362 & 201.39413975690113 & 7.334495374368062E10 & 6.459675914927969E10 & 9.215286522546547E10 & 4.607643261273273E9 & 18.820072283768706 & 7.981313445168962 & 4.438202644358058E9 & 1.1548551488393025E9\\
%   DEIMOS\_COSMOS\_586681 & 5.866099834442139 & -2.3403816697948785 & 0.10129599333117063 & 2.820751396126914E-9 & 1.0082768719186267E-9 & 5.284943758504971E-4 & 4.240433005390748E-4 & 7.419745989355901E-4 & 5.953315157658511E-4 & 4.622817132070735E-4 & 3.7091683924114E-4 & 3361663.3699819483 & 2559313.6306549925 & 4719574.975012431 & 3593123.770900467 & 2940495.817765016 & 2238668.8371270252 & 0.31784869764336016 & 0.20661393142352377 & -0.401772029637432 & 0.3012222365597594 & 656.9953511761881 & 190.311422740334 & 5.368362797554869E10 & 4.0953558685739395E10 & 1.0743406543203899E11 & 8.6869702258133E9 & 17.942322714268045 & 4.524905929557459 & 6.360830925725709E9 & 1.6113083086017947E9\\
%   DEIMOS\_COSMOS\_592644 & 4.526700019836426 & -2.351521713051494 & 0.10836996204733183 & 5.510934189834456E-9 & 1.5746606597486168E-9 & 8.324705132381042E-4 & 6.148416973461784E-4 & 0.0011687389751149917 & 8.632010909542001E-4 & 7.281740594396537E-4 & 5.378109705385789E-4 & 2458946.9393064114 & 1755595.94714986 & 3452214.9193350878 & 2464752.0547086243 & 2150876.6331875212 & 1535645.2958307648 & 0.2688992146379227 & 0.16062109252076445 & -0.4761375920078587 & 0.26694679896141865 & 394.0019843776134 & 105.73333605930061 & 3.9240770632799286E10 & 2.808807983255025E10 & 9.609231240420287E10 & 4.804615620210143E9 & 16.27816786699398 & 3.487240917993175 & 2.9537946392139664E9 & 5.584951461031474E8\\
%   DEIMOS\_COSMOS\_627939 & 4.53410005569458 & -1.3184890020869506 & 0.2525273166718043 & 4.669811141145712E-9 & 9.35957837970062E-10 & 0.0023567101778112056 & 4.743973017013513E-4 & 0.0033086806007630054 & 6.660255316805092E-4 & 0.00206144865170581 & 4.149622160470287E-4 & 2.3197455324505925E7 & 1840854.8552748775 & 3.2567844422237594E7 & 2584450.479237633 & 2.029115139058875E7 & 1610222.5021648342 & 1.4448504273773695 & 0.08612109405107515 & 0.59042277513708 & 0.046738117549243514 & 439.11519143371345 & 88.09398401714998 & 3.711261130733765E11 & 2.945541329672427E10 & 9.512625003922081E10 & 4.756312501961041E9 & 45.96565854407141 & 3.545091597717188 & 9.843151501153425E9 & 1.8209268151436715E9\\
%   DEIMOS\_COSMOS\_628063 & 4.532700061798096 & -1.6698914759212593 & 0.19432179840056416 & 1.945020118240048E-9 & 3.624000112007472E-10 & 8.709144271961256E-4 & 2.0327162333234238E-4 & 0.0012227119385824143 & 2.853812416722224E-4 & 7.618015098326676E-4 & 1.7780464386065763E-4 & 8323251.99733286 & 1454877.5804370977 & 1.1685349636166973E7 & 2042561.394353544 & 7280469.5160458665 & 1272602.5689652395 & 0.9681567436146318 & 0.14346374681530263 & 0.30973172181012004 & 0.09900776856796739 & 822.2256802166781 & 117.63047073289515 & 1.331414188337876E11 & 2.3285308754386086E10 & 6.435197604589956E10 & 3.7906653435275297E9 & 18.58838489576246 & 1.931236475145012 & 9.556911376619675E9 & 1.4781348798132474E9\\
%   DEIMOS\_COSMOS\_629750 & 5.118100166320801 & -2.283444199482142 & 0.17966581761352055 & 4.375289613760172E-9 & 2.2138425299642445E-9 & 0.001025687314118095 & 9.609439394604397E-4 & 0.0014400038454550764 & 0.0013491080069363717 & 8.971836039356573E-4 & 8.405516329570011E-4 & 3150352.260796174 & 2819344.9739538124 & 4422906.774454131 & 3958192.2758288984 & 2755658.918759453 & 2466122.033150667 & 0.429764092896687 & 0.3037547346510323 & -0.2741380738242374 & 0.3679132802813066 & 508.00067913745784 & 211.2508333021153 & 5.033886253468879E10 & 4.510723514815049E10 & 6.676965607098185E10 & 6.655697940622083E9 & 13.438504441481623 & 5.6885181842253685 & 3.071454835633709E9 & 8.514118433893518E8\\
%   DEIMOS\_COSMOS\_630594 & 4.440299987792969 & -1.4474870055520621 & 0.26433593440545705 & 1.4424303578206836E-8 & 3.3010436449476093E-9 & 0.006780177796141616 & 0.0015086664637719903 & 0.009518965443876894 & 0.002118077780077373 & 0.005930720080804731 & 0.001319652487139929 & 2.6742184599127803E7 & 1826020.98682368 & 3.754443301438721E7 & 2563624.6122129783 & 2.3391777616346397E7 & 1597247.1017926496 & 1.8027723118408547 & 0.09964507591795922 & 0.7734541405995662 & 0.0499033727115786 & 160.51450924414985 & 45.05624846994453 & 4.2780767159912524E11 & 2.921230830837131E10 & 7.205212499163188E10 & 3.7339988320779953E9 & 56.891928294532015 & 4.935137472925255 & 3.944171584164936E9 & 8.35278413319002E8\\
%   DEIMOS\_COSMOS\_665509 & 4.525599956512451 & -2.17225247751762 & 0.2570547408500491 & 2.038325393172115E-8 & 5.120966281004297E-9 & 0.0075483813753311185 & 0.0018665380268037314 & 0.010597477474686577 & 0.002620508121031547 & 0.00660267891879242 & 0.0016326879456538832 & 2.337249486988396E7 & 1953270.076997232 & 3.281358950944071E7 & 2742274.7492073383 & 2.0444261025456905E7 & 1708553.73077012 & 1.2474620276685255 & 0.08142228623083081 & 0.4773348078739305 & 0.04902184817208737 & 114.4090866708703 & 36.29597349136465 & 3.737894624596558E11 & 3.124502369816657E10 & 1.2422265824000568E11 & 6.211132912000284E9 & 63.11386166942266 & 5.973176155403287 & 3.096358504919698E9 & 7.206041799018271E8\\
%   DEIMOS\_COSMOS\_680104 & 4.5295000076293945 & -1.7241320352560554 & 0.31437549640425466 & 5.682530157210349E-8 & 1.2815642674075968E-8 & 0.01717257541903374 & 0.003971868581243077 & 0.02410927219182582 & 0.005576266715894762 & 0.01502110135441497 & 0.003474251186525036 & 1.6805519421282746E7 & 1949690.0865317408 & 2.359394745203097E7 & 2737248.6560052074 & 1.4700032137339208E7 & 1705422.2610681218 & 1.3407810294707392 & 0.11032701668181744 & 0.5425469200022175 & 0.06315403917939219 & 39.39605005515889 & 11.196907825514451 & 2.6869678063232315E11 & 3.1191811583654434E10 & 7.660983918803207E10 & 3.8304919594016037E9 & 55.61068656782574 & 5.7862377307220925 & 9.786254543192072E8 & 1.9581376112068415E8\\
%   DEIMOS\_COSMOS\_683613 & 5.541999816894531 & -1.9099271523067591 & 0.28133955770432223 & 6.2586385558098475E-9 & 1.8436862887315383E-9 & 0.003164294720805884 & 9.272264930057013E-4 & 0.004442481157165833 & 0.00130177072208802 & 0.0027678545912095845 & 8.110584923971219E-4 & 3.3411487413945332E7 & 3129937.4241996496 & 4.6907736593996316E7 & 4394245.560847712 & 2.922551373921247E7 & 2737801.764420778 & 1.594377436958108 & 0.13636341817806816 & 0.6680202835142665 & 0.07184354503108406 & 345.36877290192257 & 106.25750745998157 & 5.34538239312985E11 & 5.008559057792262E10 & 1.1478515027842117E11 & 9.694294747172087E9 & 66.08437006860643 & 6.504954195545806 & 1.0558905020527317E10 & 2.9316826981640115E9\\
%   DEIMOS\_COSMOS\_709575 & 4.412099838256836 & -1.6634274433517835 & 0.25446762761498193 & 1.0077213361323521E-8 & 2.182547634316106E-9 & 0.004563457972886087 & 0.0010169469871826203 & 0.00640682295576484 & 0.0014277329474685493 & 0.003991723027249458 & 8.895383129082571E-4 & 1.7791538034404673E7 & 1898764.208999201 & 2.497825880602943E7 & 2665751.759757559 & 1.5562516951855024E7 & 1660876.6556878749 & 1.448375181500576 & 0.11915053631665301 & 0.5876383307417697 & 0.06549045938499418 & 225.35782778498444 & 55.29893398880205 & 2.846059511967496E11 & 3.0382633521800156E10 & 7.325332819103397E10 & 3.6626664095516987E9 & 39.28799736166077 & 3.6513598275127492 & 3.898696589321868E9 & 7.626953944119474E8\\
%   DEIMOS\_COSMOS\_722679 & 5.716800212860107 & -2.7550662761501568 & 0.09962463394948656 & 1.576415671513804E-7 & 2.476250731978204E-8 & 0.020686249014220785 & 0.008610805670472158 & 0.02904226046134901 & 0.012089057851522407 & 0.018094562725918792 & 0.007531996894069329 & 3582814.9125543707 & 1418543.7326603928 & 5030058.557434847 & 1991550.8380188188 & 3133940.286902919 & 1240820.8241347673 & 0.6788443717213373 & 0.3015093317472547 & 0.0733308176260186 & 0.2803513364887993 & 13.130561064810742 & 1.7175994941014494 & 5.718385644323655E10 & 2.2701534249100113E10 & 4.459971274792377E10 & 8.035315677066664E9 & 27.30318856937931 & 2.467082965679748 & 1.731979011802169E8 & 2.2254248759487465E7\\
%   DEIMOS\_COSMOS\_733857 & 4.54449987411499 & -1.6475478354922082 & 0.12954163577416267 & 1.4450269678191539E-8 & 3.0307737697444937E-9 & 0.005524072705582775 & 0.0012286065780649355 & 0.007755468776029671 & 0.0017248903955550028 & 0.004831986698264571 & 0.0010746800339196158 & 2.0538529102915406E7 & 2515762.9190864363 & 2.8834870511798028E7 & 3531981.1680157394 & 1.7965349972115774E7 & 2200574.3966272566 & 1.1695048371440564 & 0.10418471830380396 & 0.42761734467017126 & 0.06446951519762525 & 159.77216451567173 & 39.093758759725375 & 3.28478370287196E11 & 4.025137513899296E10 & 1.2187953768908891E11 & 6.093976884454446E9 & 53.72617272588969 & 5.244260324252921 & 3.718004848516679E9 & 6.902106259150685E8\\
%   DEIMOS\_COSMOS\_742174 & 5.636000156402588 & -2.320944979772318 & 0.20770081158763865 & 9.646381427708972E-9 & 2.9959570467931522E-9 & 0.003031237864032469 & 0.0011068845407636212 & 0.0042556772620795155 & 0.0015539999113130018 & 0.002651467824360504 & 9.682079984355058E-4 & 6835063.13932728 & 1488045.4000760356 & 9596021.193868726 & 2089127.0359170232 & 5978729.088349979 & 1301614.942959488 & 0.7808549754740758 & 0.16819743028749792 & 0.15300753624640007 & 0.1369377290988812 & 235.06080544549337 & 79.26848506984972 & 1.0928101085202443E11 & 2.3817755834130703E10 & 7.517335669739558E10 & 6.334260769265904E9 & 21.751386424262023 & 2.2303642314463525 & 2.2548752179528947E9 & 6.610464446744823E8\\
%   DEIMOS\_COSMOS\_761315 & 4.584700107574463 & -2.115708431316073 & 0.3005496233965986 & 8.309400580054975E-9 & 6.893974597595995E-9 & 0.002385548380140682 & 0.00241255805479634 & 0.003349167717722391 & 0.0033870876908304527 & 0.0020866738465004165 & 0.002110299601557677 & 4390591.433428487 & 3983398.9161957595 & 6164128.639336162 & 5592454.618818689 & 3840514.152248594 & 3484336.9381230543 & 0.6699242326754813 & 0.4638525218006766 & -0.04783939090055828 & 0.4564400269514436 & 373.83784679854284 & 253.81250944338655 & 7.018893619115111E10 & 6.3714007983937225E10 & 4.8744860819108444E10 & 3.284950641114054E9 & 15.293415680617455 & 10.690956614848806 & 1.8404956570906193E9 & 8.223857892650113E8\\
%   DEIMOS\_COSMOS\_773957 & 5.677299976348877 & -1.510970074483927 & 0.37396479991891096 & 3.2720298189252433E-9 & 8.815746564201839E-10 & 0.0015051845401203015 & 4.082256680990842E-4 & 0.002113189366835834 & 5.731245027453519E-4 & 0.0013166067979055477 & 3.570809262071153E-4 & 1.457157835071596E7 & 1180033.2467898673 & 2.045762735929185E7 & 1656696.33401218 & 1.2745971408417856E7 & 1032192.2349494232 & 1.1320137062019733 & 0.10777274806802137 & 0.41080117730057386 & 0.06797012560884319 & 574.0766514015497 & 138.67626338461648 & 2.3309971357601837E11 & 1.8886783027534164E10 & 9.063943668772176E10 & 8.05569339514135E9 & 31.67627463708698 & 2.368889780462339 & 9.68092480510817E9 & 2.505816306130869E9\\
%   DEIMOS\_COSMOS\_787780 & 4.510900020599365 & -1.7407812468038224 & 0.33232798286255927 & 2.159755466515321E-9 & 1.130321039029327E-9 & 0.001046743535607747 & 6.877177499681422E-4 & 0.001469565525217025 & 9.655147245272596E-4 & 9.15601786964075E-4 & 6.015567131562457E-4 & 6862818.382032373 & 4223518.253165666 & 9634987.900073176 & 5929567.853861564 & 6003007.0026183 & 3694372.812752675 & 1.1068429879878152 & 0.48172337119714415 & 0.36065362917192545 & 0.33121427493050126 & 829.2651977596959 & 273.03091633709363 & 1.0979018025212015E11 & 6.7586852201340225E10 & 3.968645544265296E10 & 6.118225536989821E9 & 14.160115646370322 & 6.656544746826161 & 6.556351339726947E9 & 1.5081868587196364E9\\
%   DEIMOS\_COSMOS\_803480 & 4.5416998863220215 & -2.3172562331853697 & 0.17267229192105335 & 1.4037902029364516E-8 & 3.7545884775291125E-9 & 0.003156140601161254 & 0.0011361475071550368 & 0.004431033259270494 & 0.0015950833716941927 & 0.002760722064221102 & 9.938047405298272E-4 & 4367573.883786434 & 1159114.5286172559 & 6131813.3717674995 & 1627327.700710469 & 3820380.366973711 & 1013894.328071288 & 0.5286360237434305 & 0.1270573409776055 & -0.07419427972172797 & 0.1447942438014671 & 165.16502117824686 & 51.11887208905175 & 6.978301631043822E10 & 1.8547978635398613E10 & 7.955682120153572E10 & 3.977841060076787E9 & 19.426122608113968 & 2.1616329877478195 & 1.3838337500488577E9 & 3.3656832166070056E8\\
%   DEIMOS\_COSMOS\_814483 & 4.580999851226807 & -1.6407769332404405 & 0.25132565851097577 & 9.72317472689613E-9 & 1.795158462432887E-9 & 0.00424254559937084 & 8.076506987500976E-4 & 0.005956281113670001 & 0.0011338934351397395 & 0.0037110163090762764 & 7.064638069047371E-4 & 3.1652751332301673E7 & 3069992.0015198737 & 4.443857597764899E7 & 4310085.760889058 & 2.768712172209227E7 & 2685366.6317843464 & 1.326958101933003 & 0.09184954924795503 & 0.5200377986411003 & 0.05286492996758515 & 232.61097280752728 & 49.10815871085433 & 5.063164896091518E11 & 4.911969008526716E10 & 1.522935965394965E11 & 7.614679826974825E9 & 72.54258665754926 & 6.1782965596202395 & 7.460792251000368E9 & 1.2221471167246208E9\\
%   DEIMOS\_COSMOS\_818760 & 4.561299800872803 & -0.7748529833838228 & 0.2018656566088453 & 3.735515015375504E-9 & 7.364576900387327E-10 & 0.0024057820542890316 & 4.6049995173409253E-4 & 0.00337757459005108 & 6.465144807792953E-4 & 0.0021043725354121384 & 4.0280600200678695E-4 & 1.3313894416916108E8 & 1.0538523457039233E7 & 1.8691914089652708E8 & 1.4795458708196277E7 & 1.1645856988743356E8 & 9218199.66495003 & 2.4280357129894536 & 0.10180469334370412 & 1.080263479775328 & 0.044687686563119576 & 523.6133072485724 & 98.04841961391321 & 2.1305267077009385E12 & 1.6862670470005267E11 & 1.7676460894118237E11 & 8.838230447059118E9 & 206.7280052191258 & 19.05306947325863 & 5.534123256585142E10 & 9.644922032483936E9\\
%   DEIMOS\_COSMOS\_834764 & 4.505799770355225 & -2.0297832550855683 & 0.33536445191230724 & 7.881563984550581E-9 & 1.51293867574974E-9 & 0.003418197393744055 & 6.859514410900982E-4 & 0.004798945374251971 & 9.630349321561983E-4 & 0.002989946950177123 & 6.000116971040297E-4 & 2.4359951589288116E7 & 2571930.3629978867 & 3.419991987893062E7 & 3610836.9109976203 & 2.130800377244335E7 & 2249704.8763150717 & 1.2378389885832637 & 0.09308459403615164 & 0.4683967114469811 & 0.05546999439511233 & 281.755329942014 & 59.40676990415375 & 3.896572991839848E11 & 4.1152024990516464E10 & 1.3186944140637561E11 & 6.59347207031878E9 & 56.16835278820205 & 4.936594849695832 & 7.126549108565647E9 & 1.2161954729185119E9\\
%   DEIMOS\_COSMOS\_838532 & 4.526299953460693 & -2.1002120948010337 & 0.2605960802305365 & 1.2933635549351951E-8 & 7.706522891676501E-9 & 0.0029481463854594586 & 0.0025022903610939532 & 0.004139021779436092 & 0.0035130664997242897 & 0.0025787865001632025 & 0.0021887897543024933 & 4390713.830657489 & 3366209.2327219583 & 6164300.477749302 & 4725957.095310131 & 3840621.214884073 & 2944472.1499862894 & 0.5255022982864541 & 0.3257699044745909 & -0.15793249884577304 & 0.37912762249157267 & 218.59148435706905 & 132.68084479504256 & 7.015654351631644E10 & 5.384086453134017E10 & 7.282270190022118E10 & 3.641135095011059E9 & 19.262236355462647 & 9.084117444531005 & 1.4893133707040164E9 & 5.42383843061028E8\\
%   DEIMOS\_COSMOS\_842313 & 4.553699970245361 & -1.6667289096089195 & 0.06193913008783693 & 1.012544978132859E-9 & 8.193772327331343E-11 & 3.864134503138923E-4 & 5.490285266152535E-5 & 5.425014492511334E-4 & 7.708033225216156E-5 & 3.380014622291737E-4 & 4.8024323338315425E-5 & 2.8151128775874842E7 & 3612732.458153164 & 3.952250664815517E7 & 5072061.008002232 & 2.462420156937632E7 & 3160109.598945462 & 0.6828332688778144 & 0.07017363401933992 & 0.1112595893783848 & 0.061807943340567634 & 1183.821734243534 & 20.885643897525096 & 4.502183450189738E11 & 5.782653497815337E10 & 3.457968130156499E11 & 1.7289840650782494E10 & 73.76628336210558 & 3.9244162153270357 & 7.285235219686853E10 & 4.442289683378461E9\\
%   DEIMOS\_COSMOS\_843045 & 5.847300052642822 & -1.848283674407846 & 0.21126805942647955 & 4.643699422347672E-9 & 1.2447867194583378E-9 & 0.001556393379186224 & 5.263960694039043E-4 & 0.002185083524208368 & 7.390287017694202E-4 & 0.0013613999138524177 & 4.6044629405544426E-4 & 1.1091666772776596E7 & 2502193.018277167 & 1.5572038949353341E7 & 3512929.8362123496 & 9702042.164194422 & 2188704.6071255915 & 0.7414485982673216 & 0.17232138766011856 & 0.12154571555283418 & 0.14656645442485716 & 439.91764399268527 & 110.42243544624739 & 1.7735431867451657E11 & 4.0054829585402565E10 & 1.3108835158138489E11 & 1.3177789870677649E10 & 33.09341152077258 & 3.0254694456381594 & 7.126518861559272E9 & 1.7957947335693514E9\\
%   DEIMOS\_COSMOS\_845652 & 5.30709981918335 & -1.6281958368488127 & 0.07408274551710058 & 1.2003827043844046E-9 & 8.487987502892596E-11 & 3.506530224025287E-4 & 4.090410107825093E-5 & 4.922959402244774E-4 & 5.74269195268439E-5 & 3.0672129609064195E-4 & 3.577941183048328E-5 & 1.49128903853181E7 & 1571701.627148871 & 2.093680910948224E7 & 2206575.3917882517 & 1.3044522006690836E7 & 1374790.2608792575 & 0.496810040560636 & 0.049765830337087986 & -0.07522428963790352 & 0.05604060962798447 & 1084.8180690851004 & 23.832898170263018 & 2.3839616555906458E11 & 2.5160358168911743E10 & 2.8207308478456354E11 & 1.4103654239228178E10 & 51.050966474678916 & 2.552548323733946 & 4.252890872903697E10 & 2.1264454364518487E9\\
%   DEIMOS\_COSMOS\_848185 & 5.293099880218506 & -1.1742761704435491 & 0.17332191573233116 & 2.2424504474048817E-9 & 4.1139949388097417E-10 & 0.0010635532373836317 & 2.0874705947402546E-4 & 0.0014931653444455976 & 2.9306842761187376E-4 & 9.30305477467783E-4 & 1.8259408744945605E-4 & 4.077465116439231E7 & 4299841.321245777 & 5.72451795645918E7 & 6036720.891653388 & 3.566618010903539E7 & 3761133.7099003773 & 1.0928996976216476 & 0.08755885823051664 & 0.39273592921554246 & 0.05465708997322299 & 749.0454515847255 & 110.79116668128292 & 6.522891095216304E11 & 6.881081658812764E10 & 2.6287589250661816E11 & 1.3143794625330908E10 & 85.97137551036212 & 6.799245791873712 & 3.8338138356570656E10 & 6.34640272744088E9\\
%   DEIMOS\_COSMOS\_859732 & 4.531799793243408 & -2.3440917859242725 & 0.2919793421040324 & 1.3921030954779599E-8 & 3.8044156633531665E-9 & 0.00667039115136305 & 0.0018011935945117653 & 0.009364831539240785 & 0.0025287684334246905 & 0.005834688106663441 & 0.0015755302208250027 & 2.188894191543447E7 & 1579630.4768659328 & 3.07307695993784E7 & 2217707.02413414 & 1.9146575689993028E7 & 1381725.7409873782 & 1.878305431739698 & 0.1487155663065398 & 0.81041802448198 & 0.07301805601682083 & 166.1854160051192 & 53.771440989837444 & 3.501755766731567E11 & 2.527907259560334E10 & 5.434492957557746E10 & 5.331067128236386E9 & 45.681974423624176 & 3.8159140853565483 & 3.2815079983670235E9 & 8.53869145379221E8\\
%   DEIMOS\_COSMOS\_869970 & 5.2006001472473145 & -2.4365933672788165 & 0.08389852140464332 & 8.784926076689122E-9 & 3.193852363607873E-9 & 0.0011673639292553357 & 8.889361715437941E-4 & 0.0016389093674406936 & 0.0012480133933291415 & 0.001021110198729828 & 7.775653915932121E-4 & 1705731.3083571484 & 1212218.0838663792 & 2394745.074388826 & 1701881.9266558527 & 1492027.9714033287 & 1060344.7798068344 & 0.2538358479090648 & 0.15465740575287193 & -0.5025641129817823 & 0.26174353884476337 & 268.97376642049596 & 109.58592998534928 & 2.7207797836140568E10 & 1.9392131764287315E10 & 7.172271420354193E10 & 5.6106283951645355E9 & 12.836376964440353 & 3.0744615601194103 & 1.461182126335905E9 & 3.996551807236924E8\\
%   DEIMOS\_COSMOS\_873321 & 5.154200077056885 & -1.2892388147909064 & 0.19916908077479117 & 4.96071207856711E-9 & 9.403619595747604E-10 & 0.0021513670764453942 & 4.2302757545001585E-4 & 0.003020391127417337 & 5.939054982905082E-4 & 0.0018818320558964836 & 3.7002836974028304E-4 & 2.692335767306385E7 & 2344382.408870291 & 3.779878921005211E7 & 3291373.1480564647 & 2.355025233780651E7 & 2050665.373006097 & 1.1089537300351193 & 0.07959277224047781 & 0.3923129388073475 & 0.05002000031400593 & 417.7810705581928 & 79.52284523905496 & 4.30659525444403E11 & 3.751465833359988E10 & 1.7404908046128964E11 & 8.702454023064482E9 & 62.081002850068614 & 4.32425704657721 & 1.2514534580285612E10 & 2.2063192087816963E9\\
%   DEIMOS\_COSMOS\_873756 & 4.5457000732421875 & -1.4378127515872585 & 0.2837954379715908 & 2.3970139981650762E-8 & 5.728949867406032E-9 & 0.012393822750133288 & 0.0028331074305707965 & 0.017400188317066054 & 0.003977513944507626 & 0.010841056926852121 & 0.002478160254016497 & 1.2680410173411173E8 & 6340205.086705587 & 1.7802539975216427E8 & 8901269.987608215 & 1.1091739112075563E8 & 5545869.556037781 & 3.5677998484505706 & 0.12121534195116448 & 1.56621467855042 & 0.051041472754076375 & 96.77711718194062 & 29.479196283036366 & 2.028778329734975E12 & 1.0143891648674876E11 & 5.5194308210628265E10 & 3.8936544644622674E9 & 245.24411314349757 & 21.052755770866412 & 1.0231234082539064E10 & 2.282127545456382E9\\
%   DEIMOS\_COSMOS\_880016 & 4.541500091552734 & -1.1185560918155997 & 0.29178408767829844 & 1.497425776117711E-8 & 3.896043670118756E-9 & 0.007051095629804446 & 0.0017913126232175012 & 0.009899317932307803 & 0.002514896138754842 & 0.006167695848205199 & 0.0015668871915955785 & 2.513204742126378E7 & 1567227.816141883 & 3.5283896400625974E7 & 2200294.427828546 & 2.198336722052424E7 & 1370876.9533562642 & 1.8516352890963361 & 0.11212161613819993 & 0.7978511717689168 & 0.055444505974380706 & 154.90152367647747 & 48.723213929144066 & 4.0205075593622437E11 & 2.5075184542772205E10 & 6.4106383157581726E10 & 4.387081009328678E9 & 53.37238011088604 & 4.479375112474236 & 3.564275502807326E9 & 8.777917851804153E8\\
%   DEIMOS\_COSMOS\_881725 & 4.577700138092041 & -0.8548539264834502 & 0.182103025562111 & 7.089692120687676E-9 & 1.2750603579370547E-9 & 0.0038846166578558093 & 6.928980043350001E-4 & 0.005453770216745751 & 9.72787492851517E-4 & 0.0033979306607688857 & 6.060879569555872E-4 & 3.998997950678442E7 & 3272882.094030277 & 5.614354733338251E7 & 4594931.356031204 & 3.497981640346092E7 & 2862837.545088792 & 1.9785810708190208 & 0.10945534749339468 & 0.8609312786463065 & 0.05258688010329076 & 309.44793301978825 & 60.78570715537409 & 6.398382656976735E11 & 5.236862299527359E10 & 8.798950960821568E10 & 4.399475480410785E9 & 72.98445833576889 & 6.204715161462542 & 1.0294446795905384E10 & 1.6315173398651383E9\\
%   DEIMOS\_COSMOS\_920848 & 4.552800178527832 & -2.2321025995819075 & 0.15333296915869338 & 2.2025938199936415E-9 & 9.126191938839644E-10 & 5.136694029395381E-4 & 4.688293826570269E-4 & 7.211612207191463E-4 & 6.58208505258667E-4 & 4.493140938932489E-4 & 4.1009187631887864E-4 & 2163653.902196562 & 1916613.5732397295 & 3037641.098326191 & 2690811.203109834 & 1892579.52099294 & 1676489.7540628382 & 0.384652103575892 & 0.2654825240351925 & -0.31487136188394793 & 0.3383000773282165 & 788.1666212406101 & 218.8702275550039 & 3.4571855229765564E10 & 3.066839546876027E10 & 5.221052094875314E10 & 2.678928290988139E9 & 9.277661247314393 & 3.2580967166320245 & 4.212152582604257E9 & 9.262078656808653E8\\
%   DEIMOS\_COSMOS\_926434 & 4.449999809265137 & -1.9133213134380969 & 0.10648154069090557 & 1.102044240126919E-9 & 1.4993870928248032E-10 & 4.914040896073463E-4 & 9.856852040571518E-5 & 6.899020480870016E-4 & 1.3838432675467849E-4 & 4.298383006537582E-4 & 8.621931767601333E-5 & 2.2287163247805618E7 & 3877603.8360307366 & 3.1289848611143067E7 & 5443924.632953699 & 1.9494905678307258E7 & 3391796.4435740607 & 0.8613643586930183 & 0.11438103173614284 & 0.2499673873543996 & 0.0868941736190789 & 1134.5940135585427 & 62.35706893875254 & 3.5651009722890857E11 & 6.206310638784467E10 & 1.973975291035987E11 & 9.869876455179935E9 & 49.982164181088166 & 4.620793883806354 & 4.535404511104915E10 & 4.527277019236413E9\\
%   DEIMOS\_COSMOS\_933876 & 4.4166998863220215 & -2.2741286215429075 & 0.17493668666521117 & 5.730214435882312E-9 & 2.743438319724295E-9 & 0.0011809478209882792 & 0.0010576409367559871 & 0.0016579803416668913 & 0.0014848648268101477 & 0.0010329922262958147 & 9.251339021624745E-4 & 2834427.682449874 & 2403178.55626276 & 3979367.499442618 & 3373919.4340226674 & 2479315.097527447 & 2102095.217841863 & 0.38500429781230033 & 0.25956737000985486 & -0.3226827583051386 & 0.34200236765836256 & 404.4375425259081 & 166.2306892012592 & 4.527658509972154E10 & 3.8445388294498184E10 & 6.965877185550325E10 & 3.4829385927751627E9 & 13.753256608616844 & 5.255072433648007 & 2.400129482501501E9 & 6.923870704092631E8\\
%   vuds\_cosmos\_5100537582 & 4.550099849700928 & -1.8564992699302598 & 0.37742589578813485 & 1.4112118897949223E-8 & 3.012831879991315E-9 & 0.006745947423633004 & 0.0014281061434559448 & 0.009470908041425597 & 0.002004975892738595 & 0.005900778276369192 & 0.0012491852038650976 & 2.4199888822297096E7 & 2055977.2568657114 & 3.397520129578285E7 & 2886469.507132781 & 2.116799454334569E7 & 1798393.194041341 & 1.854684731450635 & 0.12536863132507253 & 0.7987817882888595 & 0.06211506564580225 & 163.63991557039333 & 42.20891951765924 & 3.8714447773610724E11 & 3.2895667977623043E10 & 6.145890909285344E10 & 3.7248194091557364E9 & 50.62472132246314 & 4.522558008671067 & 3.5873224771242495E9 & 6.955921026435738E8\\
%   vuds\_cosmos\_5100541407 & 4.563000202178955 & -2.1643818540980546 & 0.13377280983261833 & 1.0698908422600867E-8 & 3.15655478555671E-9 & 0.005700591373596178 & 0.001624983988420917 & 0.008003290463238959 & 0.002281380650730782 & 0.004986390143203691 & 0.001421397116842333 & 4.213289981574288E7 & 2732228.2405633787 & 5.915207970277934E7 & 3835885.575376458 & 3.685425994904708E7 & 2389919.7600499853 & 2.2392670746827643 & 0.116185930428098 & 0.9832354480750288 & 0.05390574332393505 & 214.68016240501794 & 73.25410545429442 & 6.741091357372656E11 & 4.370829073902947E10 & 7.012240499046867E10 & 4.712090697190183E9 & 79.07531116773961 & 7.905348431099234 & 7.390969998462394E9 & 2.0515940204602988E9\\
%   vuds\_cosmos\_5100559223 & 4.562699794769287 & -1.4450857796220564 & 0.31675415941517804 & 1.0345472883092317E-8 & 2.028980778180627E-9 & 0.0052608261300072425 & 0.0010272619477722908 & 0.007385886276652088 & 0.0014422145372380538 & 0.004601721091829098 & 8.985609588832168E-4 & 2.5595815075412296E7 & 2336997.6845574644 & 3.593499854079991E7 & 3281005.4353415626 & 2.2389031529335067E7 & 2044205.8472989374 & 1.8977234616932537 & 0.1233009876278326 & 0.8197825604358633 & 0.06045656544120173 & 219.97684844297936 & 50.11199360347589 & 4.095021647267132E11 & 3.739255031826971E10 & 6.187485642666733E10 & 3.241061954459957E9 & 50.3344539886854 & 4.687201538791264 & 4.865360390721952E9 & 8.397859853897148E8\\
%   vuds\_cosmos\_5100822662 & 4.520500183105469 & -0.9945562732976893 & 0.21255113666765837 & 2.7534968574646403E-9 & 5.409654086788442E-10 & 0.0015186815357788467 & 3.051188780995237E-4 & 0.0021321383441536505 & 4.283687160175451E-4 & 0.0013284128162120616 & 2.6689191814515946E-4 & 2.8199607306831934E7 & 2819486.268418455 & 3.9590567615702815E7 & 3958390.6448343704 & 2.4666606445130274E7 & 2466245.625472868 & 1.5064783257468723 & 0.10361471118993526 & 0.6315444262956027 & 0.05445026299541032 & 652.9988328808273 & 111.43012370418501 & 4.511937097725328E11 & 4.511840371839686E10 & 1.0499677164715376E11 & 5.249838582357689E9 & 51.12825057247935 & 4.638350332808961 & 1.856847972565225E10 & 3.2358389766256013E9\\
%   vuds\_cosmos\_5100969402 & 4.578499794006348 & -1.775685771479118 & 0.3219585744406674 & 8.09041673216147E-9 & 1.5617206729020463E-9 & 0.0041033539415620286 & 8.001794491766594E-4 & 0.005760864323639511 & 0.0011234042461169078 & 0.003589263342580769 & 6.99928596294315E-4 & 2.9507325242448777E7 & 2830456.4406895563 & 4.1426525641251735E7 & 3973792.1127459356 & 2.5810486333531562E7 & 2475841.394630298 & 1.7175969933194906 & 0.10785475852105758 & 0.7305329829226186 & 0.054738901680821364 & 275.2931910675446 & 58.037755981270514 & 4.720791887268922E11 & 4.528924112648414E10 & 8.748896168849571E10 & 4.374448084424786E9 & 58.17839778451132 & 5.343508916520993 & 7.191026088092267E9 & 1.2209089776699162E9\\
%   vuds\_cosmos\_5100994794 & 4.5802001953125 & -1.3950899978801197 & 0.24658841348203298 & 1.2267247833202358E-8 & 3.064008277706914E-9 & 0.0054453412887313256 & 0.0013361710561262112 & 0.007644934560130067 & 0.001875904510588477 & 0.004763119183436743 & 0.0011687682465299574 & 2.0291977342678417E7 & 2067643.5605076998 & 2.8488726537939634E7 & 2902848.3019910892 & 1.774968756334718E7 & 1808597.879428453 & 1.4941384110394789 & 0.11535357734157273 & 0.6130039428443802 & 0.06265875647861936 & 189.1554339028532 & 58.177152462265326 & 3.245979665322811E11 & 3.307761281978923E10 & 7.887111928951979E10 & 4.143409311295778E9 & 45.71370312518262 & 5.122701450765603 & 3.726484028589898E9 & 8.318345135966165E8\\
%   vuds\_cosmos\_5101013812 & 4.416299819946289 & -2.260745457434047 & 0.12765384857413822 & 1.5600448358414752E-9 & 5.306463288414141E-10 & 3.7923503417921155E-4 & 3.069040643702909E-4 & 5.324233809198457E-4 & 4.308750111226655E-4 & 3.317223972845123E-4 & 2.6845344652720875E-4 & 4247178.590319195 & 3329838.1168978703 & 5962785.556778306 & 4674894.216858513 & 3715068.85360796 & 2912657.8062530104 & 0.3927260115115557 & 0.25308098861355854 & -0.2890982994353858 & 0.3262096461483151 & 952.4997037673152 & 191.14171080091788 & 6.7869599745993774E10 & 5.328955224323542E10 & 1.0162309161680408E11 & 5.966449779878619E9 & 17.471458144852853 & 4.7992495249701745 & 1.1199330777841969E10 & 2.246734542916639E9\\
%   vuds\_cosmos\_5101210235 & 4.576099872589111 & -2.2237543029091507 & 0.10905846008166152 & 4.973920401802617E-9 & 1.0365447401602568E-9 & 9.94322048057163E-4 & 3.6445475606649826E-4 & 0.0013959688816607759 & 5.116727515357799E-4 & 8.697479497595661E-4 & 3.1879387316043544E-4 & 5985705.1898269765 & 1912137.4774556817 & 8403573.264940307 & 2684527.031459338 & 5235783.342921421 & 1672574.4480121376 & 0.3778565096352737 & 0.10771574312395378 & -0.25990724764170026 & 0.16294949091139116 & 418.30530206004045 & 84.00450492774229 & 9.560577361145383E10 & 3.059807713843398E10 & 1.6397533513620657E11 & 8.198766756810329E9 & 29.942432857673698 & 3.158749041079007 & 6.019885812169843E9 & 1.0819036686933427E9\\
%   vuds\_cosmos\_5101218326 & 4.57390022277832 & -0.4291648102146993 & 0.13665642945583834 & 1.0263337389453919E-9 & 7.997929014037916E-11 & 7.403532503087284E-4 & 6.345201374350625E-5 & 0.0010394118292828807 & 8.908284477621721E-5 & 6.475977504592443E-4 & 5.5502398814712495E-5 & 8.037662088811041E7 & 4936924.896922415 & 1.1284398429269986E8 & 6931148.253894316 & 7.030659871480292E7 & 4318399.974741761 & 2.0183737798698993 & 0.07172630025076489 & 0.9252814106545022 & 0.03502483156334386 & 1175.7874446648148 & 28.69291936058234 & 1.2863215577792021E12 & 7.90228382736962E10 & 1.5262308038890012E11 & 7.631154019445006E9 & 111.42415840747756 & 5.571207920373879 & 1.0856522998257013E11 & 6.489118070600704E9\\
%   vuds\_cosmos\_5101244930 & 4.5802998542785645 & -1.9239948795605761 & 0.2304393427036423 & 1.6377868317501384E-8 & 3.29903310508562E-9 & 0.0064884813359655895 & 0.0013472351276656378 & 0.009109441002482904 & 0.0018914378074752216 & 0.005675568946737113 & 0.0011784461507423922 & 2.2034967016738575E7 & 2383632.037731015 & 3.093578013671908E7 & 3346477.287216773 & 1.927430596885071E7 & 2084997.5939370724 & 1.3010954786757352 & 0.10277866974993023 & 0.5063770241041707 & 0.060068215509645285 & 141.42796173423406 & 34.82615094439069 & 3.5242960186732764E11 & 3.813559381784913E10 & 1.0928157024308931E11 & 5.464078512154466E9 & 55.619453843574185 & 5.324552073534778 & 3.396013007635387E9 & 6.018749096392831E8\\
%   vuds\_cosmos\_5101288969 & 5.720900058746338 & -2.1004767903011485 & 0.19965432129040517 & 3.010824634500857E-9 & 8.261969391711142E-10 & 9.670120308966441E-4 & 3.762285128598058E-4 & 0.001357627245579993 & 5.282024042130122E-4 & 8.458594807472663E-4 & 3.2909254938103785E-4 & 4866189.968472269 & 1441583.9424561746 & 6831840.631021177 & 2023897.919092493 & 4256527.104562412 & 1260974.4305755242 & 0.6492460778111071 & 0.19223267655332335 & 0.037767537993442464 & 0.18900988028846438 & 610.8067708335365 & 139.8066232946321 & 7.780402450221852E10 & 2.3076130161597904E10 & 6.803769334097517E10 & 6.831368423453488E9 & 15.151046900266753 & 1.6382276825541144 & 5.032191754595012E9 & 1.2691593431517231E9\\
%   vuds\_cosmos\_510148750 & 4.508800029754639 & -2.4615572916284165 & 0.07547772153731716 & 1.108024522087609E-8 & 5.330939210206448E-9 & 0.0013953425671723006 & 0.001138337653879259 & 0.0019589777847480775 & 0.0015981582071353455 & 0.0012205264274101554 & 9.957204937073685E-4 & 1687125.7767233376 & 1190097.0001554373 & 2368624.0170932505 & 1670825.2438140851 & 1475753.4424171592 & 1040995.1463136973 & 0.25134118371848035 & 0.14961731962106067 & -0.5035702650850542 & 0.2584890028719613 & 218.38068973523812 & 112.03936488634021 & 2.6905619989989845E10 & 1.9036252794672047E10 & 7.106159156498656E10 & 3.5530795782493286E9 & 13.397260116875131 & 3.3764182330150034 & 1.209112239829638E9 & 4.955322723823919E8\\
%   vuds\_cosmos\_510327576 & 4.566100120544434 & -2.3019034673864205 & 0.1885808157211991 & 1.5945797794134774E-8 & 9.687532647421443E-9 & 0.0033815226811848872 & 0.00286979796125333 & 0.004747456264082395 & 0.004029025262379452 & 0.002957867045966325 & 0.0025102539945697482 & 3769926.481260964 & 2871496.011148748 & 5292752.045750335 & 4031409.2232079813 & 3297609.4960659244 & 2511739.30349759 & 0.5057278506738924 & 0.31255248030965194 & -0.17612710569608803 & 0.3740188727819444 & 181.06675201675438 & 113.39827664538765 & 6.022775967101698E10 & 4.5923730881289314E10 & 6.565244725976647E10 & 3.2826223629883237E9 & 17.7773420546383 & 8.507417098710286 & 1.114860622475547E9 & 4.172580373108057E8\\
%   vuds\_cosmos\_510581738 & 4.50439977645874 & -2.2787636056346243 & 0.14122041807226426 & 3.1563824841809717E-9 & 1.4710506163701177E-9 & 7.03228458617914E-4 & 6.796755545537249E-4 & 9.872908348427213E-4 & 9.542239615790806E-4 & 6.151241554892569E-4 & 5.945220879189573E-4 & 2519110.2230578694 & 2348479.936722244 & 3536680.583251187 & 3297125.8328975993 & 2203502.33207037 & 2054249.5401834033 & 0.3813586436729621 & 0.27400888800557605 & -0.32936401198864945 & 0.3474253778133007 & 627.773378552058 & 211.0429366533516 & 4.024728480006884E10 & 3.757558370430191E10 & 6.137089826161026E10 & 3.140720538736893E9 & 11.306816847839283 & 4.410972455133993 & 3.5822074493526444E9 & 9.134097378921969E8\\
%   vuds\_cosmos\_510605533 & 4.5019001960754395 & -1.999047649253923 & 0.2527208673387991 & 1.6771859458498012E-8 & 4.672140238930345E-9 & 0.0058854495154372095 & 0.0017455552891521662 & 0.008262820274567125 & 0.00245065556942645 & 0.00514808824712963 & 0.0015268625863205064 & 1.192201743790122E7 & 1680302.96560282 & 1.6737801784086E7 & 2359045.1970034195 & 1.0428361961673269E7 & 1469785.4303477681 & 1.0612078605506245 & 0.11873869886577493 & 0.36016305864754605 & 0.07747647343411268 & 138.08695108900847 & 43.708594387133665 & 1.9064901577691318E11 & 2.688812735061637E10 & 8.244202219327702E10 & 4.1221011096638513E9 & 33.97436345444345 & 3.311614352553523 & 2.0256766125731647E9 & 5.286208392479099E8\\
%   vuds\_cosmos\_510786441 & 4.463500022888184 & -1.9466749404687251 & 0.09596765572210356 & 6.707271710308263E-9 & 1.1677827574490937E-9 & 0.002119440013302019 & 4.108569883905916E-4 & 0.002975567434009295 & 5.768187195756075E-4 & 0.0018539049896456117 & 3.5938258031724087E-4 & 1.8416740650244888E7 & 2008348.5167036578 & 2.5856006008911207E7 & 2819601.595203395 & 1.6109390768415593E7 & 1756731.642649095 & 0.7219845402773054 & 0.06300384696674359 & 0.11403675357744526 & 0.0529687310205364 & 323.9035294601199 & 59.665686449161555 & 2.94453252027805E11 & 3.2134237765365234E10 & 2.252032417227306E11 & 1.126016208613653E10 & 58.28241553627276 & 3.9643629593326937 & 8.68943708463454E9 & 1.392657709977549E9\\
%   vuds\_cosmos\_5110377875 & 4.55049991607666 & -0.761508212471262 & 0.14626853737656523 & 3.9323951949104275E-9 & 7.009030362075547E-10 & 0.002146427956826596 & 3.8467236545510614E-4 & 0.0030134568979047604 & 5.400570698994479E-4 & 0.0018775117361666126 & 3.364785099932802E-4 & 4.2047707586659946E7 & 3384141.729691101 & 5.903247489165051E7 & 4751133.252057646 & 3.677974106784042E7 & 2960157.96576746 & 1.6188146478083685 & 0.0860529016183138 & 0.6860772147807965 & 0.043863635320502754 & 502.8443668512539 & 85.90978975260644 & 6.727572132248606E11 & 5.41506306688434E10 & 1.382891366017021E11 & 6.914456830085104E9 & 77.0341267429449 & 6.030531130212405 & 1.9589619792702347E10 & 3.136816764096629E9\\
%   vuds\_cosmos\_5131465996 & 4.473599910736084 & -2.155181020204242 & 0.2507117603022014 & 4.276142234750413E-9 & 3.5203523912071347E-9 & 0.0013772120879381742 & 0.0014994817913254487 & 0.0019335236727026988 & 0.0021051830474817603 & 0.0012046674336637618 & 0.001311618520634609 & 2706029.736867151 & 2793878.7480866145 & 3799104.437939681 & 3922439.212811322 & 2367003.548022821 & 2443846.355185577 & 0.6607801026207542 & 0.5017236346300233 & -0.06316321833311449 & 0.4676451819662839 & 596.7127982589313 & 315.8580444378781 & 4.326689009806636E10 & 4.469538631127866E10 & 2.9863047313223923E10 & 3.7322331143098507E9 & 8.402023295941063 & 6.277872923327978 & 1.9648605763534586E9 & 6.79117078076711E8\\
%   vuds\_cosmos\_5180966608 & 4.529600143432617 & -0.9098892949484128 & 0.19656561366393677 & 1.116069923338792E-9 & 1.1944560717351278E-10 & 8.221705152911523E-4 & 9.200018240422757E-5 & 0.001154278392003907 & 1.2916277175424116E-4 & 7.191645015057899E-4 & 8.047389694307865E-5 & 6.5778854238131456E7 & 4539620.843958438 & 9.234959012238717E7 & 6373357.047736196 & 5.753772002032399E7 & 3970872.344059352 & 2.1957935153559434 & 0.09530402318520734 & 1.0072717521446808 & 0.04440469975315361 & 1126.4580492199623 & 64.72752878740476 & 1.0527203493072771E12 & 7.266026398272993E10 & 1.0341431563452747E11 & 5.170715781726373E9 & 89.29267036639861 & 5.4281102935593655 & 8.000634055191997E10 & 7.047179821601525E9\\
%   HZ4 & 5.539999961853027 & -2.0743219660201873 & 0.18908890030304912 & 1.1986413523183947E-8 & 4.5566757643311125E-9 & 0.004194979381864882 & 0.001594694786478003 & 0.005889500979822655 & 0.002238856416811535 & 0.0036694094471602006 & 0.0013949027115928692 & 2.712559364417641E7 & 3124057.005492544 & 3.808271645774534E7 & 4385989.803528144 & 2.372715108161539E7 & 2732658.0766948285 & 0.981401744369243 & 0.08987612946519727 & 0.3076576481263269 & 0.061177937923180575 & 194.09483883837171 & 83.55888003331982 & 4.337707580708506E11 & 4.998550113212836E10 & 2.1236438646170026E11 & 1.0618219323085012E10 & 77.50659845589227 & 8.928933064970348 & 6.466204282538737E9 & 2.34256086414632E9\\
%   HZ6 & 5.289999961853027 & -1.1246840100067022 & 0.1262033639563695 & 1.666033790963239E-9 & 2.51056952803574E-10 & 6.321248549117232E-4 & 9.525577495867268E-5 & 8.87465613887673E-4 & 1.3373342962736377E-4 & 5.529287997040646E-4 & 8.332161107655661E-5 & 2.605692077438074E7 & 1302846.038719037 & 3.658236345458626E7 & 1829118.1727293131 & 2.2792367387253404E7 & 1139618.3693626702 & 0.7392713358976971 & 0.03694381563274263 & 0.14605067683614495 & 0.030010185855535873 & 899.7311175679959 & 91.81164671453233 & 4.167232915266105E11 & 2.0836164576330524E10 & 2.9768075387604834E11 & 1.4884037693802418E10 & 68.67584807218631 & 3.4337924036093157 & 4.122116156628521E10 & 5.859772751312891E9\\
%   566428 & 5.889999866485596 & -1.7247198308040363 & 0.21994562204914003 & 3.200584701194812E-9 & 1.2212497343446664E-9 & 0.00143153545774204 & 6.437402923212761E-4 & 0.002009790445567005 & 9.037729955878947E-4 & 0.001252184874922619 & 5.630889916582295E-4 & 2.2511184270436283E7 & 8408548.554011855 & 3.160436077251099E7 & 1.1805100917021452E7 & 1.9690860123365343E7 & 7355079.654117391 & 1.0653424852120406 & 0.2818431220556624 & 0.3557395667369545 & 0.1886709705026582 & 611.7238658580007 & 202.48612584777604 & 3.600967066923393E11 & 1.3454798305158333E11 & 1.477522324689251E11 & 1.0209425294900137E10 & 50.32984100539041 & 14.491357809451 & 1.572520201905663E10 & 3.9373941268238506E9\\
%   HZ9 & 5.547999858856201 & -2.4724782759646406 & 0.20459249954084302 & 5.227374353599531E-8 & 1.775955713871963E-8 & 0.01868849073127358 & 0.006291104630191133 & 0.02623752692303162 & 0.008832335873652439 & 0.01634709451468525 & 0.005502920672957952 & 4.320823595128202E7 & 3868791.4692797936 & 6.066178753382976E7 & 5431552.595360713 & 3.779487209881787E7 & 3384088.1382728377 & 1.9233284702552664 & 0.12176284968357923 & 0.8447426234802436 & 0.05717193879721455 & 43.66914765248916 & 19.177349517445442 & 6.910209524674553E11 & 6.193391239106474E10 & 9.85639222024152E10 & 4.928196110120761E9 & 120.85814083319323 & 12.159115500093556 & 2.3120238318109207E9 & 7.502600327397776E8\\
%   HZ10 & 5.658999919891357 & -1.8751804883618821 & 0.228544324568629 & 8.069880975428592E-9 & 1.7541127031074226E-9 & 0.004627218137501313 & 0.0010050881514082277 & 0.006496338425995373 & 0.0014110838489736256 & 0.0040474949701112106 & 8.791652168661178E-4 & 8.926219112845849E7 & 4753062.536720335 & 1.2531879522098358E8 & 6673016.460626412 & 7.807893617235778E7 & 4157572.8954909523 & 2.3918956698751392 & 0.10516940066535127 & 1.0543502673787923 & 0.04836738317209704 & 273.8284345473637 & 60.21552238444012 & 1.4282559910226753E12 & 7.607435783962924E10 & 1.2615309734247673E11 & 7.43848314463415E9 & 155.67350330313093 & 8.386104937608362 & 1.9290681458268112E10 & 4.0623146669758387E9\\
%   CLM1 & 6.1656999588012695 & -1.9814802101777753 & 0.12342473866739936 & 1.7910633740406976E-9 & 1.805819034888342E-10 & 1.264339700752159E-4 & 1.274755952957921E-5 & 1.775057569674693E-4 & 1.789681366834965E-5 & 1.1059363157816598E-4 & 1.115047563005677E-5 & 2276496.393598335 & 113824.81967991675 & 3196065.2294552764 & 159803.2614727638 & 1991284.4885979737 & 99564.22442989869 & 0.10594888390121328 & 0.005167367401446149 & -0.8387919071427611 & 0.021445620435219026 & 863.1037931946817 & 52.17406114577236 & 3.617883743553497E10 & 1.8089418717767487E9 & 2.495505618782326E11 & 1.2477528093911633E10 & 32.24884348157452 & 1.612442174078726 & 1.8005417311850933E10 & 1.5764201533131635E9\\
%   WMH5 & 6.069499969482422 & -1.658684729448018 & 0.18237343957591107 & 2.2593159081585406E-9 & 4.837493520011173E-10 & 0.0011576776734715975 & 2.5909205806352094E-4 & 0.0016253104417401866 & 3.637498044510113E-4 & 0.0010126374899880133 & 2.2663158957406408E-4 & 3.7297412558385186E7 & 3215829.3899723436 & 5.236334384790419E7 & 4514832.760576044 & 3.262458895221771E7 & 2812932.7154819425 & 1.2527176137975269 & 0.09610191828909616 & 0.49114007175260654 & 0.057259034862693126 & 741.2310936725041 & 119.2871983913246 & 5.967132500848519E11 & 5.14747824198444E10 & 1.9219719052077902E11 & 9.609859526038952E9 & 72.78937778390107 & 4.111573710700953 & 3.2217441359596405E10 & 6.653802880354073E9\\
\end{tabular}

%\end{sidewaystable}
\end{adjustbox}
 \caption{Physical parameters. Only the first rows are shown. The table contains for each object in the sample the following information, for PL+OT\_MBB: id, redshift, $\beta_{FUV}$, sSFR, sM\_dust, M\_dust, A\_FUV,  IRX, age\_main, L\_dust, L\_FUV, SFR, M\_star.}
 \label{Tab.Physical_parameters_plotmbb}
\end{table}

